Lower Mass Bound on the $W^\prime$ mass via Neutrinoless Double Beta Decay in a 3-3-1 Model

The discovery of neutrino masses has raised the importance of studies in the context of neutrinoless double beta decay, which constitutes a landmark for lepton number violation. The standard interpretation is that the light massive neutrinos, that we observed oscillating in terrestrial experiments, mediate double beta decay. In the minimal 3-3-1 model, object of our study, there is an additional contribution that stems from the mixing between a new charged vector boson, $W^{\prime}$, and the Standard Model W boson. Even after setting this mixing to be very small, we show that tight constraints arise from the non-observation of neutrinoless double beta decay. Indeed, we derive bounds on the mass of the $W^{\prime}$ gauge boson that might exceed those from collider probes, and most importantly push the scale of symmetry breaking beyond its validity, leading to the exclusion of the minimal 3-3-1 model.

==> darkmatter <==
@article{Akerib:2013tjd,
      author         = "Akerib, D. S. and others",
      title          = "{First results from the LUX dark matter experiment at the
                        Sanford Underground Research Facility}",
      collaboration  = "LUX",
      journal        = "Phys. Rev. Lett.",
      volume         = "112",
      year           = "2014",
      pages          = "091303",
      doi            = "10.1103/PhysRevLett.112.091303",
      eprint         = "1310.8214",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1310.8214;%%"
}

@article{Ade:2015xua,
      author         = "Ade, P. A. R. and others",
      title          = "{Planck 2015 results. XIII. Cosmological parameters}",
      collaboration  = "Planck",
      journal        = "Astron. Astrophys.",
      volume         = "594",
      year           = "2016",
      pages          = "A13",
      doi            = "10.1051/0004-6361/201525830",
      eprint         = "1502.01589",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1502.01589;%%"
}

@article{Doff:2015nru,
      author         = "Doff, A. and Siqueira, Clarissa",
      title          = "{Composite Higgs Models, Technicolor and The Muon
                        Anomalous Magnetic Moment}",
      journal        = "Phys. Lett.",
      volume         = "B754",
      year           = "2016",
      pages          = "294-301",
      doi            = "10.1016/j.physletb.2016.01.043",
      eprint         = "1512.03256",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1512.03256;%%"
}

@article{DellOro:2016tmg,
      author         = "Dell'Oro, Stefano and Marcocci, Simone and Viel, Matteo
                        and Vissani, Francesco",
      title          = "{Neutrinoless double beta decay: 2015 review}",
      journal        = "Adv. High Energy Phys.",
      volume         = "2016",
      year           = "2016",
      pages          = "2162659",
      doi            = "10.1155/2016/2162659",
      eprint         = "1601.07512",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1601.07512;%%"
}

@article{Griest:1988yr,
      author         = "Griest, Kim",
      title          = "{Calculations of Rates for Direct Detection of Neutralino
                        Dark Matter}",
      journal        = "Phys. Rev. Lett.",
      volume         = "61",
      year           = "1988",
      pages          = "666-669",
      doi            = "10.1103/PhysRevLett.61.666",
      reportNumber   = "FERMILAB-PUB-88-052-A",
      SLACcitation   = "%%CITATION = PRLTA,61,666;%%"
}

@article{Griest:1988ma,
      author         = "Griest, Kim",
      title          = "{Cross-Sections, Relic Abundance and Detection Rates for
                        Neutralino Dark Matter}",
      journal        = "Phys. Rev.",
      volume         = "D38",
      year           = "1988",
      pages          = "2357",
      doi            = "10.1103/PhysRevD.38.2357, 10.1103/PhysRevD.39.3802",
      note           = "[Erratum: Phys. Rev.D39,3802(1989)]",
      reportNumber   = "FERMILAB-PUB-88-074-A, FERMILAB-PUB-89-139-A",
      SLACcitation   = "%%CITATION = PHRVA,D38,2357;%%"
}

@article{Pato:2010zk,
      author         = "Pato, Miguel and Baudis, Laura and Bertone, Gianfranco
                        and Ruiz de Austri, Roberto and Strigari, Louis E. and
                        Trotta, Roberto",
      title          = "{Complementarity of Dark Matter Direct Detection
                        Targets}",
      journal        = "Phys. Rev.",
      volume         = "D83",
      year           = "2011",
      pages          = "083505",
      doi            = "10.1103/PhysRevD.83.083505",
      eprint         = "1012.3458",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1012.3458;%%"
}

@article{Queiroz:2016sxf,
      author         = "Queiroz, Farinaldo S. and Rodejohann, Werner and Yaguna,
                        Carlos E.",
      title          = "{Is the dark matter particle its own antiparticle?}",
      journal        = "Phys. Rev.",
      volume         = "D95",
      year           = "2017",
      number         = "9",
      pages          = "095010",
      doi            = "10.1103/PhysRevD.95.095010",
      eprint         = "1610.06581",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1610.06581;%%"
}

@article{Arcadi:2017hfi,
      author         = "Arcadi, Giorgio and Campos, Miguel D. and Lindner,
                        Manfred and Masiero, Antonio and Queiroz, Farinaldo S.",
      title          = "{The Dark Sequential Z' Portal: Collider and Direct
                        Detection Experiments}",
      year           = "2017",
      eprint         = "1708.00890",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1708.00890;%%"
}

@article{Pato:2010yq,
      author         = "Pato, Miguel and Agertz, Oscar and Bertone, Gianfranco
                        and Moore, Ben and Teyssier, Romain",
      title          = "{Systematic uncertainties in the determination of the
                        local dark matter density}",
      journal        = "Phys. Rev.",
      volume         = "D82",
      year           = "2010",
      pages          = "023531",
      doi            = "10.1103/PhysRevD.82.023531",
      eprint         = "1006.1322",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1006.1322;%%"
}

@article{Abercrombie:2015wmb,
      author         = "Abercrombie, Daniel and others",
      editor         = "Boveia, Antonio and Doglioni, Caterina and Lowette,
                        Steven and Malik, Sarah and Mrenna, Stephen",
      title          = "{Dark Matter Benchmark Models for Early LHC Run-2
                        Searches: Report of the ATLAS/CMS Dark Matter Forum}",
      year           = "2015",
      eprint         = "1507.00966",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "FERMILAB-PUB-15-282-CD",
      SLACcitation   = "%%CITATION = ARXIV:1507.00966;%%"
}

@article{Navarro:1995iw,
      author         = "Navarro, Julio F. and Frenk, Carlos S. and White, Simon
                        D. M.",
      title          = "{The Structure of cold dark matter halos}",
      journal        = "Astrophys. J.",
      volume         = "462",
      year           = "1996",
      pages          = "563-575",
      doi            = "10.1086/177173",
      eprint         = "astro-ph/9508025",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9508025;%%"
}

@article{Racker:2013lua,
      author         = "Racker, J.",
      title          = "{Mass bounds for baryogenesis from particle decays and
                        the inert doublet model}",
      journal        = "JCAP",
      volume         = "1403",
      pages          = "025",
      doi            = "10.1088/1475-7516/2014/03/025",
      year           = "2014",
      eprint         = "1308.1840",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-13-50",
      SLACcitation   = "%%CITATION = ARXIV:1308.1840;%%",
}

@article{Dienes:2011ja,
      author         = "Dienes, Keith R. and Thomas, Brooks",
      title          = "{Dynamical Dark Matter: I. Theoretical Overview}",
      journal        = "Phys. Rev.",
      volume         = "D85",
      year           = "2012",
      pages          = "083523",
      doi            = "10.1103/PhysRevD.85.083523",
      eprint         = "1106.4546",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1106.4546;%%"
}

@article{Profumo:2009tb,
      author         = "Profumo, Stefano and Sigurdson, Kris and Ubaldi, Lorenzo",
      title          = "{Can we discover multi-component WIMP dark matter?}",
      journal        = "JCAP",
      volume         = "0912",
      year           = "2009",
      pages          = "016",
      doi            = "10.1088/1475-7516/2009/12/016",
      eprint         = "0907.4374",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0907.4374;%%"
}

@article{McDermott:2011hx,
      author         = "McDermott, Samuel D. and Yu, Hai-Bo and Zurek, Kathryn
                        M.",
      title          = "{The Dark Matter Inverse Problem: Extracting Particle
                        Physics from Scattering Events}",
      journal        = "Phys. Rev.",
      volume         = "D85",
      year           = "2012",
      pages          = "123507",
      doi            = "10.1103/PhysRevD.85.123507",
      eprint         = "1110.4281",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MCTP-11-34",
      SLACcitation   = "%%CITATION = ARXIV:1110.4281;%%"
}

@article{Pato:2011de,
      author         = "Pato, Miguel",
      title          = "{What can(not) be measured with ton-scale dark matter
                        direct detection experiments}",
      journal        = "JCAP",
      volume         = "1110",
      year           = "2011",
      pages          = "035",
      doi            = "10.1088/1475-7516/2011/10/035",
      eprint         = "1106.0743",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1106.0743;%%"
}

@inproceedings{Gondolo:1996qw,
      author         = "Gondolo, Paolo",
      title          = "{Phenomenological introduction to direct dark matter
                        detection}",
      booktitle      = "{Dark matter in cosmology, quantum measurements,
                        experimental gravitation. Proceedings, 31st Rencontres de
                        Moriond, 16th Moriond Workshop, Les Arcs, France, January
                        2-27, 1996}",
      year           = "1996",
      url            = "http://alice.cern.ch/format/showfull?sysnb=0225064",
      pages          = "41-51",
      eprint         = "hep-ph/9605290",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/9605290;%%"
}

@article{Ma:2006km,
      author         = "Ma, Ernest",
      title          = "{Verifiable radiative seesaw mechanism of neutrino mass
                        and dark matter}",
      journal        = "Phys.Rev.",
      volume         = "D73",
      pages          = "077301",
      doi            = "10.1103/PhysRevD.73.077301",
      year           = "2006",
      eprint         = "hep-ph/0601225",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T403",
      SLACcitation   = "%%CITATION = HEP-PH/0601225;%%",
}
@article{Ma:1998dn,
      author         = "Ma, Ernest",
      title          = "{Pathways to naturally small neutrino masses}",
      journal        = "Phys. Rev. Lett.",
      volume         = "81",
      year           = "1998",
      pages          = "1171-1174",
      doi            = "10.1103/PhysRevLett.81.1171",
      eprint         = "hep-ph/9805219",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T-222",
      SLACcitation   = "%%CITATION = HEP-PH/9805219;%%"
}

@book{Bertone:2010zza,
      author         = "J. Silk and others",
      editor         = "Bertone, Gianfranco",
      title          = "{Particle Dark Matter: Observations, Models and
                        Searches}",
      url            = "http://www.cambridge.org/uk/catalogue/catalogue.asp?isbn=9780521763684",
      journal        = "Cambridge, UK: Univ. Pr. (2010) 738 p",
      year           = "2010",
      ISBN           = "9781107653924",
      SLACcitation   = "%%CITATION = INSPIRE-895273;%%"
}

@article{Bertone:2004pz,
      author         = "Bertone, Gianfranco and Hooper, Dan and Silk, Joseph",
      title          = "{Particle dark matter: Evidence, candidates and
                        constraints}",
      journal        = "Phys. Rept.",
      volume         = "405",
      year           = "2005",
      pages          = "279-390",
      doi            = "10.1016/j.physrep.2004.08.031",
      eprint         = "hep-ph/0404175",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-04-047-A",
      SLACcitation   = "%%CITATION = HEP-PH/0404175;%%"
}

@article{Kelso:2016qqj,
      author         = "Kelso, Chris and Savage, Christopher and Valluri, Monica
                        and Freese, Katherine and Stinson, Gregory S. and Bailin,
                        Jeremy",
      title          = "{The impact of baryons on the direct detection of dark
                        matter}",
      journal        = "JCAP",
      volume         = "1608",
      year           = "2016",
      number         = "08",
      pages          = "071",
      doi            = "10.1088/1475-7516/2016/08/071",
      eprint         = "1601.04725",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.GA",
      reportNumber   = "NORDITA-2015-15, CETUP2015-030",
      SLACcitation   = "%%CITATION = ARXIV:1601.04725;%%"
}

@article{Duda:2006uk,
      author         = "Duda, Gintaras and Kemper, Ann and Gondolo, Paolo",
      title          = "{Model Independent Form Factors for Spin Independent
                        Neutralino-Nucleon Scattering from Elastic Electron
                        Scattering Data}",
      journal        = "JCAP",
      volume         = "0704",
      year           = "2007",
      pages          = "012",
      doi            = "10.1088/1475-7516/2007/04/012",
      eprint         = "hep-ph/0608035",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0608035;%%"
}
@article{Bozorgnia:2016ogo,
      author         = "Bozorgnia, Nassim and Calore, Francesca and Schaller,
                        Matthieu and Lovell, Mark and Bertone, Gianfranco and
                        Frenk, Carlos S. and Crain, Robert A. and Navarro, Julio
                        F. and Schaye, Joop and Theuns, Tom",
      title          = "{Simulated Milky Way analogues: implications for dark
                        matter direct searches}",
      journal        = "JCAP",
      volume         = "1605",
      year           = "2016",
      number         = "05",
      pages          = "024",
      doi            = "10.1088/1475-7516/2016/05/024",
      eprint         = "1601.04707",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1601.04707;%%"
}

@article{Sloane:2016kyi,
      author         = "Sloane, Jonathan D. and Buckley, Matthew R. and Brooks,
                        Alyson M. and Governato, Fabio",
      title          = "{Assessing Astrophysical Uncertainties in Direct
                        Detection with Galaxy Simulations}",
      year           = "2016",
      eprint         = "1601.05402",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.GA",
      SLACcitation   = "%%CITATION = ARXIV:1601.05402;%%"
}

@article{O'Hare:2015mda,
      author         = "O'Hare, Ciaran A. J. and Green, Anne M. and Billard,
                        Julien and Figueroa-Feliciano, Enectali and Strigari,
                        Louis E.",
      title          = "{Readout strategies for directional dark matter detection
                        beyond the neutrino background}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "6",
      pages          = "063518",
      doi            = "10.1103/PhysRevD.92.063518",
      eprint         = "1505.08061",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1505.08061;%%"
}

@article{Kavanagh:2013wba,
      author         = "Kavanagh, Bradley J. and Green, Anne M.",
      title          = "{Model independent determination of the dark matter mass
                        from direct detection experiments}",
      journal        = "Phys. Rev. Lett.",
      volume         = "111",
      year           = "2013",
      number         = "3",
      pages          = "031302",
      doi            = "10.1103/PhysRevLett.111.031302",
      eprint         = "1303.6868",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1303.6868;%%"
}

@article{Kavanagh:2012nr,
      author         = "Kavanagh, Bradley J. and Green, Anne M.",
      title          = "{Improved determination of the WIMP mass from direct
                        detection data}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "065027",
      doi            = "10.1103/PhysRevD.86.065027",
      eprint         = "1207.2039",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1207.2039;%%"
}

@article{Babu:1988ki,
      author         = "Babu, K. S.",
      title          = "{Model of 'Calculable' Majorana Neutrino Masses}",
      journal        = "Phys. Lett.",
      volume         = "B203",
      year           = "1988",
      pages          = "132",
      doi            = "10.1016/0370-2693(88)91584-5",
      reportNumber   = "UR-1039, ER13065-517",
      SLACcitation   = "%%CITATION = PHLTA,B203,132;%%"
}

@article{Zee:1980ai,
      author         = "Zee, A.",
      title          = "{A Theory of Lepton Number Violation, Neutrino Majorana
                        Mass, and Oscillation}",
      journal        = "Phys. Lett.",
      volume         = "B93",
      year           = "1980",
      pages          = "389",
      doi            = "10.1016/0370-2693(80)90349-4",
      note           = "[Erratum: Phys. Lett.B95,461(1980)]",
      reportNumber   = "UPR-0150T",
      SLACcitation   = "%%CITATION = PHLTA,B93,389;%%"
}

@article{Dev:2012sg,
      author         = "Dev, P. S. Bhupal and Pilaftsis, Apostolos",
      title          = "{Minimal Radiative Neutrino Mass Mechanism for Inverse
                        Seesaw Models}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "113001",
      doi            = "10.1103/PhysRevD.86.113001",
      eprint         = "1209.4051",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MAN-HEP-2012-14",
      SLACcitation   = "%%CITATION = ARXIV:1209.4051;%%"
}

@article{Krauss:2002px,
      author         = "Krauss, Lawrence M. and Nasri, Salah and Trodden, Mark",
      title          = "{A Model for neutrino masses and dark matter}",
      journal        = "Phys. Rev.",
      volume         = "D67",
      year           = "2003",
      pages          = "085002",
      doi            = "10.1103/PhysRevD.67.085002",
      eprint         = "hep-ph/0210389",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SU-DP-02-10-3, SU-4252-770, CWRU-P41-02",
      SLACcitation   = "%%CITATION = HEP-PH/0210389;%%"
}

@article{Law:2013saa,
      author         = "Law, Sandy S. C. and McDonald, Kristian L.",
      title          = "{A Class of Inert N-tuplet Models with Radiative Neutrino
                        Mass and Dark Matter}",
      journal        = "JHEP",
      volume         = "09",
      year           = "2013",
      pages          = "092",
      doi            = "10.1007/JHEP09(2013)092",
      eprint         = "1305.6467",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1305.6467;%%"
}
@article{Farzan:2012ev,
      author         = "Farzan, Yasaman and Pascoli, Silvia and Schmidt, Michael
                        A.",
      title          = "{Recipes and Ingredients for Neutrino Mass at Loop
                        Level}",
      journal        = "JHEP",
      volume         = "03",
      year           = "2013",
      pages          = "107",
      doi            = "10.1007/JHEP03(2013)107",
      eprint         = "1208.2732",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IPM-P-2012-027, IPPP-12-64, DCPT-12-128",
      SLACcitation   = "%%CITATION = ARXIV:1208.2732;%%"
}

@article{Hirsch:2013ola,
      author         = "Hirsch, M. and Lineros, R. A. and Morisi, S. and Palacio,
                        J. and Rojas, N. and Valle, J. W. F.",
      title          = "{WIMP dark matter as radiative neutrino mass messenger}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2013",
      pages          = "149",
      doi            = "10.1007/JHEP10(2013)149",
      eprint         = "1307.8134",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-13-53",
      SLACcitation   = "%%CITATION = ARXIV:1307.8134;%%"
}

@article{Farzan:2009ji,
      author         = "Farzan, Yasaman",
      title          = "{A Minimal model linking two great mysteries: neutrino
                        mass and dark matter}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "073009",
      doi            = "10.1103/PhysRevD.80.073009",
      eprint         = "0908.3729",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0908.3729;%%"
}

@article{Longas:2015sxk,
      author         = "Longas, Robinson and Portillo, Dilia and Restrepo, Diego
                        and Zapata, Oscar",
      title          = "{The Inert Zee Model}",
      year           = "2015",
      eprint         = "1511.01873",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1511.01873;%%"
}

@article{Tortola:2012te,
      author         = "Forero, D.V. and Tortola, M. and Valle, J.W.F.",
      title          = "{Global status of neutrino oscillation parameters after
                        Neutrino-2012}",
      journal        = "Phys.Rev.",
      volume         = "D86",
      pages          = "073012",
      doi            = "10.1103/PhysRevD.86.073012",
      year           = "2012",
      eprint         = "1205.4018",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-12-31",
      SLACcitation   = "%%CITATION = ARXIV:1205.4018;%%",
}
@article{Belanger:2010gh,
      author         = "Belanger, G. and Boudjema, F. and Brun, P. and Pukhov, A.
                        and Rosier-Lees, S. and others",
      title          = "{Indirect search for dark matter with micrOMEGAs2.4}",
      journal        = "Comput.Phys.Commun.",
      volume         = "182",
      pages          = "842-856",
      doi            = "10.1016/j.cpc.2010.11.033",
      year           = "2011",
      eprint         = "1004.1092",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IRFU-10-24, LAPTH-012-10.",
      SLACcitation   = "%%CITATION = ARXIV:1004.1092;%%",
}
@article{Miao:2010rg,
      author         = "Miao, Xinyu and Su, Shufang and Thomas, Brooks",
      title          = "{Trilepton Signals in the Inert Doublet Model}",
      journal        = "Phys.Rev.",
      volume         = "D82",
      pages          = "035009",
      doi            = "10.1103/PhysRevD.82.035009",
      year           = "2010",
      eprint         = "1005.0090",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1005.0090;%%",
}
@article{Dolle:2009fn,
      author         = "Dolle, Ethan M. and Su, Shufang",
      title          = "{The Inert Dark Matter}",
      journal        = "Phys.Rev.",
      volume         = "D80",
      pages          = "055012",
      doi            = "10.1103/PhysRevD.80.055012",
      year           = "2009",
      eprint         = "0906.1609",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0906.1609;%%",
}
@article{Profumo:2006bx,
      author         = "Profumo, Stefano and Provenza, Alessio",
      title          = "{Increasing the neutralino relic abundance with slepton
                        coannihilations: Consequences for indirect dark matter
                        detection}",
      journal        = "JCAP",
      volume         = "0612",
      pages          = "019",
      doi            = "10.1088/1475-7516/2006/12/019",
      year           = "2006",
      eprint         = "hep-ph/0609290",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SISSA-56-2006-EP",
      SLACcitation   = "%%CITATION = HEP-PH/0609290;%%",
}

@article{Fitzpatrick:2012ix,
      author         = "Fitzpatrick, A. Liam and Haxton, Wick and Katz, Emanuel
                        and Lubbers, Nicholas and Xu, Yiming",
      title          = "{The Effective Field Theory of Dark Matter Direct
                        Detection}",
      journal        = "JCAP",
      volume         = "1302",
      year           = "2013",
      pages          = "004",
      doi            = "10.1088/1475-7516/2013/02/004",
      eprint         = "1203.3542",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1203.3542;%%"
}


@article{Suematsu:2011va,
      author         = "Suematsu, Daijiro",
      title          = "{Thermal Leptogenesis in a TeV Scale Model for Neutrino
                        Masses}",
      journal        = "Eur.Phys.J.",
      volume         = "C72",
      pages          = "1951",
      doi            = "10.1140/epjc/s10052-012-1951-z",
      year           = "2012",
      eprint         = "1103.0857",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KANAZAWA-11-04",
      SLACcitation   = "%%CITATION = ARXIV:1103.0857;%%",
}
@article{Dolle:2009ft,
      author         = "Dolle, Ethan and Miao, Xinyu and Su, Shufang and Thomas,
                        Brooks",
      title          = "{Dilepton Signals in the Inert Doublet Model}",
      journal        = "Phys.Rev.",
      volume         = "D81",
      pages          = "035003",
      doi            = "10.1103/PhysRevD.81.035003",
      year           = "2010",
      eprint         = "0909.3094",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0909.3094;%%",
}

@article{Roszkowski:2016bhs,
      author         = "Roszkowski, Leszek and Sessolo, Enrico Maria and
                        Trojanowski, Sebastian and Williams, Andrew J.",
      title          = "{Reconstructing WIMP properties through an interplay of
                        signal measurements in direct detection, Fermi-LAT, and
                        CTA searches for dark matter}",
      year           = "2016",
      eprint         = "1603.06519",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1603.06519;%%"
}



@article{Suematsu:2009ww,
      author         = "Suematsu, Daijiro and Toma, Takashi and Yoshida, Tetsuro",
      title          = "{Reconciliation of CDM abundance and mu to e gamma
                        in a radiative seesaw model}",
      journal        = "Phys.Rev.",
      volume         = "D79",
      pages          = "093004",
      doi            = "10.1103/PhysRevD.79.093004",
      year           = "2009",
      eprint         = "0903.0287",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KANAZAWA-09-04",
      SLACcitation   = "%%CITATION = ARXIV:0903.0287;%%",
}
@article{Gelmini:2009xd,
      author         = "Gelmini, Graciela B. and Osoba, Efunwande and
                        Palomares-Ruiz, Sergio",
      title          = "{Inert-Sterile Neutrino: Cold or Warm Dark Matter
                        Candidate}",
      journal        = "Phys.Rev.",
      volume         = "D81",
      pages          = "063529",
      doi            = "10.1103/PhysRevD.81.063529",
      year           = "2010",
      eprint         = "0912.2478",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CFTP-09-39",
      SLACcitation   = "%%CITATION = ARXIV:0912.2478;%%",
}
@article{Kubo:2006yx,
      author         = "Kubo, Jisuke and Ma, Ernest and Suematsu, Daijiro",
      title          = "{Cold Dark Matter, Radiative Neutrino Mass, mu to e
                        gamma, and Neutrinoless Double Beta Decay}",
      journal        = "Phys.Lett.",
      volume         = "B642",
      pages          = "18-23",
      doi            = "10.1016/j.physletb.2006.08.085",
      year           = "2006",
      eprint         = "hep-ph/0604114",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T409, KANAZAWA-06-01",
      SLACcitation   = "%%CITATION = HEP-PH/0604114;%%",
}
@article{s,
      author         = "Ma, Ernest",
      title          = "{Verifiable radiative seesaw mechanism of neutrino mass
                        and dark matter}",
      journal        = "Phys.Rev.",
      volume         = "D73",
      pages          = "077301",
      doi            = "10.1103/PhysRevD.73.077301",
      year           = "2006",
      eprint         = "hep-ph/0601225",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T403",
      SLACcitation   = "%%CITATION = HEP-PH/0601225;%%",
}
@article{Gustafsson:2012aj,
      author         = "Gustafsson, Michael and Rydbeck, Sara and Lopez-Honorez,
                        Laura and Lundstrom, Erik",
      title          = "{Status of the Inert Doublet Model and the Role of
                        multileptons at the LHC}",
      journal        = "Phys.Rev.",
      volume         = "D86",
      pages          = "075019",
      doi            = "10.1103/PhysRevD.86.075019",
      year           = "2012",
      eprint         = "1206.6316",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-11-261, ULB-TH-12-08",
      SLACcitation   = "%%CITATION = ARXIV:1206.6316;%%",
}
@article{Komatsu:2010fb,
      author         = "Komatsu, E. and others",
      title          = "{Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP)
                        Observations: Cosmological Interpretation}",
      collaboration  = "WMAP Collaboration",
      journal        = "Astrophys.J.Suppl.",
      volume         = "192",
      pages          = "18",
      doi            = "10.1088/0067-0049/192/2/18",
      year           = "2011",
      eprint         = "1001.4538",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1001.4538;%%",
}
@article{Kashiwase:2012xd,
      author         = "Kashiwase, Shoichi and Suematsu, Daijiro",
      title          = "{Baryon number asymmetry and dark matter in the neutrino
                        mass model with an inert doublet}",
      journal        = "Phys.Rev.",
      volume         = "D86",
      pages          = "053001",
      doi            = "10.1103/PhysRevD.86.053001",
      year           = "2012",
      eprint         = "1207.2594",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KANAZAWA-12-06",
      SLACcitation   = "%%CITATION = ARXIV:1207.2594;%%",
}
@article{Hu:2012az,
      author         = "Hu, Ping-Kai",
      title          = "{Radiative Seesaw Model with Non-zero $\theta_{13}$ and
                        Warm Dark Matter Scenario}",
      year           = "2012",
      eprint         = "1208.2613",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1208.2613;%%",
}
@article{Griest:1990kh,
      author         = "Griest, Kim and Seckel, David",
      title          = "{Three exceptions in the calculation of relic
                        abundances}",
      journal        = "Phys.Rev.",
      volume         = "D43",
      pages          = "3191-3203",
      doi            = "10.1103/PhysRevD.43.3191",
      year           = "1991",
      reportNumber   = "CFPA-TH-90-001A, BA-90-79",
      SLACcitation   = "%%CITATION = PHRVA,D43,3191;%%",
}
@article{LopezHonorez:2006gr,
      author         = "Lopez Honorez, Laura and Nezri, Emmanuel and Oliver,
                        Josep F. and Tytgat, Michel H.G.",
      title          = "{The Inert Doublet Model: An Archetype for Dark Matter}",
      journal        = "JCAP",
      volume         = "0702",
      pages          = "028",
      doi            = "10.1088/1475-7516/2007/02/028",
      year           = "2007",
      eprint         = "hep-ph/0612275",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ULB-TH-06-27",
      SLACcitation   = "%%CITATION = HEP-PH/0612275;%%",
}
@article{Ackermann:2012rg,
      author         = "Ackermann, M. and others",
      title          = "{Constraints on the Galactic Halo Dark Matter from
                        Fermi-LAT Diffuse Measurements}",
      collaboration  = "LAT collaboration",
      journal        = "Astrophys.J.",
      volume         = "761",
      pages          = "91",
      doi            = "10.1088/0004-637X/761/2/91",
      year           = "2012",
      eprint         = "1205.6474",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "SACLAY-T12-043",
      SLACcitation   = "%%CITATION = ARXIV:1205.6474;%%",
}

@article{Hooper:2007qk,
      author         = "Hooper, Dan and Profumo, Stefano",
      title          = "{Dark matter and collider phenomenology of universal
                        extra dimensions}",
      journal        = "Phys.Rept.",
      volume         = "453",
      pages          = "29-115",
      doi            = "10.1016/j.physrep.2007.09.003",
      year           = "2007",
      eprint         = "hep-ph/0701197",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-07-018-A",
      SLACcitation   = "%%CITATION = HEP-PH/0701197;%%",
}

@article{Kashiwase:2013uy,
      author         = "Kashiwase, Shoichi and Suematsu, Daijiro",
      title          = "{Leptogenesis in a TeV scale neutrino mass model with
                        inverted mass hierarchy}",
      year           = "2013",
      eprint         = "1301.2087",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KANAZAWA-13-01",
      SLACcitation   = "%%CITATION = ARXIV:1301.2087;%%",
}
@article{Edsjo:2003us,
      author         = "Edsjo, Joakim and Schelke, Mia and Ullio, Piero and
                        Gondolo, Paolo",
      title          = "{Accurate relic densities with neutralino, chargino and
                        sfermion coannihilations in mSUGRA}",
      journal        = "JCAP",
      volume         = "0304",
      pages          = "001",
      doi            = "10.1088/1475-7516/2003/04/001",
      year           = "2003",
      eprint         = "hep-ph/0301106",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "NSF-ITP-03-03, CWRU-P1-03",
      SLACcitation   = "%%CITATION = HEP-PH/0301106;%%",
}
@article{Cao:2007rm,
      author         = "Cao, Qing-Hong and Ma, Ernest and Rajasekaran, G.",
      title          = "{Observing the Dark Scalar Doublet and its Impact on the
                        Standard-Model Higgs Boson at Colliders}",
      journal        = "Phys.Rev.",
      volume         = "D76",
      pages          = "095011",
      doi            = "10.1103/PhysRevD.76.095011",
      year           = "2007",
      eprint         = "0708.2939",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T437",
      SLACcitation   = "%%CITATION = ARXIV:0708.2939;%%",
}
@article{Hambye:2009pw,
      author         = "Hambye, T. and Ling, F.-S. and Lopez Honorez, L. and
                        Rocher, J.",
      title          = "{Scalar Multiplet Dark Matter}",
      journal        = "JHEP",
      volume         = "0907",
      pages          = "090",
      doi            = "10.1007/JHEP05(2010)066, 10.1088/1126-6708/2009/07/090",
      year           = "2009",
      eprint         = "0903.4010",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ULB-TH-09-03, FTUAM-09-04",
      SLACcitation   = "%%CITATION = ARXIV:0903.4010;%%",
}
@article{Barbieri:2006dq,
      author         = "Barbieri, Riccardo and Hall, Lawrence J. and Rychkov,
                        Vyacheslav S.",
      title          = "{Improved naturalness with a heavy Higgs: An Alternative
                        road to LHC physics}",
      journal        = "Phys.Rev.",
      volume         = "D74",
      pages          = "015007",
      doi            = "10.1103/PhysRevD.74.015007",
      year           = "2006",
      eprint         = "hep-ph/0603188",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCB-PTH-06-04, LBNL-59894",
      SLACcitation   = "%%CITATION = HEP-PH/0603188;%%",
}
@article{Schmidt:2012yg,
      author         = "Schmidt, Daniel and Schwetz, Thomas and Toma, Takashi",
      title          = "{Direct Detection of Leptophilic Dark Matter in a Model
                        with Radiative Neutrino Masses}",
      journal        = "Phys.Rev.",
      volume         = "D85",
      pages          = "073009",
      doi            = "10.1103/PhysRevD.85.073009",
      year           = "2012",
      eprint         = "1201.0906",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KANAZAWA-11-14",
      SLACcitation   = "%%CITATION = ARXIV:1201.0906;%%",
}
@article{Bertone:2010at,
      author         = "Bertone, Gianfranco",
      title          = "{The moment of truth for WIMP Dark Matter}",
      journal        = "Nature",
      volume         = "468",
      pages          = "389-393",
      doi            = "10.1038/nature09509",
      year           = "2010",
      eprint         = "1011.3532",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1011.3532;%%",
}



@article{Fukuda:1998mi,
      author         = "Fukuda, Y. and others",
      title          = "{Evidence for oscillation of atmospheric neutrinos}",
      collaboration  = "Super-Kamiokande Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "81",
      pages          = "1562-1567",
      doi            = "10.1103/PhysRevLett.81.1562",
      year           = "1998",
      eprint         = "hep-ex/9807003",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "BU-98-17, ICRR-REPORT-422-98-18, UCI-98-8,
                        KEK-PREPRINT-98-95, LSU-HEPA-5-98, UMD-98-003, SBHEP-98-5,
                        TKU-PAP-98-06, TIT-HPE-98-09",
      SLACcitation   = "%%CITATION = HEP-EX/9807003;%%",
}
@article{Ahmad:2002jz,
      author         = "Ahmad, Q.R. and others",
      title          = "{Direct evidence for neutrino flavor transformation from
                        neutral current interactions in the Sudbury Neutrino
                        Observatory}",
      collaboration  = "SNO Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "89",
      pages          = "011301",
      doi            = "10.1103/PhysRevLett.89.011301",
      year           = "2002",
      eprint         = "nucl-ex/0204008",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
      SLACcitation   = "%%CITATION = NUCL-EX/0204008;%%",
}

@article{Araki:2004mb,
      author         = "Araki, T. and others",
      title          = "{Measurement of neutrino oscillation with KamLAND:
                        Evidence of spectral distortion}",
      collaboration  = "KamLAND Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "94",
      pages          = "081801",
      doi            = "10.1103/PhysRevLett.94.081801",
      year           = "2005",
      eprint         = "hep-ex/0406035",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = HEP-EX/0406035;%%",
}

@article{Adamson:2008zt,
      author         = "Adamson, P. and others",
      title          = "{Measurement of Neutrino Oscillations with the MINOS
                        Detectors in the NuMI Beam}",
      collaboration  = "MINOS Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "101",
      pages          = "131802",
      doi            = "10.1103/PhysRevLett.101.131802",
      year           = "2008",
      eprint         = "0806.2237",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "FERMILAB-PUB-08-168-E, BNL-XXXX",
      SLACcitation   = "%%CITATION = ARXIV:0806.2237;%%",
}


@article{Servant:2002aq,
      author         = "Servant, Geraldine and Tait, Timothy M.P.",
      title          = "{Is the lightest Kaluza-Klein particle a viable dark
                        matter candidate?}",
      journal        = "Nucl.Phys.",
      volume         = "B650",
      pages          = "391-419",
      doi            = "10.1016/S0550-3213(02)01012-X",
      year           = "2003",
      eprint         = "hep-ph/0206071",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ANL-HEP-PR-02-032, EFI-02-74",
      SLACcitation   = "%%CITATION = HEP-PH/0206071;%%",
}
@article{Kong:2005hn,
      author         = "Kong, Kyoungchul and Matchev, Konstantin T.",
      title          = "{Precise calculation of the relic density of Kaluza-Klein
                        dark matter in universal extra dimensions}",
      journal        = "JHEP",
      volume         = "0601",
      pages          = "038",
      doi            = "10.1088/1126-6708/2006/01/038",
      year           = "2006",
      eprint         = "hep-ph/0509119",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UFIFT-HEP-05-22",
      SLACcitation   = "%%CITATION = HEP-PH/0509119;%%",
}
@article{Burnell:2005hm,
      author         = "Burnell, Fiona and Kribs, Graham D.",
      title          = "{The Abundance of Kaluza-Klein dark matter with
                        coannihilation}",
      journal        = "Phys.Rev.",
      volume         = "D73",
      pages          = "015001",
      doi            = "10.1103/PhysRevD.73.015001",
      year           = "2006",
      eprint         = "hep-ph/0509118",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0509118;%%",
}

@article{Klasen:2013btp,
      author         = "Klasen, Michael and Yaguna, Carlos E. and Ruiz-Alvarez,
                        Jose D.",
      title          = "{Electroweak corrections to the direct detection cross
                        section of inert higgs dark matter}",
      journal        = "Phys. Rev.",
      volume         = "D87",
      year           = "2013",
      pages          = "075025",
      doi            = "10.1103/PhysRevD.87.075025",
      eprint         = "1302.1657",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MS-TP-13-01",
      SLACcitation   = "%%CITATION = ARXIV:1302.1657;%%"
}

@article{Ibarra:2016dlb,
      author         = "Ibarra, Alejandro and Yaguna, Carlos E. and Zapata,
                        Oscar",
      title          = "{Direct detection of fermion dark matter in the radiative
                        seesaw model}",
      year           = "2016",
      eprint         = "1601.01163",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1601.01163;%%"
}

@article{Ade:2013zuv,
      author         = "Ade, P. A. R. and others",
      title          = "{Planck 2013 results. XVI. Cosmological parameters}",
      collaboration  = "Planck",
      journal        = "Astron. Astrophys.",
      volume         = "571",
      year           = "2014",
      pages          = "A16",
      doi            = "10.1051/0004-6361/201321591",
      eprint         = "1303.5076",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1303.5076;%%"
}

@article{Jungman:1995df,
      author         = "Jungman, Gerard and Kamionkowski, Marc and Griest, Kim",
      title          = "{Supersymmetric dark matter}",
      journal        = "Phys.Rept.",
      volume         = "267",
      pages          = "195-373",
      doi            = "10.1016/0370-1573(95)00058-5",
      year           = "1996",
      eprint         = "hep-ph/9506380",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SU-4240-605, UCSD-PTH-95-02, IASSNS-HEP-95-14, CU-TP-677",
      SLACcitation   = "%%CITATION = HEP-PH/9506380;%%",
}

@article{Ellis:2012aa,
      author         = "Ellis, John and Olive, Keith A.",
      title          = "{Revisiting the Higgs Mass and Dark Matter in the CMSSM}",
      journal        = "Eur.Phys.J.",
      volume         = "C72",
      pages          = "2005",
      doi            = "10.1140/epjc/s10052-012-2005-2",
      year           = "2012",
      eprint         = "1202.3262",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KCL-PH-TH-2012-08, LCTS-2012-04, CERN-PH-TH-2012-045,
                        UMN-TH-3034-12, FTPI-MINN-12-07",
      SLACcitation   = "%%CITATION = ARXIV:1202.3262;%%",
}

@article{Queiroz:2016zwd,
      author         = "Queiroz, Farinaldo S. and Yaguna, Carlos E. and Weniger,
                        Christoph",
      title          = "{Gamma-ray Limits on Neutrino Lines}",
      journal        = "JCAP",
      volume         = "1605",
      year           = "2016",
      number         = "05",
      pages          = "050",
      doi            = "10.1088/1475-7516/2016/05/050",
      eprint         = "1602.05966",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1602.05966;%%"
}

@article{Belanger:2006is,
      author         = "Belanger, G. and Boudjema, F. and Pukhov, A. and Semenov,
                        A.",
      title          = "{MicrOMEGAs 2.0: A Program to calculate the relic density
                        of dark matter in a generic model}",
      journal        = "Comput. Phys. Commun.",
      volume         = "176",
      year           = "2007",
      pages          = "367-382",
      doi            = "10.1016/j.cpc.2006.11.008",
      eprint         = "hep-ph/0607059",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-1152-06",
      SLACcitation   = "%%CITATION = HEP-PH/0607059;%%"
}

@article{Arcadi:2017vis,
      author         = "Arcadi, Giorgio and Queiroz, Farinaldo S. and Siqueira,
                        Clarissa",
      title          = "{The Semi-Hooperon: Gamma-ray and anti-proton excesses in
                        the Galactic Center}",
      year           = "2017",
      eprint         = "1706.02336",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1706.02336;%%"
}

@article{Balazs:2017hxh,
      author         = "Balázs, Csaba and Conrad, Jan and Farmer, Ben and
                        Jacques, Thomas and Li, Tong and Meyer, Manuel and
                        Queiroz, Farinaldo S. and Sánchez-Conde, Migual A.",
      title          = "{Sensitivity of the Cherenkov Telescope Array to the
                        Detection of a Dark Matter Signal in comparison to Direct
                        Detection and Collider Experiments}",
      year           = "2017",
      eprint         = "1706.01505",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1706.01505;%%"
}
@article{Campos:2017odj,
      author         = "Campos, Miguel D. and Queiroz, Farinaldo S. and Yaguna,
                        Carlos E. and Weniger, Christoph",
      title          = "{Search for right-handed neutrinos from dark matter
                        annihilation with gamma-rays}",
      year           = "2017",
      eprint         = "1702.06145",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1702.06145;%%"
}

@article{Aartsen:2017ulx,
      author         = "Aartsen, M. G. and others",
      title          = "{Search for Neutrinos from Dark Matter Self-Annihilations
                        in the center of the Milky Way with 3 years of
                        IceCube/DeepCore}",
      collaboration  = "IceCube",
      year           = "2017",
      eprint         = "1705.08103",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1705.08103;%%"
}

@article{Choi:2015ara,
      author         = "Choi, K. and others",
      title          = "{Search for neutrinos from annihilation of captured
                        low-mass dark matter particles in the Sun by
                        Super-Kamiokande}",
      collaboration  = "Super-Kamiokande",
      journal        = "Phys. Rev. Lett.",
      volume         = "114",
      year           = "2015",
      number         = "14",
      pages          = "141301",
      doi            = "10.1103/PhysRevLett.114.141301",
      eprint         = "1503.04858",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1503.04858;%%"
}

@article{Hehn:2016nll,
      author         = "Hehn, L. and others",
      title          = "{Improved EDELWEISS-III sensitivity for low-mass WIMPs
                        using a profile likelihood approach}",
      collaboration  = "EDELWEISS",
      journal        = "Eur. Phys. J.",
      volume         = "C76",
      year           = "2016",
      number         = "10",
      pages          = "548",
      doi            = "10.1140/epjc/s10052-016-4388-y",
      eprint         = "1607.03367",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1607.03367;%%"
}

@article{Amole:2016pye,
      author         = "Amole, C. and others",
      title          = "{Improved dark matter search results from PICO-2L Run 2}",
      collaboration  = "PICO",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "6",
      pages          = "061101",
      doi            = "10.1103/PhysRevD.93.061101",
      eprint         = "1601.03729",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "FERMILAB-PUB-16-028-AE-E-PPD",
      SLACcitation   = "%%CITATION = ARXIV:1601.03729;%%"
}

@article{Agnese:2015nto,
      author         = "Agnese, R. and others",
      title          = "{New Results from the Search for Low-Mass Weakly
                        Interacting Massive Particles with the CDMS Low Ionization
                        Threshold Experiment}",
      collaboration  = "SuperCDMS",
      journal        = "Phys. Rev. Lett.",
      volume         = "116",
      year           = "2016",
      number         = "7",
      pages          = "071301",
      doi            = "10.1103/PhysRevLett.116.071301",
      eprint         = "1509.02448",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "IPPP-15-56, DCTP-15-112, FERMILAB-PUB-15-394-AE",
      SLACcitation   = "%%CITATION = ARXIV:1509.02448;%%"
}

@article{Sirunyan:2017onm,
      author         = "Sirunyan, Albert M and others",
      title          = "{Search for dark matter and unparticles in events with a
                        Z boson and missing transverse momentum in proton-proton
                        collisions at sqrt(s) = 13 TeV}",
      collaboration  = "CMS",
      journal        = "JHEP",
      volume         = "03",
      year           = "2017",
      pages          = "061",
      doi            = "10.1007/JHEP03(2017)061",
      eprint         = "1701.02042",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-EXO-16-010, CERN-EP-2016-309,
                        FERMILAB-PUB-17-011-CMS",
      SLACcitation   = "%%CITATION = ARXIV:1701.02042;%%"
}

@article{Aaboud:2017dor,
      author         = "Aaboud, Morad and others",
      title          = "{Search for dark matter at $\sqrt{s}=13$ TeV in final
                        states containing an energetic photon and large missing
                        transverse momentum with the ATLAS detector}",
      collaboration  = "ATLAS",
      year           = "2017",
      eprint         = "1704.03848",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-EP-2017-044",
      SLACcitation   = "%%CITATION = ARXIV:1704.03848;%%"
}



@article{Abdallah:2016ygi,
      author         = "Abdallah, H. and others",
      title          = "{Search for dark matter annihilations towards the inner
                        Galactic halo from 10 years of observations with H.E.S.S}",
      collaboration  = "H.E.S.S.",
      journal        = "Phys. Rev. Lett.",
      volume         = "117",
      year           = "2016",
      number         = "11",
      pages          = "111301",
      doi            = "10.1103/PhysRevLett.117.111301",
      eprint         = "1607.08142",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1607.08142;%%"
}

@article{Archambault:2017wyh,
      author         = "Archambault, S. and others",
      title          = "{Dark Matter Constraints from a Joint Analysis of Dwarf
                        Spheroidal Galaxy Observations with VERITAS}",
      collaboration  = "VERITAS",
      journal        = "Phys. Rev.",
      volume         = "D95",
      year           = "2017",
      number         = "8",
      pages          = "082001",
      doi            = "10.1103/PhysRevD.95.082001",
      eprint         = "1703.04937",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1703.04937;%%"
}

@article{Ahnen:2016qkx,
      author         = "Ahnen, M. L. and others",
      title          = "{Limits to dark matter annihilation cross-section from a
                        combined analysis of MAGIC and Fermi-LAT observations of
                        dwarf satellite galaxies}",
      collaboration  = "Fermi-LAT, MAGIC",
      journal        = "JCAP",
      volume         = "1602",
      year           = "2016",
      number         = "02",
      pages          = "039",
      doi            = "10.1088/1475-7516/2016/02/039",
      eprint         = "1601.06590",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "FERMILAB-PUB-16-283-AE",
      SLACcitation   = "%%CITATION = ARXIV:1601.06590;%%"
}

@article{TheFermi-LAT:2017vmf,
      author         = "Ackermann, M. and others",
      title          = "{The Fermi Galactic Center GeV Excess and Implications
                        for Dark Matter}",
      collaboration  = "Fermi-LAT",
      journal        = "Astrophys. J.",
      volume         = "840",
      year           = "2017",
      number         = "1",
      pages          = "43",
      doi            = "10.3847/1538-4357/aa6cab",
      eprint         = "1704.03910",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1704.03910;%%"
}

@inproceedings{Hooper:2009zm,
      author         = "Hooper, Dan",
      title          = "{Particle Dark Matter}",
      booktitle      = "{Proceedings of Theoretical Advanced Study Institute in
                        Elementary Particle Physics on The dawn of the LHC era
                        (TASI 2008): Boulder, USA, June 2-27, 2008}",
      year           = "2010",
      url            = "http://lss.fnal.gov/cgi-bin/find_paper.pl?conf-09-025",
      pages          = "709-764",
      doi            = "10.1142/9789812838360_0014",
      eprint         = "0901.4090",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-CONF-09-025-A",
      SLACcitation   = "%%CITATION = ARXIV:0901.4090;%%"
}

@inproceedings{Olive:2003iq,
      author         = "Olive, Keith A.",
      title          = "{TASI lectures on dark matter}",
      booktitle      = "{Particle physics and cosmology: The quest for physics
                        beyond the standard model(s). Proceedings, Theoretical
                        Advanced Study Institute, TASI 2002, Boulder, USA, June
                        3-28, 2002}",
      year           = "2003",
      pages          = "797-851",
      eprint         = "astro-ph/0301505",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "UMN-TH-2127-03, TPI-MINN-03-02",
      SLACcitation   = "%%CITATION = ASTRO-PH/0301505;%%"
}

@article{Ellis:2010kf,
      author         = "Ellis, John and Olive, Keith A.",
      title          = "{Supersymmetric Dark Matter Candidates}",
      year           = "2010",
      eprint         = "1001.3651",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "CERN-PH-TH-2010-004, UMN-TH-2831-10, FTPI-MINN-10-02",
      SLACcitation   = "%%CITATION = ARXIV:1001.3651;%%",
}
@article{Bailly:2009pe,
      author         = "Bailly, Sean and Choi, Ki-Young and Jedamzik, Karsten and
                        Roszkowski, Leszek",
      title          = "{A Re-analysis of Gravitino Dark Matter in the
                        Constrained MSSM}",
      journal        = "JHEP",
      volume         = "0905",
      pages          = "103",
      doi            = "10.1088/1126-6708/2009/05/103",
      year           = "2009",
      eprint         = "0903.3974",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FGUAM-09-3, IFT-UAM-CSIC-09-15",
      SLACcitation   = "%%CITATION = ARXIV:0903.3974;%%",
}
@article{Buchmuller:2007ui,
      author         = "Buchmuller, Wilfried and Covi, Laura and Hamaguchi,
                        Koichi and Ibarra, Alejandro and Yanagida, Tsutomu",
      title          = "{Gravitino Dark Matter in R-Parity Breaking Vacua}",
      journal        = "JHEP",
      volume         = "0703",
      pages          = "037",
      doi            = "10.1088/1126-6708/2007/03/037",
      year           = "2007",
      eprint         = "hep-ph/0702184",
      archivePrefix  = "arXiv",
      primaryClass   = "HEP-PH",
      reportNumber   = "DESY-06-244, UT-07-03",
      SLACcitation   = "%%CITATION = HEP-PH/0702184;%%",
}
@article{McDonald:1993ex,
      author         = "McDonald, John",
      title          = "{Gauge singlet scalars as cold dark matter}",
      journal        = "Phys.Rev.",
      volume         = "D50",
      pages          = "3637-3649",
      doi            = "10.1103/PhysRevD.50.3637",
      year           = "1994",
      eprint         = "hep-ph/0702143",
      archivePrefix  = "arXiv",
      primaryClass   = "HEP-PH",
      reportNumber   = "IFM-13-93",
      SLACcitation   = "%%CITATION = HEP-PH/0702143;%%",
}

@article{Burgess:2000yq,
      author         = "Burgess, C.P. and Pospelov, Maxim and ter Veldhuis,
                        Tonnis",
      title          = "{The Minimal model of nonbaryonic dark matter: A Singlet
                        scalar}",
      journal        = "Nucl.Phys.",
      volume         = "B619",
      pages          = "709-728",
      doi            = "10.1016/S0550-3213(01)00513-2",
      year           = "2001",
      eprint         = "hep-ph/0011335",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TPI-MINN-00-46, UMN-TH-1922-00, MCGILL-00-31,
                        IASSNS-HEP-00-83",
      SLACcitation   = "%%CITATION = HEP-PH/0011335;%%",
}

@article{Yaguna:2008hd,
      author         = "Yaguna, Carlos E.",
      title          = "{Gamma rays from the annihilation of singlet scalar dark
                        matter}",
      journal        = "JCAP",
      volume         = "0903",
      pages          = "003",
      doi            = "10.1088/1475-7516/2009/03/003",
      year           = "2009",
      eprint         = "0810.4267",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0810.4267;%%",
}
@article{Goudelis:2009zz,
      author         = "Goudelis, A. and Mambrini, Y. and Yaguna, C.",
      title          = "{Antimatter signals of singlet scalar dark matter}",
      journal        = "JCAP",
      volume         = "0912",
      pages          = "008",
      doi            = "10.1088/1475-7516/2009/12/008",
      year           = "2009",
      eprint         = "0909.2799",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LPT-ORSAY-09-71, FTUAM-09-20, IFT-UAM-CSIC-09-42",
      SLACcitation   = "%%CITATION = ARXIV:0909.2799;%%",
}

@article{Cirelli:2005uq,
      author         = "Cirelli, Marco and Fornengo, Nicolao and Strumia,
                        Alessandro",
      title          = "{Minimal dark matter}",
      journal        = "Nucl.Phys.",
      volume         = "B753",
      pages          = "178-194",
      doi            = "10.1016/j.nuclphysb.2006.07.012",
      year           = "2006",
      eprint         = "hep-ph/0512090",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DFTT40-2005, IFUP-TH-2005-34",
      SLACcitation   = "%%CITATION = HEP-PH/0512090;%%",
}

@article{Ma:2008cu,
      author         = "Ma, Ernest and Suematsu, Daijiro",
      title          = "{Fermion Triplet Dark Matter and Radiative Neutrino
                        Mass}",
      journal        = "Mod.Phys.Lett.",
      volume         = "A24",
      pages          = "583-589",
      doi            = "10.1142/S021773230903059X",
      year           = "2009",
      eprint         = "0809.0942",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T454, KANAZAWA-08-07",
      SLACcitation   = "%%CITATION = ARXIV:0809.0942;%%",
}

@article{Belanger:2012zr,
      author         = "Belanger, Genevieve and Kannike, Kristjan and Pukhov,
                        Alexander and Raidal, Martti",
      title          = "{$Z_3$ Scalar Singlet Dark Matter}",
      journal        = "JCAP",
      volume         = "1301",
      pages          = "022",
      doi            = "10.1088/1475-7516/2013/01/022",
      year           = "2013",
      eprint         = "1211.1014",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-049-12",
      SLACcitation   = "%%CITATION = ARXIV:1211.1014;%%",
}

@article{Klasen:2013jpa,
      author         = "Klasen, Michael and Yaguna, Carlos E. and Ruiz-Alvarez,
                        Jose D. and Restrepo, Diego and Zapata, Oscar",
      title          = "{Scalar dark matter and fermion coannihilations in the
                        radiative seesaw model}",
      year           = "2013",
      eprint         = "1302.5298",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MS-TP-13-03",
      SLACcitation   = "%%CITATION = ARXIV:1302.5298;%%",
}

@article{Restrepo:2013aga,
      author         = "Restrepo, Diego and Zapata, Oscar and Yaguna, Carlos E.",
      title          = "{Models with radiative neutrino masses and viable dark
                        matter candidates}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2013",
      pages          = "011",
      doi            = "10.1007/JHEP11(2013)011",
      eprint         = "1308.3655",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1308.3655;%%"
}

@article{Fraser:2014yha,
      author         = "Fraser, Sean and Ma, Ernest and Popov, Oleg",
      title          = "{Scotogenic Inverse Seesaw Model of Neutrino Mass}",
      journal        = "Phys. Lett.",
      volume         = "B737",
      year           = "2014",
      pages          = "280-282",
      doi            = "10.1016/j.physletb.2014.08.069",
      eprint         = "1408.4785",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T543-(AUG-2014)",
      SLACcitation   = "%%CITATION = ARXIV:1408.4785;%%"
}

@article{Agashe:2014kda,
      author         = "Olive, K. A. and others",
      title          = "{Review of Particle Physics}",
      collaboration  = "Particle Data Group",
      journal        = "Chin. Phys.",
      volume         = "C38",
      year           = "2014",
      pages          = "090001",
      doi            = "10.1088/1674-1137/38/9/090001",
      SLACcitation   = "%%CITATION = CHPHD,C38,090001;%%"
}



@article{Restrepo:2015ura,
      author         = "Restrepo, Diego and Rivera, Andrés and Sánchez-Peláez,
                        Marta and Zapata, Oscar and Tangarife, Walter",
      title          = "{Radiative Neutrino Masses in the Singlet-Doublet Fermion
                        Dark Matter Model with Scalar Singlets}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "1",
      pages          = "013005",
      doi            = "10.1103/PhysRevD.92.013005",
      eprint         = "1504.07892",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TAUP2993-15",
      SLACcitation   = "%%CITATION = ARXIV:1504.07892;%%"
}

@article{Saab:2012th,
      author         = "Saab, Tarek",
      title          = "{An Introduction to Dark Matter Direct Detection Searches
                        &amp; Techniques}",
      year           = "2012",
      eprint         = "1203.2566",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1203.2566;%%",
}

@article{Salati:2010rc,
      author         = "Salati, P. and Donato, F. and Fornengo, N.",
      title          = "{Indirect Dark Matter Detection with Cosmic Antimatter}",
      year           = "2010",
      eprint         = "1003.4124",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1003.4124;%%",
}

@article{Conrad:2011na,
      author         = "Conrad, Jan",
      title          = "{Indirect detection of Dark matter with gamma-rays -
                        status and perspectives}",
      journal        = "PoS",
      volume         = "IDM2010",
      pages          = "048",
      year           = "2011",
      eprint         = "1103.5638",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1103.5638;%%",
}

@article{Abbasi:2012ws,
      author         = "Abbasi, R. and others",
      title          = "{Search for Neutrinos from Annihilating Dark Matter in
                        the Direction of the Galactic Center with the 40-String
                        IceCube Neutrino Observatory}",
      collaboration  = "IceCube collaboration",
      year           = "2012",
      eprint         = "1210.3557",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1210.3557;%%",
}

@article{Aprile:2013doa,
      author         = "Aprile, E. and others",
      title          = "{Limits on spin-dependent WIMP-nucleon cross sections
                        from 225 live days of XENON100 data}",
      collaboration  = "XENON100 Collaboration",
      year           = "2013",
      eprint         = "1301.6620",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1301.6620;%%",
}
@article{Aprile:2012nq,
      author         = "Aprile, E. and others",
      title          = "{Dark Matter Results from 225 Live Days of XENON100
                        Data}",
      collaboration  = "XENON100 Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "109",
      pages          = "181301",
      doi            = "10.1103/PhysRevLett.109.181301",
      year           = "2012",
      eprint         = "1207.5988",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1207.5988;%%",
}
@article{Aprile:2011dd,
      author         = "Aprile, E. and others",
      title          = "{The XENON100 Dark Matter Experiment}",
      collaboration  = "XENON100 Collaboration",
      journal        = "Astropart.Phys.",
      volume         = "35",
      pages          = "573-590",
      doi            = "10.1016/j.astropartphys.2012.01.003",
      year           = "2012",
      eprint         = "1107.2155",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1107.2155;%%",
}

@article{Angloher:2014bua,
      author         = "Angloher, G. and others",
      title          = "{EURECA Conceptual Design Report}",
      collaboration  = "EURECA",
      journal        = "Phys. Dark Univ.",
      volume         = "3",
      year           = "2014",
      pages          = "41-74",
      doi            = "10.1016/j.dark.2014.03.004",
      SLACcitation   = "%%CITATION = INSPIRE-1320073;%%"
}

@article{Agnese:2014aze,
      author         = "Agnese, R. and others",
      title          = "{Search for Low-Mass Weakly Interacting Massive Particles
                        with SuperCDMS}",
      collaboration  = "SuperCDMS",
      journal        = "Phys. Rev. Lett.",
      volume         = "112",
      year           = "2014",
      number         = "24",
      pages          = "241302",
      doi            = "10.1103/PhysRevLett.112.241302",
      eprint         = "1402.7137",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "FERMILAB-PUB-14-042-AE",
      SLACcitation   = "%%CITATION = ARXIV:1402.7137;%%"
}


@article{Calvo:2015uln,
      author         = "Calvo, J. and others",
      title          = "{Status of ArDM-1t: First observations from operation
                        with a full ton-scale liquid argon target}",
      collaboration  = "ArDM",
      year           = "2015",
      eprint         = "1505.02443",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1505.02443;%%"
}

@article{Aalseth:2015mba,
      author         = "Aalseth, C. E. and others",
      title          = "{The DarkSide Multiton Detector for the Direct Dark
                        Matter Search}",
      journal        = "Adv. High Energy Phys.",
      volume         = "2015",
      year           = "2015",
      pages          = "541362",
      doi            = "10.1155/2015/541362",
      SLACcitation   = "%%CITATION = 00642,2015,541362;%%"
}

@article{Aprile:2017yea,
      author         = "Aprile, E. and others",
      title          = "{Search for Electronic Recoil Event Rate Modulation with
                        4 Years of XENON100 Data}",
      collaboration  = "XENON",
      journal        = "Phys. Rev. Lett.",
      volume         = "118",
      year           = "2017",
      number         = "10",
      pages          = "101101",
      doi            = "10.1103/PhysRevLett.118.101101",
      eprint         = "1701.00769",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1701.00769;%%"
}

@article{Agnes:2014bvk,
      author         = "Agnes, P. and others",
      title          = "{First Results from the DarkSide-50 Dark Matter
                        Experiment at Laboratori Nazionali del Gran Sasso}",
      collaboration  = "DarkSide",
      journal        = "Phys. Lett.",
      volume         = "B743",
      year           = "2015",
      pages          = "456-466",
      doi            = "10.1016/j.physletb.2015.03.012",
      eprint         = "1410.0653",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "FERMILAB-PUB-14-389-AE-E",
      SLACcitation   = "%%CITATION = ARXIV:1410.0653;%%"
}


@article{Aprile:2012zx,
      author         = "Aprile, Elena",
      title          = "{The XENON1T Dark Matter Search Experiment}",
      collaboration  = "XENON1T collaboration",
      year           = "2012",
      eprint         = "1206.6288",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1206.6288;%%",
}
@article{Persic:2013aoa,
      author         = "Persic, Massimo",
      title          = "{CTA: the future of ground-based gamma-ray astrophysics}",
      collaboration  = "Consortium for the CTA",
      year           = "2013",
      eprint         = "1303.2346",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1303.2346;%%",
}

@article{Goodman:2010ku,
      author         = "Goodman, Jessica and Ibe, Masahiro and Rajaraman, Arvind
                        and Shepherd, William and Tait, Tim M.P. and others",
      title          = "{Constraints on Dark Matter from Colliders}",
      journal        = "Phys.Rev.",
      volume         = "D82",
      pages          = "116010",
      doi            = "10.1103/PhysRevD.82.116010",
      year           = "2010",
      eprint         = "1008.1783",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCI-HEP-TR-2010-15",
      SLACcitation   = "%%CITATION = ARXIV:1008.1783;%%",
}
@article{Zhou:2013fla,
      author         = "Zhou, Ning and Berge, David and Whiteson, Daniel",
      title          = "{Mono-everything: combined limits on dark matter
                        production at colliders from multiple final states}",
      year           = "2013",
      eprint         = "1302.3619",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1302.3619;%%",
}

@article{Citron:2012fg,
      author         = "Citron, M. and Ellis, J. and Luo, F. and Marrouche, J.
                        and Olive, K.A. and others",
      title          = "{The End of the CMSSM Coannihilation Strip is Nigh}",
      doi            = "10.1103/PhysRevD.87.036012",
      year           = "2012",
      eprint         = "1212.2886",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KCL-PH-TH-2012-46, LCTS-2012-32, CERN-PH-TH-2012-331,
                        UMN-TH-3127-12, FTPI-MINN-12-38, --UMN--TH--3127-12,
                        FTPI--MINN--12-38",
      SLACcitation   = "%%CITATION = ARXIV:1212.2886;%%",
}
@article{Strege:2012bt,
      author         = "Strege, C. and Bertone, G. and Feroz, F. and Fornasa, M.
                        and de Austri, R. Ruiz and others",
      title          = "{Global Fits of the cMSSM and NUHM including the LHC
                        Higgs discovery and new XENON100 constraints}",
      journal        = "JCAP",
      volume         = "1304",
      pages          = "013",
      doi            = "10.1088/1475-7516/2013/04/013",
      year           = "2013",
      eprint         = "1212.2636",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1212.2636;%%",
}

@article{Farina:2011bh,
      author         = "Farina, Marco and Kadastik, Mario and Pappadopulo, Duccio
                        and Pata, Joosep and Raidal, Martti and others",
      title          = "{Implications of XENON100 and LHC results for Dark Matter
                        models}",
      journal        = "Nucl.Phys.",
      volume         = "B853",
      pages          = "607-624",
      doi            = "10.1016/j.nuclphysb.2011.08.003",
      year           = "2011",
      eprint         = "1104.3572",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1104.3572;%%",
}


@article{Sierra:2008wj,
      author         = "Aristizabal Sierra, D. and Kubo, Jisuke and Restrepo, D.
                        and Suematsu, Daijiro and Zapata, Oscar",
      title          = "{Radiative seesaw: Warm dark matter, collider and lepton
                        flavour violating signals}",
      journal        = "Phys.Rev.",
      volume         = "D79",
      pages          = "013011",
      doi            = "10.1103/PhysRevD.79.013011",
      year           = "2009",
      eprint         = "0808.3340",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KANAZAWA-08-08",
      SLACcitation   = "%%CITATION = ARXIV:0808.3340;%%",
}

@article{Bonnet:2012kz,
      author         = "Bonnet, Florian and Hirsch, Martin and Ota, Toshihiko and
                        Winter, Walter",
      title          = "{Systematic study of the d=5 Weinberg operator at
                        one-loop order}",
      journal        = "JHEP",
      volume         = "1207",
      pages          = "153",
      doi            = "10.1007/JHEP07(2012)153",
      year           = "2012",
      eprint         = "1204.5862",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-12-26, MPP-2012-76",
      SLACcitation   = "%%CITATION = ARXIV:1204.5862;%%",
}
@article{Kim:2008pp,
      author         = "Kim, Yeong Gyun and Lee, Kang Young and Shin, Seodong",
      title          = "{Singlet fermionic dark matter}",
      journal        = "JHEP",
      volume         = "0805",
      pages          = "100",
      doi            = "10.1088/1126-6708/2008/05/100",
      year           = "2008",
      eprint         = "0803.2932",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0803.2932;%%",
}

@article{Baek:2011aa,
      author         = "Baek, Seungwon and Ko, P. and Park, Wan-Il",
      title          = "{Search for the Higgs portal to a singlet fermionic dark
                        matter at the LHC}",
      journal        = "JHEP",
      volume         = "1202",
      pages          = "047",
      doi            = "10.1007/JHEP02(2012)047",
      year           = "2012",
      eprint         = "1112.1847",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1112.1847;%%",
}


@article{LopezHonorez:2012kv,
      author         = "Lopez-Honorez, Laura and Schwetz, Thomas and Zupan, Jure",
      title          = "{Higgs portal, fermionic dark matter, and a Standard
                        Model like Higgs at 125 GeV}",
      journal        = "Phys.Lett.",
      volume         = "B716",
      pages          = "179-185",
      doi            = "10.1016/j.physletb.2012.07.017",
      year           = "2012",
      eprint         = "1203.2064",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCHEP-12-01",
      SLACcitation   = "%%CITATION = ARXIV:1203.2064;%%",
}

@article{Baek:2012uj,
      author         = "Baek, Seungwon and Ko, P. and Park, Wan-Il and Senaha,
                        Eibun",
      title          = "{Vacuum structure and stability of a singlet fermion dark
                        matter model with a singlet scalar messenger}",
      journal        = "JHEP",
      volume         = "1211",
      pages          = "116",
      doi            = "10.1007/JHEP11(2012)116",
      year           = "2012",
      eprint         = "1209.4163",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KIAS-P12061",
      SLACcitation   = "%%CITATION = ARXIV:1209.4163;%%",
}

@article{Fairbairn:2013uta,
      author         = "Fairbairn, Malcolm and Hogan, Robert",
      title          = "{Singlet Fermionic Dark Matter and the Electroweak Phase
                        Transition}",
      year           = "2013",
      eprint         = "1305.3452",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1305.3452;%%",
}

@article{Aad:2012tfa,
      author         = "Aad, Georges and others",
      title          = "{Observation of a new particle in the search for the
                        Standard Model Higgs boson with the ATLAS detector at the
                        LHC}",
      collaboration  = "ATLAS Collaboration",
      journal        = "Phys.Lett.",
      volume         = "B716",
      pages          = "1-29",
      doi            = "10.1016/j.physletb.2012.08.020",
      year           = "2012",
      eprint         = "1207.7214",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-PH-EP-2012-218",
      SLACcitation   = "%%CITATION = ARXIV:1207.7214;%%",
}

@article{Chatrchyan:2012ufa,
      author         = "Chatrchyan, Serguei and others",
      title          = "{Observation of a new boson at a mass of 125 GeV with the
                        CMS experiment at the LHC}",
      collaboration  = "CMS Collaboration",
      journal        = "Phys.Lett.",
      volume         = "B716",
      pages          = "30-61",
      doi            = "10.1016/j.physletb.2012.08.021",
      year           = "2012",
      eprint         = "1207.7235",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-HIG-12-028, CERN-PH-EP-2012-220",
      SLACcitation   = "%%CITATION = ARXIV:1207.7235;%%",
}

@article{Espinosa:2012ir,
      author         = "Espinosa, J.R. and Grojean, C. and Muhlleitner, M. and
                        Trott, M.",
      title          = "{Fingerprinting Higgs Suspects at the LHC}",
      journal        = "JHEP",
      volume         = "1205",
      pages          = "097",
      doi            = "10.1007/JHEP05(2012)097",
      year           = "2012",
      eprint         = "1202.3697",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1202.3697;%%",
}

@article{CMS:yva,
      key            = "1230214",
      title          = "{Combination of standard model Higgs boson searches and
                        measurements of the properties of the new boson with a
                        mass near 125 GeV}",
      collaboration  = "CMS Collaboration",
      year           = "2013",
      eprint   	     = "CMS-PAS-HIG-13-005",
      SLACcitation   = "%%CITATION = CMS-PAS-HIG-13-005 ETC.;%%",
}

@article{ATLAS:2013sla,
      key            = "1229948",
      title          = "{Combined coupling measurements of the Higgs-like boson
                        with the ATLAS detector using up to 25 fb$^{-1}$ of
                        proton-proton collision data}",
      collaboration  = "ATLAS Collaboration",
      year           = "2013",
      eprint         = "ATLAS-CONF-2013-034, ATLAS-COM-CONF-2013-035",
      SLACcitation   = "%%CITATION = ATLAS-CONF-2013-034 ETC.;%%",
}

@article{Ellis:2013lra,
      author         = "Ellis, John and You, Tevong",
      title          = "{Updated Global Analysis of Higgs Couplings}",
      journal        = "JHEP",
      volume         = "1306",
      pages          = "103",
      doi            = "10.1007/JHEP06(2013)103",
      year           = "2013",
      eprint         = "1303.3879",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KCL-PH-TH-2013-10, LCTS-2013-05, CERN-PH-TH-2013-050",
      SLACcitation   = "%%CITATION = ARXIV:1303.3879;%%",
}

@article{Patt:2006fw,
      author         = "Patt, Brian and Wilczek, Frank",
      title          = "{Higgs-field portal into hidden sectors}",
      year           = "2006",
      eprint         = "hep-ph/0605188",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MIT-CTP-3745",
      SLACcitation   = "%%CITATION = HEP-PH/0605188;%%",
}

@article{Kim:2006af,
      author         = "Kim, Yeong Gyun and Lee, Kang Young",
      title          = "{The Minimal model of fermionic dark matter}",
      journal        = "Phys.Rev.",
      volume         = "D75",
      pages          = "115012",
      doi            = "10.1103/PhysRevD.75.115012",
      year           = "2007",
      eprint         = "hep-ph/0611069",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KAIST-TH-2006-04",
      SLACcitation   = "%%CITATION = HEP-PH/0611069;%%",
}

@article{Abazajian:2006yn,
      author         = "Abazajian, Kevork and Koushiappas, Savvas M.",
      title          = "{Constraints on Sterile Neutrino Dark Matter}",
      journal        = "Phys.Rev.",
      volume         = "D74",
      pages          = "023527",
      doi            = "10.1103/PhysRevD.74.023527",
      year           = "2006",
      eprint         = "astro-ph/0605271",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "LA-UR-06-2765",
      SLACcitation   = "%%CITATION = ASTRO-PH/0605271;%%",
}


@article{Djouadi:2011aa,
      author         = "Djouadi, Abdelhak and Lebedev, Oleg and Mambrini, Yann
                        and Quevillon, Jeremie",
      title          = "{Implications of LHC searches for Higgs--portal dark
                        matter}",
      journal        = "Phys.Lett.",
      volume         = "B709",
      pages          = "65-69",
      doi            = "10.1016/j.physletb.2012.01.062",
      year           = "2012",
      eprint         = "1112.3299",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-11-240, LPT-ORSAY-11-117",
      SLACcitation   = "%%CITATION = ARXIV:1112.3299;%%",
}

@article{Kanemura:2010sh,
      author         = "Kanemura, Shinya and Matsumoto, Shigeki and Nabeshima,
                        Takehiro and Okada, Nobuchika",
      title          = "{Can WIMP Dark Matter overcome the Nightmare Scenario?}",
      journal        = "Phys.Rev.",
      volume         = "D82",
      pages          = "055026",
      doi            = "10.1103/PhysRevD.82.055026",
      year           = "2010",
      eprint         = "1005.5651",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UT-HET-039",
      SLACcitation   = "%%CITATION = ARXIV:1005.5651;%%",
}
@article{Belanger:2013oya,
      author         = "Belanger, G. and Boudjema, F. and Pukhov, A. and Semenov,
                        A.",
      title          = "{micrOMEGAs_3: A program for calculating dark matter
                        observables}",
      journal        = "Comput. Phys. Commun.",
      volume         = "185",
      year           = "2014",
      pages          = "960-985",
      doi            = "10.1016/j.cpc.2013.10.016",
      eprint         = "1305.0237",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-023-13",
      SLACcitation   = "%%CITATION = ARXIV:1305.0237;%%"
}


@article{Ackermann:2011wa,
      author         = "Ackermann, M. and others",
      title          = "{Constraining Dark Matter Models from a Combined Analysis
                        of Milky Way Satellites with the Fermi Large Area
                        Telescope}",
      collaboration  = "Fermi-LAT collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "107",
      pages          = "241302",
      doi            = "10.1103/PhysRevLett.107.241302",
      year           = "2011",
      eprint         = "1108.3546",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "SLAC-PUB-15004",
      SLACcitation   = "%%CITATION = ARXIV:1108.3546;%%",
}


@article{Halzen:1900zz,
      author         = "Halzen, Francis and Hooper, Dan",
      title          = "{High-energy neutrinos from WIMP annihilations in the
                        Sun}",
      year           = "2010",
      SLACcitation   = "%%CITATION = INSPIRE-896183;%%",
}

@article{Halzen:2009vu,
      author         = "Halzen, Francis and Hooper, Dan",
      title          = "{The Indirect Search for Dark Matter with IceCube}",
      journal        = "New J.Phys.",
      volume         = "11",
      pages          = "105019",
      doi            = "10.1088/1367-2630/11/10/105019",
      year           = "2009",
      eprint         = "0910.4513",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "FERMILAB-PUB-09-032-A",
      SLACcitation   = "%%CITATION = ARXIV:0910.4513;%%",
}

@article{Aartsen:2012kia,
      author         = "Aartsen, M.G. and others",
      title          = "{Search for dark matter annihilations in the Sun with the
                        79-string IceCube detector}",
      collaboration  = "IceCube collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "110",
      pages          = "131302",
      doi            = "10.1103/PhysRevLett.110.131302",
      year           = "2013",
      eprint         = "1212.4097",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1212.4097;%%",
}
@article{Danninger,
      author         = "M. Danninger",
      title          = "{Thesis: A search for dark matter annihilations in the Sun with 
                        IceCube and related studies}",
      eprint        = "\texttt{http://icecube.wisc.edu/~mda65/talks/thesis.pdf}",
}

@article{IceCube:2011ab,
      author         = "Abbasi, R. and others",
      title          = "{IceCube - Astrophysics and Astroparticle Physics at the
                        South Pole}",
      collaboration  = "IceCube Collaboration",
      year           = "2011",
      eprint         = "1111.5188",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1111.5188;%%",
}

@article{DeYoung:2011ke,
      author         = "DeYoung, Tyce",
      title          = "{Particle Physics in Ice with IceCube DeepCore}",
      collaboration  = "IceCube Collaboration",
      journal        = "Nucl.Instrum.Meth.",
      volume         = "A692",
      pages          = "180-183",
      doi            = "10.1016/j.nima.2011.12.067",
      year           = "2012",
      eprint         = "1112.1053",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1112.1053;%%",
}

@article{Collaboration:2011ym,
      author         = "Abbasi, R. and others",
      title          = "{The Design and Performance of IceCube DeepCore}",
      collaboration  = "IceCube Collaboration",
      journal        = "Astropart.Phys.",
      volume         = "35",
      pages          = "615-624",
      doi            = "10.1016/j.astropartphys.2012.01.004",
      year           = "2012",
      eprint         = "1109.6096",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1109.6096;%%",
}

@article{Chatrchyan:2013yoa,
      author         = "Chatrchyan, Serguei and others",
      title          = "{Search for a standard-model-like Higgs boson with a mass
                        in the range 145 to 1000 GeV at the LHC}",
      collaboration  = "CMS Collaboration",
      journal        = "Eur.Phys.J.",
      volume         = "C73",
      pages          = "2469",
      doi            = "10.1140/epjc/s10052-013-2469-8",
      year           = "2013",
      eprint         = "1304.0213",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-HIG-12-034, CERN-PH-EP-2013-050",
      SLACcitation   = "%%CITATION = ARXIV:1304.0213;%%",
}

@article{Barger:2007im,
      author         = "Barger, Vernon and Langacker, Paul and McCaskey, Mathew
                        and Ramsey-Musolf, Michael J. and Shaughnessy, Gabe",
      title          = "{LHC Phenomenology of an Extended Standard Model with a
                        Real Scalar Singlet}",
      journal        = "Phys.Rev.",
      volume         = "D77",
      pages          = "035005",
      doi            = "10.1103/PhysRevD.77.035005",
      year           = "2008",
      eprint         = "0706.4311",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MAD-PH-07-1492",
      SLACcitation   = "%%CITATION = ARXIV:0706.4311;%%",
}

@article{Pospelov:2011yp,
      author         = "Pospelov, Maxim and Ritz, Adam",
      title          = "{Higgs decays to dark matter: beyond the minimal model}",
      journal        = "Phys.Rev.",
      volume         = "D84",
      pages          = "113001",
      doi            = "10.1103/PhysRevD.84.113001",
      year           = "2011",
      eprint         = "1109.4872",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1109.4872;%%",
}
@article{Semenov:2010qt,
      author         = "Semenov, A.",
      title          = "{LanHEP - a package for automatic generation of Feynman
                        rules from the Lagrangian. Updated version 3.1}",
      year           = "2010",
      eprint         = "1005.1909",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1005.1909;%%",
}

@article{McDonald:2001vt,
      author         = "McDonald, John",
      title          = "{Thermally generated gauge singlet scalars as
                        selfinteracting dark matter}",
      journal        = "Phys.Rev.Lett.",
      volume         = "88",
      pages          = "091304",
      doi            = "10.1103/PhysRevLett.88.091304",
      year           = "2002",
      eprint         = "hep-ph/0106249",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0106249;%%",
}

@article{Yaguna:2011qn,
      author         = "Yaguna, Carlos E.",
      title          = "{The Singlet Scalar as FIMP Dark Matter}",
      journal        = "JHEP",
      volume         = "1108",
      pages          = "060",
      doi            = "10.1007/JHEP08(2011)060",
      year           = "2011",
      eprint         = "1105.1654",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1105.1654;%%",
}

@article{Yaguna:2011ei,
      author         = "Yaguna, Carlos E.",
      title          = "{An intermediate framework between WIMP, FIMP, and EWIP
                        dark matter}",
      journal        = "JCAP",
      volume         = "1202",
      pages          = "006",
      doi            = "10.1088/1475-7516/2012/02/006",
      year           = "2012",
      eprint         = "1111.6831",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MS-TP-11-22",
      SLACcitation   = "%%CITATION = ARXIV:1111.6831;%%",
}
@article{Esch:2013rta,
      author         = "Esch, Sonja and Klasen, Michael and Yaguna, Carlos E.",
      title          = "{Detection prospects of singlet fermionic dark matter}",
      year           = "2013",
      eprint         = "1308.0951",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MS-TP-13-20",
      SLACcitation   = "%%CITATION = ARXIV:1308.0951;%%",
}

@article{Merle:2013wta,
      author         = "Merle, Alexander and Niro, Viviana and Schmidt, Daniel",
      title          = "{New Production Mechanism for keV Sterile Neutrino Dark
                        Matter by Decays of Frozen-In Scalars}",
      journal        = "JCAP",
      volume         = "1403",
      pages          = "028",
      doi            = "10.1088/1475-7516/2014/03/028",
      year           = "2014",
      eprint         = "1306.3996",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1306.3996;%%",
}

@article{Griest:1989wd,
      author         = "Griest, Kim and Kamionkowski, Marc",
      title          = "{Unitarity Limits on the Mass and Radius of Dark Matter
                        Particles}",
      journal        = "Phys.Rev.Lett.",
      volume         = "64",
      pages          = "615",
      doi            = "10.1103/PhysRevLett.64.615",
      year           = "1990",
      reportNumber   = "CFPA-TH-89-013, FERMILAB-PUB-89-205-A",
      SLACcitation   = "%%CITATION = PRLTA,64,615;%%",
}
@article{Hall:2009bx,
      author         = "Hall, Lawrence J. and Jedamzik, Karsten and
                        March-Russell, John and West, Stephen M.",
      title          = "{Freeze-In Production of FIMP Dark Matter}",
      journal        = "JHEP",
      volume         = "1003",
      pages          = "080",
      doi            = "10.1007/JHEP03(2010)080",
      year           = "2010",
      eprint         = "0911.1120",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "OUTP-09-18-P, UCB-PTH-09-32",
      SLACcitation   = "%%CITATION = ARXIV:0911.1120;%%",
}
@article{Chu:2011be,
      author         = "Chu, Xiaoyong and Hambye, Thomas and Tytgat, Michel H.G.",
      title          = "{The Four Basic Ways of Creating Dark Matter Through a
                        Portal}",
      journal        = "JCAP",
      volume         = "1205",
      pages          = "034",
      doi            = "10.1088/1475-7516/2012/05/034",
      year           = "2012",
      eprint         = "1112.0493",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ULB-TH-11-26",
      SLACcitation   = "%%CITATION = ARXIV:1112.0493;%%",
}

@article{Cheung:2011nn,
      author         = "Cheung, Clifford and Elor, Gilly and Hall, Lawrence",
      title          = "{Gravitino Freeze-In}",
      journal        = "Phys.Rev.",
      volume         = "D84",
      pages          = "115021",
      doi            = "10.1103/PhysRevD.84.115021",
      year           = "2011",
      eprint         = "1103.4394",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1103.4394;%%",
}

@article{Asaka:2005cn,
      author         = "Asaka, Takehiko and Ishiwata, Koji and Moroi, Takeo",
      title          = "{Right-handed sneutrino as cold dark matter}",
      journal        = "Phys.Rev.",
      volume         = "D73",
      pages          = "051301",
      doi            = "10.1103/PhysRevD.73.051301",
      year           = "2006",
      eprint         = "hep-ph/0512118",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TU-760",
      SLACcitation   = "%%CITATION = HEP-PH/0512118;%%",
}

@article{Asaka:2006fs,
      author         = "Asaka, Takehiko and Ishiwata, Koji and Moroi, Takeo",
      title          = "{Right-handed sneutrino as cold dark matter of the
                        universe}",
      journal        = "Phys.Rev.",
      volume         = "D75",
      pages          = "065001",
      doi            = "10.1103/PhysRevD.75.065001",
      year           = "2007",
      eprint         = "hep-ph/0612211",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TU-781",
      SLACcitation   = "%%CITATION = HEP-PH/0612211;%%",
}

@article{Biermann:2013nxa,
      author         = "Biermann, P.L. and de Vega, H.J. and Sanchez, N.G.",
      title          = "{Towards the Chalonge Meudon Workshop 2013. Highlights
                        and Conclusions of the Chalonge Meudon workshop 2012: warm
                        dark matter galaxy formation in agreement with
                        observations}",
      year           = "2013",
      eprint         = "1305.7452",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1305.7452;%%",
}

@article{Viel:2013fqw,
      author         = "Viel, M. and Becker, G.D. and Bolton, J.S. and Haehnelt,
                        M.G.",
      title          = "{Warm Dark Matter as a solution to the small scale
                        crisis: new constraints from high redshift Lyman-alpha
                        forest data}",
      journal        = "Physical Review D, vol. 88, Issue 4, id.",
      volume         = "043502",
      year           = "2013",
      eprint         = "1306.2314",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1306.2314;%%",
}



@article{Canetti:2012kh,
      author         = "Canetti, Laurent and Drewes, Marco and Frossard, Tibor
                        and Shaposhnikov, Mikhail",
      title          = "{Dark Matter, Baryogenesis and Neutrino Oscillations from
                        Right Handed Neutrinos}",
      journal        = "Phys.Rev.",
      volume         = "D87",
      pages          = "093006",
      doi            = "10.1103/PhysRevD.87.093006",
      year           = "2013",
      eprint         = "1208.4607",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TTK-12-05, TUM-HEP-852-12, CAS-KITPC-ITP-368,
                        CAS-KITPC-ITP-368",
      SLACcitation   = "%%CITATION = ARXIV:1208.4607;%%",
}

@article{Lovell:2011rd,
      author         = "Lovell, Mark R. and Eke, Vincent and Frenk, Carlos S. and
                        Gao, Liang and Jenkins, Adrian and others",
      title          = "{The Haloes of Bright Satellite Galaxies in a Warm Dark
                        Matter Universe}",
      journal        = "Mon.Not.Roy.Astron.Soc.",
      volume         = "420",
      pages          = "2318-2324",
      doi            = "10.1111/j.1365-2966.2011.20200.x",
      year           = "2012",
      eprint         = "1104.2929",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1104.2929;%%",
}
@article{Ma:2012if,
      author         = "Ma, Ernest",
      title          = "{Radiative Scaling Neutrino Mass and Warm Dark Matter}",
      journal        = "Phys.Lett.",
      volume         = "B717",
      pages          = "235-237",
      doi            = "10.1016/j.physletb.2012.09.046",
      year           = "2012",
      eprint         = "1206.1812",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T522 (JUNE-2012), UCRHEP-T522-(JUNE-2012)",
      SLACcitation   = "%%CITATION = ARXIV:1206.1812;%%",
}

@article{Nemevsek:2012cd,
      author         = "Nemevsek, Miha and Senjanovic, Goran and Zhang, Yue",
      title          = "{Warm Dark Matter in Low Scale Left-Right Theory}",
      journal        = "JCAP",
      volume         = "1207",
      pages          = "006",
      doi            = "10.1088/1475-7516/2012/07/006",
      year           = "2012",
      eprint         = "1205.0844",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1205.0844;%%",
}

@article{King:2012wg,
      author         = "King, Stephen F. and Merle, Alexander",
      title          = "{Warm Dark Matter from keVins}",
      journal        = "JCAP",
      volume         = "1208",
      pages          = "016",
      doi            = "10.1088/1475-7516/2012/08/016",
      year           = "2012",
      eprint         = "1205.0551",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1205.0551;%%",
}

@article{Barry:2011fp,
      author         = "Barry, James and Rodejohann, Werner and Zhang, He",
      title          = "{Sterile Neutrinos for Warm Dark Matter and the Reactor
                        Anomaly in Flavor Symmetry Models}",
      journal        = "JCAP",
      volume         = "1201",
      pages          = "052",
      doi            = "10.1088/1475-7516/2012/01/052",
      year           = "2012",
      eprint         = "1110.6382",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1110.6382;%%",
}

@article{Feng:2003xh,
      author         = "Feng, Jonathan L. and Rajaraman, Arvind and Takayama,
                        Fumihiro",
      title          = "{Superweakly interacting massive particles}",
      journal        = "Phys.Rev.Lett.",
      volume         = "91",
      pages          = "011302",
      doi            = "10.1103/PhysRevLett.91.011302",
      year           = "2003",
      eprint         = "hep-ph/0302215",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCI-TR-2003-6",
      SLACcitation   = "%%CITATION = HEP-PH/0302215;%%",
}

@article{Choi:2005vq,
      author         = "Choi, Ki-Young and Roszkowski, Leszek",
      title          = "{E-WIMPs}",
      journal        = "AIP Conf.Proc.",
      volume         = "805",
      pages          = "30-36",
      doi            = "10.1063/1.2149672",
      year           = "2006",
      eprint         = "hep-ph/0511003",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0511003;%%",
}


@article{Hinshaw:2012aka,
      author         = "Hinshaw, G. and others",
      title          = "{Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP)
                        Observations: Cosmological Parameter Results}",
      collaboration  = "WMAP",
      journal        = "Astrophys. J. Suppl.",
      volume         = "208",
      year           = "2013",
      pages          = "19",
      doi            = "10.1088/0067-0049/208/2/19",
      eprint         = "1212.5226",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1212.5226;%%"
}


@article{Mambrini:2013iaa,
      author         = "Mambrini, Yann and Olive, Keith A. and Quevillon, Jeremie
                        and Zaldivar, Bryan",
      title          = "{Gauge Coupling Unification and Non-Equilibrium Thermal
                        Dark Matter}",
      journal        = "Phys.Rev.Lett.",
      volume         = "110",
      pages          = "241306",
      doi            = "10.1103/PhysRevLett.110.241306",
      year           = "2013",
      eprint         = "1302.4438",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1302.4438;%%",
}

@article{Canetti:2012vf,
      author         = "Canetti, Laurent and Drewes, Marco and Shaposhnikov,
                        Mikhail",
      title          = "{Sterile Neutrinos as the Origin of Dark and Baryonic
                        Matter}",
      journal        = "Phys.Rev.Lett.",
      number         = "6",
      volume         = "110",
      pages          = "061801",
      doi            = "10.1103/PhysRevLett.110.061801",
      year           = "2013",
      eprint         = "1204.3902",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TTK-12-08, CAS-KITPC-ITP-315",
      SLACcitation   = "%%CITATION = ARXIV:1204.3902;%%",
}
@article{Boyarsky:2009ix,
      author         = "Boyarsky, Alexey and Ruchayskiy, Oleg and Shaposhnikov,
                        Mikhail",
      title          = "{The Role of sterile neutrinos in cosmology and
                        astrophysics}",
      journal        = "Ann.Rev.Nucl.Part.Sci.",
      volume         = "59",
      pages          = "191-214",
      doi            = "10.1146/annurev.nucl.010909.083654",
      year           = "2009",
      eprint         = "0901.0011",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0901.0011;%%",
}

@article{Watson:2011dw,
      author         = "Watson, Casey R. and Li, Zhi-Yuan and Polley, Nicholas
                        K.",
      title          = "{Constraining Sterile Neutrino Warm Dark Matter with
                        Chandra Observations of the Andromeda Galaxy}",
      journal        = "JCAP",
      volume         = "1203",
      pages          = "018",
      doi            = "10.1088/1475-7516/2012/03/018",
      year           = "2012",
      eprint         = "1111.4217",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1111.4217;%%",
}
@article{Shaposhnikov:2006xi,
      author         = "Shaposhnikov, Mikhail and Tkachev, Igor",
      title          = "{The nuMSM, inflation, and dark matter}",
      journal        = "Phys.Lett.",
      volume         = "B639",
      pages          = "414-417",
      doi            = "10.1016/j.physletb.2006.06.063",
      year           = "2006",
      eprint         = "hep-ph/0604236",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2006-069",
      SLACcitation   = "%%CITATION = HEP-PH/0604236;%%",
}

@article{Kusenko:2006rh,
      author         = "Kusenko, Alexander",
      title          = "{Sterile neutrinos, dark matter, and the pulsar
                        velocities in models with a Higgs singlet}",
      journal        = "Phys.Rev.Lett.",
      volume         = "97",
      pages          = "241301",
      doi            = "10.1103/PhysRevLett.97.241301",
      year           = "2006",
      eprint         = "hep-ph/0609081",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCLA-06-TEP-23",
      SLACcitation   = "%%CITATION = HEP-PH/0609081;%%",
}


@article{Boyarsky:2007ge,
      author         = "Boyarsky, Alexey and Malyshev, Denys and Neronov, Andrey
                        and Ruchayskiy, Oleg",
      title          = "{Constraining DM properties with SPI}",
      journal        = "Mon.Not.Roy.Astron.Soc.",
      volume         = "387",
      pages          = "1345",
      doi            = "10.1111/j.1365-2966.2008.13003.x",
      year           = "2008",
      eprint         = "0710.4922",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ARXIV:0710.4922;%%",
}
@article{Yuksel:2007xh,
      author         = "Yuksel, Hasan and Beacom, John F. and Watson, Casey R.",
      title          = "{Strong Upper Limits on Sterile Neutrino Warm Dark
                        Matter}",
      journal        = "Phys.Rev.Lett.",
      volume         = "101",
      pages          = "121301",
      doi            = "10.1103/PhysRevLett.101.121301",
      year           = "2008",
      eprint         = "0706.4084",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ARXIV:0706.4084;%%",
}

@article{Loewenstein:2012px,
      author         = "Loewenstein, Michael and Kusenko, Alexander",
      title          = "{Dark Matter Search Using XMM-Newton Observations of
                        Willman 1}",
      journal        = "Astrophys.J.",
      volume         = "751",
      pages          = "82",
      doi            = "10.1088/0004-637X/751/2/82",
      year           = "2012",
      eprint         = "1203.5229",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "UCLA-12-TEP-00",
      SLACcitation   = "%%CITATION = ARXIV:1203.5229;%%",
}


@article{Dolgov:2000ew,
      author         = "Dolgov, A.D. and Hansen, S.H.",
      title          = "{Massive sterile neutrinos as warm dark matter}",
      journal        = "Astropart.Phys.",
      volume         = "16",
      pages          = "339-344",
      doi            = "10.1016/S0927-6505(01)00115-3",
      year           = "2002",
      eprint         = "hep-ph/0009083",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0009083;%%",
}

@article{Klasen:2013ypa,
      author         = "Klasen, Michael and Yaguna, Carlos E.",
      title          = "{Warm and cold fermionic dark matter via freeze-in}",
      journal        = "JCAP",
      volume         = "1311",
      pages          = "039",
      doi            = "10.1088/1475-7516/2013/11/039",
      year           = "2013",
      eprint         = "1309.2777",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MS-TP-13-24",
      SLACcitation   = "%%CITATION = ARXIV:1309.2777;%%",
}

@article{Teegarden:2006ni,
      author         = "Teegarden, B.J. and Watanabe, K.",
      title          = "{A Comprehensive Search for Gamma-Ray Lines in the First
                        Year of Data from the INTEGRAL Spectrometer}",
      journal        = "Astrophys.J.",
      volume         = "646",
      pages          = "965-981",
      doi            = "10.1086/504967",
      year           = "2006",
      eprint         = "astro-ph/0604277",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0604277;%%",
}

@article{Winkler:2003nn,
      author         = "Winkler, C. and Courvoisier, T.J.-L. and Di Cocco, G. and
                        Gehrels, N. and Gimenez, A. and others",
      title          = "{The INTEGRAL mission}",
      journal        = "Astron.Astrophys.",
      volume         = "411",
      pages          = "L1-L6",
      doi            = "10.1051/0004-6361:20031288",
      year           = "2003",
      SLACcitation   = "%%CITATION = AAEJA,411,L1;%%",
}

@article{Tremaine:1979we,
      author         = "Tremaine, S. and Gunn, J.E.",
      title          = "{Dynamical Role of Light Neutral Leptons in Cosmology}",
      journal        = "Phys.Rev.Lett.",
      volume         = "42",
      pages          = "407-410",
      doi            = "10.1103/PhysRevLett.42.407",
      year           = "1979",
      SLACcitation   = "%%CITATION = PRLTA,42,407;%%",
}

@article{Boyarsky:2008ju,
      author         = "Boyarsky, Alexey and Ruchayskiy, Oleg and Iakubovskyi,
                        Dmytro",
      title          = "{A Lower bound on the mass of Dark Matter particles}",
      journal        = "JCAP",
      volume         = "0903",
      pages          = "005",
      doi            = "10.1088/1475-7516/2009/03/005",
      year           = "2009",
      eprint         = "0808.3902",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0808.3902;%%",
}

@article{Gorbunov:2008ka,
      author         = "Gorbunov, D. and Khmelnitsky, A. and Rubakov, V.",
      title          = "{Constraining sterile neutrino dark matter by phase-space
                        density observations}",
      journal        = "JCAP",
      volume         = "0810",
      pages          = "041",
      doi            = "10.1088/1475-7516/2008/10/041",
      year           = "2008",
      eprint         = "0808.3910",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0808.3910;%%",
}

@article{Abazajian:2001vt,
      author         = "Abazajian, Kevork and Fuller, George M. and Tucker,
                        Wallace H.",
      title          = "{Direct detection of warm dark matter in the X-ray}",
      journal        = "Astrophys.J.",
      volume         = "562",
      pages          = "593-604",
      doi            = "10.1086/323867",
      year           = "2001",
      eprint         = "astro-ph/0106002",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0106002;%%",
}
@article{Boyarsky:2005us,
      author         = "Boyarsky, Alexey and Neronov, A. and Ruchayskiy, Oleg and
                        Shaposhnikov, M.",
      title          = "{Constraints on sterile neutrino as a dark matter
                        candidate from the diffuse x-ray background}",
      journal        = "Mon.Not.Roy.Astron.Soc.",
      volume         = "370",
      pages          = "213-218",
      doi            = "10.1111/j.1365-2966.2006.10458.x",
      year           = "2006",
      eprint         = "astro-ph/0512509",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0512509;%%",
}
@article{Boyarsky:2006zi,
      author         = "Boyarsky, Alexey and Neronov, A. and Ruchayskiy, Oleg and
                        Shaposhnikov, Mikhail",
      title          = "{Restrictions on parameters of sterile neutrino dark
                        matter from observations of galaxy clusters}",
      journal        = "Phys.Rev.",
      volume         = "D74",
      pages          = "103506",
      doi            = "10.1103/PhysRevD.74.103506",
      year           = "2006",
      eprint         = "astro-ph/0603368",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0603368;%%",
}

@article{Boyarsky:2006fg,
      author         = "Boyarsky, Alexey and Neronov, A. and Ruchayskiy, O. and
                        Shaposhnikov, M. and Tkachev, I.",
      title          = "{Where to find a dark matter sterile neutrino?}",
      journal        = "Phys.Rev.Lett.",
      volume         = "97",
      pages          = "261302",
      doi            = "10.1103/PhysRevLett.97.261302",
      year           = "2006",
      eprint         = "astro-ph/0603660",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0603660;%%",
}

@article{RiemerSorensen:2006fh,
      author         = "Riemer-Sorensen, Signe and Hansen, Steen H. and Pedersen,
                        Kristian",
      title          = "{Sterile neutrinos in the Milky Way: Observational
                        constraints}",
      journal        = "Astrophys.J.",
      volume         = "644",
      pages          = "L33-L36",
      doi            = "10.1086/505330",
      year           = "2006",
      eprint         = "astro-ph/0603661",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0603661;%%",
}
@article{Dodelson:1993je,
      author         = "Dodelson, Scott and Widrow, Lawrence M.",
      title          = "{Sterile-neutrinos as dark matter}",
      journal        = "Phys.Rev.Lett.",
      volume         = "72",
      pages          = "17-20",
      doi            = "10.1103/PhysRevLett.72.17",
      year           = "1994",
      eprint         = "hep-ph/9303287",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-93-057-A",
      SLACcitation   = "%%CITATION = HEP-PH/9303287;%%",
}

@article{Shi:1998km,
      author         = "Shi, Xiang-Dong and Fuller, George M.",
      title          = "{A New dark matter candidate: Nonthermal sterile
                        neutrinos}",
      journal        = "Phys.Rev.Lett.",
      volume         = "82",
      pages          = "2832-2835",
      doi            = "10.1103/PhysRevLett.82.2832",
      year           = "1999",
      eprint         = "astro-ph/9810076",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/9810076;%%",
}

@article{Asaka:2005an,
      author         = "Asaka, Takehiko and Blanchet, Steve and Shaposhnikov,
                        Mikhail",
      title          = "{The nuMSM, dark matter and neutrino masses}",
      journal        = "Phys.Lett.",
      volume         = "B631",
      pages          = "151-156",
      doi            = "10.1016/j.physletb.2005.09.070",
      year           = "2005",
      eprint         = "hep-ph/0503065",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0503065;%%",
}

@article{Barbieri:1989ti,
      author         = "Barbieri, Riccardo and Dolgov, A.",
      title          = "{Bounds on Sterile-neutrinos from Nucleosynthesis}",
      journal        = "Phys.Lett.",
      volume         = "B237",
      pages          = "440",
      doi            = "10.1016/0370-2693(90)91203-N",
      year           = "1990",
      reportNumber   = "IFUP-TH-59-89",
      SLACcitation   = "%%CITATION = PHLTA,B237,440;%%",
}

@article{Shaposhnikov:2008pf,
      author         = "Shaposhnikov, Mikhail",
      title          = "{The nuMSM, leptonic asymmetries, and properties of
                        singlet fermions}",
      journal        = "JHEP",
      volume         = "0808",
      pages          = "008",
      doi            = "10.1088/1126-6708/2008/08/008",
      year           = "2008",
      eprint         = "0804.4542",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0804.4542;%%",
}

@article{Laine:2008pg,
      author         = "Laine, M. and Shaposhnikov, M.",
      title          = "{Sterile neutrino dark matter as a consequence of
                        nuMSM-induced lepton asymmetry}",
      journal        = "JCAP",
      volume         = "0806",
      pages          = "031",
      doi            = "10.1088/1475-7516/2008/06/031",
      year           = "2008",
      eprint         = "0804.4543",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BI-TP-2008-02, NSF-KITP-08-39",
      SLACcitation   = "%%CITATION = ARXIV:0804.4543;%%",
}

@article{Abazajian:2012ys,
      author         = "Abazajian, K.N. and Acero, M.A. and Agarwalla, S.K. and
                        Aguilar-Arevalo, A.A. and Albright, C.H. and others",
      title          = "{Light Sterile Neutrinos: A White Paper}",
      year           = "2012",
      eprint         = "1204.5379",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-12-881-PPD",
      SLACcitation   = "%%CITATION = ARXIV:1204.5379;%%",
}

@article{Kusenko:2009up,
      author         = "Kusenko, Alexander",
      title          = "{Sterile neutrinos: The Dark side of the light fermions}",
      journal        = "Phys.Rept.",
      volume         = "481",
      pages          = "1-28",
      doi            = "10.1016/j.physrep.2009.07.004",
      year           = "2009",
      eprint         = "0906.2968",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCLA-09-TEP-55",
      SLACcitation   = "%%CITATION = ARXIV:0906.2968;%%",
}

@article{Abazajian:2001nj,
      author         = "Abazajian, Kevork and Fuller, George M. and Patel,
                        Mitesh",
      title          = "{Sterile neutrino hot, warm, and cold dark matter}",
      journal        = "Phys.Rev.",
      volume         = "D64",
      pages          = "023501",
      doi            = "10.1103/PhysRevD.64.023501",
      year           = "2001",
      eprint         = "astro-ph/0101524",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0101524;%%",
}
@article{Asaka:2006nq,
      author         = "Asaka, Takehiko and Laine, Mikko and Shaposhnikov,
                        Mikhail",
      title          = "{Lightest sterile neutrino abundance within the nuMSM}",
      journal        = "JHEP",
      volume         = "0701",
      pages          = "091",
      doi            = "10.1088/1126-6708/2007/01/091",
      year           = "2007",
      eprint         = "hep-ph/0612182",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BI-TP-2006-45",
      SLACcitation   = "%%CITATION = HEP-PH/0612182;%%",
}

@article{Boyarsky:2008mt,
      author         = "Boyarsky, Alexey and Lesgourgues, Julien and Ruchayskiy,
                        Oleg and Viel, Matteo",
      title          = "{Realistic sterile neutrino dark matter with keV mass
                        does not contradict cosmological bounds}",
      journal        = "Phys.Rev.Lett.",
      volume         = "102",
      pages          = "201304",
      doi            = "10.1103/PhysRevLett.102.201304",
      year           = "2009",
      eprint         = "0812.3256",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2008-234, LAPTH-1290-08",
      SLACcitation   = "%%CITATION = ARXIV:0812.3256;%%",
}

@article{Bezrukov:2009th,
      author         = "Bezrukov, F. and Hettmansperger, H. and Lindner, M.",
      title          = "{keV sterile neutrino Dark Matter in gauge extensions of
                        the Standard Model}",
      journal        = "Phys.Rev.",
      volume         = "D81",
      pages          = "085032",
      doi            = "10.1103/PhysRevD.81.085032",
      year           = "2010",
      eprint         = "0912.4415",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0912.4415;%%",
}

@article{Abazajian:2005xn,
      author         = "Abazajian, Kevork",
      title          = "{Linear cosmological structure limits on warm dark
                        matter}",
      journal        = "Phys.Rev.",
      volume         = "D73",
      pages          = "063513",
      doi            = "10.1103/PhysRevD.73.063513",
      year           = "2006",
      eprint         = "astro-ph/0512631",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "LA-UR-05-9175",
      SLACcitation   = "%%CITATION = ASTRO-PH/0512631;%%",
}
@article{Viel:2006kd,
      author         = "Viel, Matteo and Lesgourgues, Julien and Haehnelt, Martin
                        G. and Matarrese, Sabino and Riotto, Antonio",
      title          = "{Can sterile neutrinos be ruled out as warm dark matter
                        candidates?}",
      journal        = "Phys.Rev.Lett.",
      volume         = "97",
      pages          = "071301",
      doi            = "10.1103/PhysRevLett.97.071301",
      year           = "2006",
      eprint         = "astro-ph/0605706",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0605706;%%",
}

@article{Seljak:2006qw,
      author         = "Seljak, Uros and Makarov, Alexey and McDonald, Patrick
                        and Trac, Hy",
      title          = "{Can sterile neutrinos be the dark matter?}",
      journal        = "Phys.Rev.Lett.",
      volume         = "97",
      pages          = "191303",
      doi            = "10.1103/PhysRevLett.97.191303",
      year           = "2006",
      eprint         = "astro-ph/0602430",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ASTRO-PH/0602430;%%",
}
@article{Boyarsky:2008xj,
      author         = "Boyarsky, Alexey and Lesgourgues, Julien and Ruchayskiy,
                        Oleg and Viel, Matteo",
      title          = "{Lyman-alpha constraints on warm and on warm-plus-cold
                        dark matter models}",
      journal        = "JCAP",
      volume         = "0905",
      pages          = "012",
      doi            = "10.1088/1475-7516/2009/05/012",
      year           = "2009",
      eprint         = "0812.0010",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "CERN-PH-TH-2008-234, LAPTH-1290-08",
      SLACcitation   = "%%CITATION = ARXIV:0812.0010;%%",
}


@article{Horiuchi:2013noa,
      author         = "Horiuchi, Shunsaku and Humphrey, Philip J. and Onorbe,
                        Jose and Abazajian, Kevork N. and Kaplinghat, Manoj and
                        others",
      title          = "{Sterile neutrino dark matter bounds from galaxies of the
                        Local Group}",
      journal        = "Phys.Rev.",
      volume         = "D89",
      pages          = "025017",
      doi            = "10.1103/PhysRevD.89.025017",
      year           = "2014",
      eprint         = "1311.0282",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1311.0282;%%",
}

@article{Viel:2005qj,
      author         = "Viel, Matteo and Lesgourgues, Julien and Haehnelt, Martin
                        G. and Matarrese, Sabino and Riotto, Antonio",
      title          = "{Constraining warm dark matter candidates including
                        sterile neutrinos and light gravitinos with WMAP and the
                        Lyman-alpha forest}",
      journal        = "Phys.Rev.",
      volume         = "D71",
      pages          = "063534",
      doi            = "10.1103/PhysRevD.71.063534",
      year           = "2005",
      eprint         = "astro-ph/0501562",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "DFPD-05-08, LAPTH-1086-05",
      SLACcitation   = "%%CITATION = ASTRO-PH/0501562;%%",
}

@article{Bezrukov:2012as,
      author         = "Bezrukov, F. and Kartavtsev, A. and Lindner, M.",
      title          = "{Leptogenesis in models with keV sterile neutrino dark
                        matter}",
      journal        = "J.Phys.",
      volume         = "G40",
      pages          = "095202",
      doi            = "10.1088/0954-3899/40/9/095202",
      year           = "2013",
      eprint         = "1204.5477",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1204.5477;%%",
}

@article{Ibarra:2003up,
      author         = "Ibarra, A. and Ross, Graham G.",
      title          = "{Neutrino phenomenology: The Case of two right-handed
                        neutrinos}",
      journal        = "Phys.Lett.",
      volume         = "B591",
      pages          = "285-296",
      doi            = "10.1016/j.physletb.2004.04.037",
      year           = "2004",
      eprint         = "hep-ph/0312138",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-TH-2003-294, OUTP-0333P",
      SLACcitation   = "%%CITATION = HEP-PH/0312138;%%",
}

@article{Ibarra:2011xn,
      author         = "Ibarra, A. and Molinaro, E. and Petcov, S.T.",
      title          = "{Low Energy Signatures of the TeV Scale See-Saw
                        Mechanism}",
      journal        = "Phys.Rev.",
      volume         = "D84",
      pages          = "013005",
      doi            = "10.1103/PhysRevD.84.013005",
      year           = "2011",
      eprint         = "1103.6217",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1103.6217;%%",
}

@article{Casas:2001sr,
      author         = "Casas, J.A. and Ibarra, A.",
      title          = "{Oscillating neutrinos and $\mu\to e~\gamma$}",
      journal        = "Nucl.Phys.",
      volume         = "B618",
      pages          = "171-204",
      doi            = "10.1016/S0550-3213(01)00475-8",
      year           = "2001",
      eprint         = "hep-ph/0103065",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IEM-FT-211-01, OUTP-01-11P, IFT-UAM-CSIC-01-08",
      SLACcitation   = "%%CITATION = HEP-PH/0103065;%%",
}

@article{Capozzi:2013csa,
      author         = "Capozzi, F. and Fogli, G.L. and Lisi, E. and Marrone, A.
                        and Montanino, D. and others",
      title          = "{Status of three-neutrino oscillation parameters, circa
                        2013}",
      year           = "2013",
      eprint         = "1312.2878",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1312.2878;%%",
}

@article{Adam:2013mnn,
      author         = "Adam, J. and others",
      title          = "{New constraint on the existence of the $\mu^+ \to
                        e^+\gamma$ decay}",
      collaboration  = "MEG Collaboration",
      journal        = "Phys.Rev.Lett.",
      number         = "20",
      volume         = "110",
      pages          = "201801",
      doi            = "10.1103/PhysRevLett.110.201801",
      year           = "2013",
      eprint         = "1303.0754",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1303.0754;%%",
}
@article{Aubert:2009ag,
      author         = "Aubert, Bernard and others",
      title          = "{Searches for Lepton Flavor Violation in the Decays $\tau^\pm \to e^\pm \gamma$ and $\tau^\pm \to \mu^\pm \gamma$}",
      collaboration  = "BaBar Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "104",
      pages          = "021802",
      doi            = "10.1103/PhysRevLett.104.021802",
      year           = "2010",
      eprint         = "0908.2381",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "SLAC-PUB-13753, BABAR-PUB-09-026",
      SLACcitation   = "%%CITATION = ARXIV:0908.2381;%%",
}
@article{Toma:2013zsa,
      author         = "Toma, Takashi and Vicente, Avelino",
      title          = "{Lepton Flavor Violation in the Scotogenic Model}",
      journal        = "JHEP",
      volume         = "1401",
      pages          = "160",
      doi            = "10.1007/JHEP01(2014)160",
      year           = "2014",
      eprint         = "1312.2840",
      archivePrefix  = "arXiv",
      reportNumber   = "DCPT-13-198",
      SLACcitation   = "%%CITATION = ARXIV:1312.2840;%%",
}
@article{Ackermann:2013yva,
      author         = "Ackermann, M. and others",
      title          = "{Dark Matter Constraints from Observations of 25 Milky
                        Way Satellite Galaxies with the Fermi Large Area
                        Telescope}",
      collaboration  = "Fermi-LAT Collaboration",
      journal        = "Phys.Rev.",
      volume         = "D89",
      pages          = "042001",
      doi            = "10.1103/PhysRevD.89.042001",
      year           = "2014",
      eprint         = "1310.0828",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1310.0828;%%",
}

@article{Garcia-Cely:2013zga,
      author         = "Garcia-Cely, Camilo and Ibarra, Alejandro",
      title          = "{Novel Gamma-ray Spectral Features in the Inert Doublet
                        Model}",
      journal        = "JCAP",
      volume         = "1309",
      pages          = "025",
      doi            = "10.1088/1475-7516/2013/09/025",
      year           = "2013",
      eprint         = "1306.4681",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1306.4681;%%",
}

@article{Goudelis:2013uca,
      author         = "Goudelis, A. and Herrmann, B. and Stål, O.",
      title          = "{Dark matter in the Inert Doublet Model after the
                        discovery of a Higgs-like boson at the LHC}",
      journal        = "JHEP",
      volume         = "1309",
      pages          = "106",
      doi            = "10.1007/JHEP09(2013)106",
      year           = "2013",
      eprint         = "1303.3010",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-006-13",
      SLACcitation   = "%%CITATION = ARXIV:1303.3010;%%",
}
@article{Honorez:2010re,
      author         = "Lopez Honorez, Laura and Yaguna, Carlos E.",
      title          = "{The inert doublet model of dark matter revisited}",
      journal        = "JHEP",
      volume         = "1009",
      pages          = "046",
      doi            = "10.1007/JHEP09(2010)046",
      year           = "2010",
      eprint         = "1003.3125",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-UAM-CSIC-10-11, FTUAM-10-04, ULB-TH-10-06",
      SLACcitation   = "%%CITATION = ARXIV:1003.3125;%%",
}

@article{LopezHonorez:2010tb,
      author         = "Lopez Honorez, Laura and Yaguna, Carlos E.",
      title          = "{A new viable region of the inert doublet model}",
      journal        = "JCAP",
      volume         = "1101",
      pages          = "002",
      doi            = "10.1088/1475-7516/2011/01/002",
      year           = "2011",
      eprint         = "1011.1411",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ULB-TH-10-37",
      SLACcitation   = "%%CITATION = ARXIV:1011.1411;%%",
}
@article{Lundstrom:2008ai,
      author         = "Lundstrom, Erik and Gustafsson, Michael and Edsjo,
                        Joakim",
      title          = "{The Inert Doublet Model and LEP II Limits}",
      journal        = "Phys.Rev.",
      volume         = "D79",
      pages          = "035013",
      doi            = "10.1103/PhysRevD.79.035013",
      year           = "2009",
      eprint         = "0810.3924",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0810.3924;%%",
}
@article{Pierce:2007ut,
      author         = "Pierce, Aaron and Thaler, Jesse",
      title          = "{Natural Dark Matter from an Unnatural Higgs Boson and
                        New Colored Particles at the TeV Scale}",
      journal        = "JHEP",
      volume         = "0708",
      pages          = "026",
      doi            = "10.1088/1126-6708/2007/08/026",
      year           = "2007",
      eprint         = "hep-ph/0703056",
      archivePrefix  = "arXiv",
      primaryClass   = "HEP-PH",
      reportNumber   = "MCTP-07-11",
      SLACcitation   = "%%CITATION = HEP-PH/0703056;%%",
}
@article{ATLAS:2012jp,
      author         = "Aad, Georges and others",
      title          = "{Search for direct chargino production in
                        anomaly-mediated supersymmetry breaking models based on a
                        disappearing-track signature in $pp$ collisions at
                        $\sqrt{s}=7$ TeV with the ATLAS detector}",
      collaboration  = "ATLAS Collaboration",
      journal        = "JHEP",
      volume         = "1301",
      pages          = "131",
      doi            = "10.1007/JHEP01(2013)131",
      year           = "2013",
      eprint         = "1210.2852",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-PH-EP-2012-243",
      SLACcitation   = "%%CITATION = ARXIV:1210.2852;%%",
}
@article{Cheung:2011nn,
      author         = "Cheung, Clifford and Elor, Gilly and Hall, Lawrence",
      title          = "{Gravitino Freeze-In}",
      journal        = "Phys.Rev.",
      volume         = "D84",
      pages          = "115021",
      doi            = "10.1103/PhysRevD.84.115021",
      year           = "2011",
      eprint         = "1103.4394",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1103.4394;%%",
}
@article{Chatrchyan:2013oca,
      author         = "Chatrchyan, Serguei and others",
      title          = "{Searches for long-lived charged particles in pp
                        collisions at $\sqrt{s}$=7 and 8 TeV}",
      collaboration  = "CMS Collaboration",
      journal        = "JHEP",
      volume         = "1307",
      pages          = "122",
      doi            = "10.1007/JHEP07(2013)122",
      year           = "2013",
      eprint         = "1305.0491",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-EXO-12-026, CERN-PH-EP-2013-073",
      SLACcitation   = "%%CITATION = ARXIV:1305.0491;%%",
}

@article{Blennow:2013jba,
      author         = "Blennow, Mattias and Fernandez-Martinez, Enrique and
                        Zaldivar, Bryan",
      title          = "{Freeze-in through portals}",
      year           = "2013",
      eprint         = "1309.7348",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1309.7348;%%",
}
@article{Chu:2013jja,
      author         = "Chu, Xiaoyong and Mambrini, Yann and Quevillon, Jérémie
                        and Zaldivar, Bryan",
      title          = "{Thermal and non-thermal production of dark matter via
                        Z'-portal(s)}",
      journal        = "JCAP",
      volume         = "1401",
      pages          = "034",
      doi            = "10.1088/1475-7516/2014/01/034",
      year           = "2014",
      eprint         = "1306.4677",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1306.4677;%%",
}

@article{Arhrib:2013ela,
      author         = "Arhrib, Abdesslam and Tsai, Yue-Lin Sming and Yuan, Qiang
                        and Yuan, Tzu-Chiang",
      title          = "{An Updated Analysis of Inert Higgs Doublet Model in
                        light of the Recent Results from LUX, PLANCK, AMS-02 and
                        LHC}",
      year           = "2013",
      eprint         = "1310.0358",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1310.0358;%%",
}

@article{Ma:2012if,
      author         = "Ma, Ernest",
      title          = "{Radiative Scaling Neutrino Mass and Warm Dark Matter}",
      journal        = "Phys.Lett.",
      volume         = "B717",
      pages          = "235-237",
      doi            = "10.1016/j.physletb.2012.09.046",
      year           = "2012",
      eprint         = "1206.1812",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T522 (JUNE-2012), UCRHEP-T522-(JUNE-2012)",
      SLACcitation   = "%%CITATION = ARXIV:1206.1812;%%",
}

@article{Frigerio:2006gx,
      author         = "Frigerio, Michele and Hambye, Thomas and Ma, Ernest",
      title          = "{Right-handed sector leptogenesis}",
      journal        = "JCAP",
      volume         = "0609",
      pages          = "009",
      doi            = "10.1088/1475-7516/2006/09/009",
      year           = "2006",
      eprint         = "hep-ph/0603123",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SACLAY-T06-024, UCRHEP-T408",
      SLACcitation   = "%%CITATION = HEP-PH/0603123;%%",
}

@article{Jeltema:2014qfa,
      author         = "Jeltema, Tesla E. and Profumo, Stefano",
      title          = "{Dark matter searches going bananas: the contribution of
                        Potassium (and Chlorine) to the 3.5 keV line}",
      year           = "2014",
      eprint         = "1408.1699",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1408.1699;%%",
}

@article{Boyarsky:2014ska,
      author         = "Boyarsky, Alexey and Franse, Jeroen and Iakubovskyi,
                        Dmytro and Ruchayskiy, Oleg",
      title          = "{Checking the dark matter origin of 3.53~keV line with
                        the Milky Way center}",
      year           = "2014",
      eprint         = "1408.2503",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1408.2503;%%",
}

@article{Bulbul:2014sua,
      author         = "Bulbul, Esra and Markevitch, Maxim and Foster, Adam and
                        Smith, Randall K. and Loewenstein, Michael and others",
      title          = "{Detection of An Unidentified Emission Line in the
                        Stacked X-ray spectrum of Galaxy Clusters}",
      journal        = "Astrophys.J.",
      volume         = "789",
      pages          = "13",
      doi            = "10.1088/0004-637X/789/1/13",
      year           = "2014",
      eprint         = "1402.2301",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1402.2301;%%",
}

@article{Boyarsky:2014jta,
      author         = "Boyarsky, Alexey and Ruchayskiy, Oleg and Iakubovskyi,
                        Dmytro and Franse, Jeroen",
      title          = "{An unidentified line in X-ray spectra of the Andromeda
                        galaxy and Perseus galaxy cluster}",
      year           = "2014",
      eprint         = "1402.4119",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1402.4119;%%",
}

@article{Muhlleitner:2003me,
      author         = "Muhlleitner, Margarete and Spira, Michael",
      title          = "{A Note on doubly charged Higgs pair production at hadron
                        colliders}",
      journal        = "Phys.Rev.",
      volume         = "D68",
      pages          = "117701",
      doi            = "10.1103/PhysRevD.68.117701",
      year           = "2003",
      eprint         = "hep-ph/0305288",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "PSI-PR-03-07",
      SLACcitation   = "%%CITATION = HEP-PH/0305288;%%",
}

@article{ATLAS:2012hi,
      author         = "Aad, Georges and others",
      title          = "{Search for doubly-charged Higgs bosons in like-sign
                        dilepton final states at $\sqrt{s}=7$ TeV with the ATLAS
                        detector}",
      collaboration  = "ATLAS Collaboration",
      journal        = "Eur.Phys.J.",
      volume         = "C72",
      pages          = "2244",
      doi            = "10.1140/epjc/s10052-012-2244-2",
      year           = "2012",
      eprint         = "1210.5070",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-PH-EP-2012-265",
      SLACcitation   = "%%CITATION = ARXIV:1210.5070;%%",
}

@article{Chatrchyan:2012ya,
      author         = "Chatrchyan, Serguei and others",
      title          = "{A search for a doubly-charged Higgs boson in $pp$
                        collisions at $\sqrt{s}=7$ TeV}",
      collaboration  = "CMS Collaboration",
      journal        = "Eur.Phys.J.",
      volume         = "C72",
      pages          = "2189",
      doi            = "10.1140/epjc/s10052-012-2189-5",
      year           = "2012",
      eprint         = "1207.2666",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-HIG-12-005, CERN-PH-EP-2012-169",
      SLACcitation   = "%%CITATION = ARXIV:1207.2666;%%",
}

@article{Chatrchyan:2012vca,
      author         = "Chatrchyan, Serguei and others",
      title          = "{Search for a light charged Higgs boson in top quark
                        decays in $pp$ collisions at $\sqrt{s}=7$ TeV}",
      collaboration  = "CMS Collaboration",
      journal        = "JHEP",
      volume         = "1207",
      pages          = "143",
      doi            = "10.1007/JHEP07(2012)143",
      year           = "2012",
      eprint         = "1205.5736",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-HIG-11-019, CERN-PH-EP-2012-123",
      SLACcitation   = "%%CITATION = ARXIV:1205.5736;%%",
}

@article{DelNobile:2009st,
      author         = "Del Nobile, Eugenio and Franceschini, Roberto and
                        Pappadopulo, Duccio and Strumia, Alessandro",
      title          = "{Minimal Matter at the Large Hadron Collider}",
      journal        = "Nucl.Phys.",
      volume         = "B826",
      pages          = "217-234",
      doi            = "10.1016/j.nuclphysb.2009.10.004",
      year           = "2010",
      eprint         = "0908.1567",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFUP-TH-13-2007, CERN-PH-TH-2009-147",
      SLACcitation   = "%%CITATION = ARXIV:0908.1567;%%",
}

@article{Aad:2014vma,
      author         = "Aad, Georges and others",
      title          = "{Search for direct production of charginos, neutralinos
                        and sleptons in final states with two leptons and missing
                        transverse momentum in $pp$ collisions at $\sqrt{s} =$ 8
                        TeV with the ATLAS detector}",
      collaboration  = "ATLAS Collaboration",
      journal        = "JHEP",
      volume         = "1405",
      pages          = "071",
      doi            = "10.1007/JHEP05(2014)071",
      year           = "2014",
      eprint         = "1403.5294",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-PH-EP-2014-037",
      SLACcitation   = "%%CITATION = ARXIV:1403.5294;%%",
}

@article{Khachatryan:2014qwa,
      author         = "Khachatryan, Vardan and others",
      title          = "{Searches for electroweak production of charginos,
                        neutralinos, and sleptons decaying to leptons and W, Z,
                        and Higgs bosons in pp collisions at 8 TeV}",
      collaboration  = "CMS Collaboration",
      year           = "2014",
      eprint         = "1405.7570",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-SUS-13-006, CERN-PH-EP-2014-098",
      SLACcitation   = "%%CITATION = ARXIV:1405.7570;%%",
}

@article{Gorbunov:2007ak,
      author         = "Gorbunov, Dmitry and Shaposhnikov, Mikhail",
      title          = "{How to find neutral leptons of the $\nu$MSM?}",
      journal        = "JHEP",
      volume         = "0710",
      pages          = "015",
      doi            = "10.1007/JHEP11(2013)101, 10.1088/1126-6708/2007/10/015",
      year           = "2007",
      eprint         = "0705.1729",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0705.1729;%%",
}

@article{Merle:2011yv,
      author         = "Merle, Alexander and Niro, Viviana",
      title          = "{Deriving Models for keV sterile Neutrino Dark Matter
                        with the Froggatt-Nielsen mechanism}",
      journal        = "JCAP",
      volume         = "1107",
      pages          = "023",
      doi            = "10.1088/1475-7516/2011/07/023",
      year           = "2011",
      eprint         = "1105.5136",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1105.5136;%%",
}


@article{Shaposhnikov:2006nn,
      author         = "Shaposhnikov, Mikhail",
      title          = "{A Possible symmetry of the nuMSM}",
      journal        = "Nucl.Phys.",
      volume         = "B763",
      pages          = "49-59",
      doi            = "10.1016/j.nuclphysb.2006.11.003",
      year           = "2007",
      eprint         = "hep-ph/0605047",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2006-079",
      SLACcitation   = "%%CITATION = HEP-PH/0605047;%%",
}
@article{Lindner:2010wr,
      author         = "Lindner, Manfred and Merle, Alexander and Niro, Viviana",
      title          = "{Soft $L_e - L_\mu - L_\tau$ flavour symmetry breaking
                        and sterile neutrino keV Dark Matter}",
      journal        = "JCAP",
      volume         = "1101",
      pages          = "034",
      doi            = "10.1088/1475-7516/2011/01/034,
                        10.1088/1475-7516/2014/07/E01",
      year           = "2011",
      eprint         = "1011.4950",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1011.4950;%%",
}
@article{Merle:2013gea,
      author         = "Merle, Alexander",
      title          = "{keV Neutrino Model Building}",
      journal        = "Int.J.Mod.Phys.",
      volume         = "D22",
      pages          = "1330020",
      doi            = "10.1142/S0218271813300206",
      year           = "2013",
      eprint         = "1302.2625",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1302.2625;%%",
}

@article{Boyarsky:2007ay,
      author         = "Boyarsky, Alexey and Iakubovskyi, Dmytro and Ruchayskiy,
                        Oleg and Savchenko, Vladimir",
      title          = "{Constraints on decaying Dark Matter from XMM-Newton
                        observations of M31}",
      journal        = "Mon.Not.Roy.Astron.Soc.",
      volume         = "387",
      pages          = "1361",
      doi            = "10.1111/j.1365-2966.2008.13266.x",
      year           = "2008",
      eprint         = "0709.2301",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      SLACcitation   = "%%CITATION = ARXIV:0709.2301;%%",
}

@article{Roy:2010xq,
      author         = "Roy, Ananda and Shaposhnikov, Mikhail",
      title          = "{Resonant production of the sterile neutrino dark matter
                        and fine-tunings in the [nu]MSM}",
      journal        = "Phys.Rev.",
      volume         = "D82",
      pages          = "056014",
      doi            = "10.1103/PhysRevD.82.056014",
      year           = "2010",
      eprint         = "1006.4008",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1006.4008;%%",
}
@article{Molinaro:2014lfa,
      author         = "Molinaro, Emiliano and Yaguna, Carlos E. and Zapata,
                        Oscar",
      title          = "{FIMP realization of the scotogenic model}",
      journal        = "JCAP",
      volume         = "1407",
      pages          = "015",
      doi            = "10.1088/1475-7516/2014/07/015",
      year           = "2014",
      eprint         = "1405.1259",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FLAVOUR(267104)-ERC-67, TUM-HEP-941-14, NORDITA-2014-55,
                        MS-TP-14-19",
      SLACcitation   = "%%CITATION = ARXIV:1405.1259;%%",
}

@article{Petraki:2008ef,
      author         = "Petraki, Kalliopi",
      title          = "{Small-scale structure formation properties of chilled
                        sterile neutrinos as dark matter}",
      journal        = "Phys.Rev.",
      volume         = "D77",
      pages          = "105004",
      doi            = "10.1103/PhysRevD.77.105004",
      year           = "2008",
      eprint         = "0801.3470",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCLA-08-TEP-02",
      SLACcitation   = "%%CITATION = ARXIV:0801.3470;%%",
}

@article{Fukugita:1986hr,
      author         = "Fukugita, M. and Yanagida, T.",
      title          = "{Baryogenesis Without Grand Unification}",
      journal        = "Phys.Lett.",
      volume         = "B174",
      pages          = "45",
      doi            = "10.1016/0370-2693(86)91126-3",
      year           = "1986",
      reportNumber   = "RIFP-641",
      SLACcitation   = "%%CITATION = PHLTA,B174,45;%%",
}

@article{Davidson:2002qv,
      author         = "Davidson, Sacha and Ibarra, Alejandro",
      title          = "{A Lower bound on the right-handed neutrino mass from
                        leptogenesis}",
      journal        = "Phys.Lett.",
      volume         = "B535",
      pages          = "25-32",
      doi            = "10.1016/S0370-2693(02)01735-5",
      year           = "2002",
      eprint         = "hep-ph/0202239",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "OUTP-02-10P, IPPP-02-16, DCPT-02-32",
      SLACcitation   = "%%CITATION = HEP-PH/0202239;%%",
}

@article{Pilaftsis:1997jf,
      author         = "Pilaftsis, Apostolos",
      title          = "{CP violation and baryogenesis due to heavy Majorana
                        neutrinos}",
      journal        = "Phys.Rev.",
      volume         = "D56",
      pages          = "5431-5451",
      doi            = "10.1103/PhysRevD.56.5431",
      year           = "1997",
      eprint         = "hep-ph/9707235",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MPI-PHT-97-30",
      SLACcitation   = "%%CITATION = HEP-PH/9707235;%%",
}

@article{Akhmedov:1998qx,
      author         = "Akhmedov, Evgeny K. and Rubakov, V.A. and Smirnov, A.
                        Yu.",
      title          = "{Baryogenesis via neutrino oscillations}",
      journal        = "Phys.Rev.Lett.",
      volume         = "81",
      pages          = "1359-1362",
      doi            = "10.1103/PhysRevLett.81.1359",
      year           = "1998",
      eprint         = "hep-ph/9803255",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IC-98-22, INR-98-14-T",
      SLACcitation   = "%%CITATION = HEP-PH/9803255;%%",
}

@article{Garbrecht:2014bfa,
      author         = "Garbrecht, Bjorn",
      title          = "{More Viable Parameter Space for Leptogenesis}",
      year           = "2014",
      eprint         = "1401.3278",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1401.3278;%%",
}

@article{Asaka:2005pn,
      author         = "Asaka, Takehiko and Shaposhnikov, Mikhail",
      title          = "{The nuMSM, dark matter and baryon asymmetry of the
                        universe}",
      journal        = "Phys.Lett.",
      volume         = "B620",
      pages          = "17-26",
      doi            = "10.1016/j.physletb.2005.06.020",
      year           = "2005",
      eprint         = "hep-ph/0505013",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0505013;%%",
}

@article{Canetti:2010aw,
      author         = "Canetti, Laurent and Shaposhnikov, Mikhail",
      title          = "{Baryon Asymmetry of the Universe in the NuMSM}",
      journal        = "JCAP",
      volume         = "1009",
      pages          = "001",
      doi            = "10.1088/1475-7516/2010/09/001",
      year           = "2010",
      eprint         = "1006.0133",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1006.0133;%%",
}
@article{Shuve:2014zua,
      author         = "Shuve, Brian and Yavin, Itay",
      title          = "{Baryogenesis through Neutrino Oscillations: A Unified
                        Perspective}",
      journal        = "Phys.Rev.",
      volume         = "D89",
      pages          = "075014",
      doi            = "10.1103/PhysRevD.89.075014",
      year           = "2014",
      eprint         = "1401.2459",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1401.2459;%%",
}

@article{Ruchayskiy:2012si,
      author         = "Ruchayskiy, Oleg and Ivashko, Artem",
      title          = "{Restrictions on the lifetime of sterile neutrinos from
                        primordial nucleosynthesis}",
      journal        = "JCAP",
      volume         = "1210",
      pages          = "014",
      doi            = "10.1088/1475-7516/2012/10/014",
      year           = "2012",
      eprint         = "1202.2841",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2012-042",
      SLACcitation   = "%%CITATION = ARXIV:1202.2841;%%",
}

@article{Kusenko:2013saa,
      author         = "Kusenko, Alexander and Rosenberg, Leslie J.",
      title          = "{Working Group Report: Non-WIMP Dark Matter}",
      year           = "2013",
      eprint         = "1310.8642",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1310.8642;%%",
}

@article{Petraki:2007gq,
      author         = "Petraki, Kalliopi and Kusenko, Alexander",
      title          = "{Dark-matter sterile neutrinos in models with a gauge
                        singlet in the Higgs sector}",
      journal        = "Phys.Rev.",
      volume         = "D77",
      pages          = "065014",
      doi            = "10.1103/PhysRevD.77.065014",
      year           = "2008",
      eprint         = "0711.4646",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCLA-07-TEP-27",
      SLACcitation   = "%%CITATION = ARXIV:0711.4646;%%",
}
@article{Ibarra:2003up,
      author         = "Ibarra, A. and Ross, Graham G.",
      title          = "{Neutrino phenomenology: The Case of two right-handed
                        neutrinos}",
      journal        = "Phys.Lett.",
      volume         = "B591",
      pages          = "285-296",
      doi            = "10.1016/j.physletb.2004.04.037",
      year           = "2004",
      eprint         = "hep-ph/0312138",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-TH-2003-294, OUTP-0333P",
      SLACcitation   = "%%CITATION = HEP-PH/0312138;%%",
}

@article{Malyshev:2014xqa,
      author         = "Malyshev, D. and Neronov, A. and Eckert, D.",
      title          = "{Constraints on 3.55 keV line emission from stacked
                        observations of dwarf spheroidal galaxies}",
      year           = "2014",
      eprint         = "1408.3531",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1408.3531;%%",
}

@techreport{ATLAS-CONF-2013-090,
      title         = "{Search for charged Higgs bosons in the $\tau$+jets final
                       state with pp collision data recorded at $\sqrt s=8$ TeV
                       with the ATLAS experiment}",
      institution   = "CERN",
      address       = "Geneva",
      number        = "ATLAS-CONF-2013-090",
      month         = "Aug",
      year          = "2013",
}
@article{Boyarsky:2014paa,
      author         = "Boyarsky, A. and Franse, J. and Iakubovskyi, D. and
                        Ruchayskiy, O.",
      title          = "{Comment on the paper "Dark matter searches going
                        bananas: the contribution of Potassium (and Chlorine) to
                        the 3.5 keV line" by T. Jeltema and S. Profumo}",
      year           = "2014",
      eprint         = "1408.4388",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1408.4388;%%",
}

@article{Silverwood:2014yza,
      author         = "Silverwood, Hamish and Weniger, Christoph and Scott, Pat
                        and Bertone, Gianfranco",
      title          = "{A realistic assessment of the CTA sensitivity to dark
                        matter annihilation}",
      journal        = "JCAP",
      volume         = "1503",
      year           = "2015",
      number         = "03",
      pages          = "055",
      doi            = "10.1088/1475-7516/2015/03/055",
      eprint         = "1408.4131",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1408.4131;%%"
}

@article{Fornengo:2013xda,
      author         = "Fornengo, N. and Maccione, L. and Vittino, A.",
      title          = "{Constraints on particle dark matter from cosmic-ray
                        antiprotons}",
      journal        = "JCAP",
      volume         = "1404",
      pages          = "003",
      doi            = "10.1088/1475-7516/2014/04/003",
      year           = "2014",
      eprint         = "1312.3579",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SACLAY-T13-280-, MPP-2013-312-, LMU-ASC-84-13",
      SLACcitation   = "%%CITATION = ARXIV:1312.3579;%%",
}

@article{Bezrukov:2009yw,
      author         = "Bezrukov, F. and Gorbunov, D.",
      title          = "{Light inflaton Hunter's Guide}",
      journal        = "JHEP",
      volume         = "1005",
      pages          = "010",
      doi            = "10.1007/JHEP05(2010)010",
      year           = "2010",
      eprint         = "0912.0390",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0912.0390;%%",
}

@article{Bezrukov:2014nza,
      author         = "Bezrukov, F. and Gorbunov, D.",
      title          = "{Relic Gravity Waves and 7 keV Dark Matter from a GeV
                        scale inflaton}",
      doi            = "10.1016/j.physletb.2014.07.060",
      year           = "2014",
      eprint         = "1403.4638",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1403.4638;%%",
}

@article{Racker:2014uga,
      author         = "Racker, J. and Rius, N.",
      title          = "{Helicitogenesis: WIMPy baryogenesis with sterile
                        neutrinos and other realizations}",
      year           = "2014",
      eprint         = "1406.6105",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-14-42, FTUV-14-0419",
      SLACcitation   = "%%CITATION = ARXIV:1406.6105;%%",
}


@article{Bonivento:2013jag,
      author         = "Bonivento, W. and Boyarsky, A. and Dijkstra, H. and
                        Egede, U. and Ferro-Luzzi, M. and others",
      title          = "{Proposal to Search for Heavy Neutral Leptons at the
                        SPS}",
      year           = "2013",
      eprint         = "1310.1762",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-SPSC-2013-024, SPSC-EOI-010",
      SLACcitation   = "%%CITATION = ARXIV:1310.1762;%%",
}

@article{Canetti:2014dka,
      author         = "Canetti, Laurent and Drewes, Marco and Garbrecht, Björn",
      title          = "{Lab-to-Genesis}",
      year           = "2014",
      eprint         = "1404.7114",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TUM-HEP-939-14",
      SLACcitation   = "%%CITATION = ARXIV:1404.7114;%%",
}

@article{Drewes:2012ma,
      author         = "Drewes, Marco and Garbrecht, Björn",
      title          = "{Leptogenesis from a GeV Seesaw without Mass Degeneracy}",
      journal        = "JHEP",
      volume         = "1303",
      pages          = "096",
      doi            = "10.1007/JHEP03(2013)096",
      year           = "2013",
      eprint         = "1206.5537",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TTK-12-28",
      SLACcitation   = "%%CITATION = ARXIV:1206.5537;%%",
}

@article{Aad:2014yka,
      author         = "Aad, Georges and others",
      title          = "{Search for the direct production of charginos,
                        neutralinos and staus in final states with at least two
                        hadronically decaying taus and missing transverse momentum
                        in $pp$ collisions at $\sqrt{s}$ = 8 TeV with the ATLAS
                        detector}",
      collaboration  = "ATLAS Collaboration",
      journal        = "JHEP",
      volume         = "1410",
      pages          = "96",
      doi            = "10.1007/JHEP10(2014)096",
      year           = "2014",
      eprint         = "1407.0350",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-PH-EP-2014-121",
      SLACcitation   = "%%CITATION = ARXIV:1407.0350;%%",
}

@article{Giudice:2003jh,
      author         = "Giudice, G.F. and Notari, A. and Raidal, M. and Riotto,
                        A. and Strumia, A.",
      title          = "{Towards a complete theory of thermal leptogenesis in the
                        SM and MSSM}",
      journal        = "Nucl.Phys.",
      volume         = "B685",
      pages          = "89-149",
      doi            = "10.1016/j.nuclphysb.2004.02.019",
      year           = "2004",
      eprint         = "hep-ph/0310123",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFUP-TH-2003-37, CERN-TH-2003-240",
      SLACcitation   = "%%CITATION = HEP-PH/0310123;%%",
}

@inproceedings{Buckley:2013bha,
      author         = "Buckley, J. and others",
      title          = "{Working Group Report: WIMP Dark Matter Indirect
                        Detection}",
      booktitle      = "{Community Summer Study 2013: Snowmass on the Mississippi
                        (CSS2013) Minneapolis, MN, USA, July 29-August 6, 2013}",
      url            = "http://inspirehep.net/record/1262275/files/arXiv:1310.7040.pdf",
      year           = "2013",
      eprint         = "1310.7040",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1310.7040;%%"
}

@inproceedings{Cushman:2013zza,
      author         = "Cushman, P. and others",
      title          = "{Working Group Report: WIMP Dark Matter Direct
                        Detection}",
      booktitle      = "{Community Summer Study 2013: Snowmass on the Mississippi
                        (CSS2013) Minneapolis, MN, USA, July 29-August 6, 2013}",
      url            = "http://inspirehep.net/record/1262767/files/arXiv:1310.8327.pdf",
      year           = "2013",
      eprint         = "1310.8327",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "FERMILAB-CONF-13-688-AE",
      SLACcitation   = "%%CITATION = ARXIV:1310.8327;%%"
}

@article{Akerib:2016vxi,
      author         = "Akerib, D. S. and others",
      title          = "{Results from a search for dark matter in LUX with 332
                        live days of exposure}",
      year           = "2016",
      eprint         = "1608.07648",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1608.07648;%%"
}

@article{ATLAS:2012zim,
      title          = "{Search for New Phenomena in Monojet plus Missing
                        Transverse Momentum Final States using 10fb-1 of pp
                        Collisions at sqrt{s}=8 TeV with the ATLAS detector at the
                        LHC}",
      collaboration  = "ATLAS",
      year           = "2012",
      reportNumber   = "ATLAS-CONF-2012-147",
      SLACcitation   = "%%CITATION = ATLAS-CONF-2012-147;%%"
}

@article{Agnese:2013rvf,
      author         = "Agnese, R. and others",
      title          = "{Silicon Detector Dark Matter Results from the Final
                        Exposure of CDMS II}",
      collaboration  = "CDMS",
      journal        = "Phys. Rev. Lett.",
      volume         = "111",
      year           = "2013",
      number         = "25",
      pages          = "251301",
      doi            = "10.1103/PhysRevLett.111.251301",
      eprint         = "1304.4279",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "FERMILAB-PUB-13-104-AE-E",
      SLACcitation   = "%%CITATION = ARXIV:1304.4279;%%"
}


@article{Feng:2011vu,
      author         = "Feng, Jonathan L. and Kumar, Jason and Marfatia, Danny
                        and Sanford, David",
      title          = "{Isospin-Violating Dark Matter}",
      journal        = "Phys. Lett.",
      volume         = "B703",
      year           = "2011",
      pages          = "124-127",
      doi            = "10.1016/j.physletb.2011.07.083",
      eprint         = "1102.4331",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCI-TR-2011-03, UH511-1157-2011",
      SLACcitation   = "%%CITATION = ARXIV:1102.4331;%%"
}

@article{Kavanagh:2014rya,
      author         = "Kavanagh, Bradley J. and Fornasa, Mattia and Green, Anne
                        M.",
      title          = "{Probing WIMP particle physics and astrophysics with
                        direct detection and neutrino telescope data}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "10",
      pages          = "103533",
      doi            = "10.1103/PhysRevD.91.103533",
      eprint         = "1410.8051",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "SACLAY-T14-179",
      SLACcitation   = "%%CITATION = ARXIV:1410.8051;%%"
}


@article{Undagoitia:2015gya,
      author         = "Marrodán Undagoitia, Teresa and Rauch, Ludwig",
      title          = "{Dark matter direct-detection experiments}",
      journal        = "J. Phys.",
      volume         = "G43",
      year           = "2016",
      number         = "1",
      pages          = "013001",
      doi            = "10.1088/0954-3899/43/1/013001",
      eprint         = "1509.08767",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1509.08767;%%"
}


@article{Belanger:2008sj,
      author         = "Belanger, G. and Boudjema, F. and Pukhov, A. and Semenov,
                        A.",
      title          = "{Dark matter direct detection rate in a generic model
                        with micrOMEGAs 2.2}",
      journal        = "Comput. Phys. Commun.",
      volume         = "180",
      year           = "2009",
      pages          = "747-767",
      doi            = "10.1016/j.cpc.2008.11.019",
      eprint         = "0803.2360",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-1237-08",
      SLACcitation   = "%%CITATION = ARXIV:0803.2360;%%"
}

@article{Mizukoshi:2010ky,
      author         = "Mizukoshi, J. K. and de S. Pires, C. A. and Queiroz, F.
                        S. and Rodrigues da Silva, P. S.",
      title          = "{WIMPs in a 3-3-1 model with heavy Sterile neutrinos}",
      journal        = "Phys. Rev.",
      volume         = "D83",
      year           = "2011",
      pages          = "065024",
      doi            = "10.1103/PhysRevD.83.065024",
      eprint         = "1010.4097",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1010.4097;%%"
}

@article{Cogollo:2012ek,
      author         = "Cogollo, D. and de Andrade, A. Vital and Queiroz, F. S.
                        and Rebello Teles, P.",
      title          = "{Novel sources of Flavor Changed Neutral Currents in the
                        $331_{RHN}$ model}",
      journal        = "Eur. Phys. J.",
      volume         = "C72",
      year           = "2012",
      pages          = "2029",
      doi            = "10.1140/epjc/s10052-012-2029-7",
      eprint         = "1201.1268",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-12-896-A",
      SLACcitation   = "%%CITATION = ARXIV:1201.1268;%%"
}

@article{Abdallah:2015ter,
      author         = "Abdallah, Jalal and others",
      title          = "{Simplified Models for Dark Matter Searches at the LHC}",
      journal        = "Phys. Dark Univ.",
      volume         = "9-10",
      year           = "2015",
      pages          = "8-23",
      doi            = "10.1016/j.dark.2015.08.001",
      eprint         = "1506.03116",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-15-283-CD, CERN-PH-TH-2015-139",
      SLACcitation   = "%%CITATION = ARXIV:1506.03116;%%"
}

@article{Alvares:2012qv,
      author         = "Ruiz-Alvarez, J. D. and de S. Pires, C. A. and Queiroz,
                        Farinaldo S. and Restrepo, D. and Rodrigues da Silva, P.
                        S.",
      title          = "{On the Connection of Gamma-Rays, Dark Matter and Higgs
                        Searches at LHC}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "075011",
      doi            = "10.1103/PhysRevD.86.075011",
      eprint         = "1206.5779",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-12-873-AE",
      SLACcitation   = "%%CITATION = ARXIV:1206.5779;%%"
}

@article{Profumo:2013sca,
      author         = "Profumo, Stefano and Queiroz, Farinaldo S.",
      title          = "{Constraining the $Z'$ mass in 331 models using direct
                        dark matter detection}",
      journal        = "Eur. Phys. J.",
      volume         = "C74",
      year           = "2014",
      number         = "7",
      pages          = "2960",
      doi            = "10.1140/epjc/s10052-014-2960-x",
      eprint         = "1307.7802",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2013-012",
      SLACcitation   = "%%CITATION = ARXIV:1307.7802;%%"
}


@article{Alves:2016fqe,
      author         = "Alves, Alexandre and Arcadi, Giorgio and Dong, P. V. and
                        Duarte, Laura and Queiroz, Farinaldo S. and Valle, José
                        W. F.",
      title          = "{R-parity as a residual gauge symmetry : probing a theory
                        of cosmological dark matter}",
      journal        = "Phys. Lett.",
      volume         = "B772",
      year           = "2017",
      pages          = "825-831",
      doi            = "10.1016/j.physletb.2017.07.056",
      eprint         = "1612.04383",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-16-XX",
      SLACcitation   = "%%CITATION = ARXIV:1612.04383;%%"
}

@article{Queiroz:2016qmc,
      author         = "Queiroz, Farinaldo S.",
      title          = "{Comment on ''Polarized window for left-right symmetry
                        and a right-handed neutrino at the Large Hadron-Electron
                        Collider''}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "11",
      pages          = "118701",
      doi            = "10.1103/PhysRevD.93.118701",
      SLACcitation   = "%%CITATION = PHRVA,D93,118701;%%"
}

@article{Dong:2017ayu,
      author         = "Dong, P. V. and Phong, D. Q. and Soa, D. V. and Thao, N.
                        C.",
      title          = "{The economical 3-3-1 model revisited}",
      year           = "2017",
      eprint         = "1706.06152",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1706.06152;%%"
}

@article{Cogollo:2017foz,
      author         = "Cogollo, D.",
      title          = "{Muon Magnetic Moment and Lepton Flavor Violation in the
                        Economical 3-3-1 Model}",
      year           = "2017",
      eprint         = "1706.00397",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1706.00397;%%"
}


@article{Caetano:2012qc,
      author         = "Caetano, W. and Cogollo, D. and de S. Pires, C. A. and
                        Rodrigues da Silva, P. S.",
      title          = "{Combining type I and type II seesaw mechanisms in the
                        minimal 3-3-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "055021",
      doi            = "10.1103/PhysRevD.86.055021",
      eprint         = "1206.5741",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1206.5741;%%"
}

@article{Cogollo:2009yi,
      author         = "Cogollo, D. and Diniz, H. and de S. Pires, C. A.",
      title          = "{KeV right-handed neutrinos from type II seesaw mechanism
                        in a 3-3-1 model}",
      journal        = "Phys. Lett.",
      volume         = "B677",
      year           = "2009",
      number         = "5",
      pages          = "338-342",
      doi            = "10.1016/j.physletb.2009.05.060",
      eprint         = "0903.0370",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0903.0370;%%"
}

@article{Pas:2015eia,
      author         = "Pas, Heinrich and Rodejohann, Werner",
      title          = "{Neutrinoless Double Beta Decay}",
      journal        = "New J. Phys.",
      volume         = "17",
      year           = "2015",
      number         = "11",
      pages          = "115010",
      doi            = "10.1088/1367-2630/17/11/115010",
      eprint         = "1507.00170",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1507.00170;%%"
}

@article{Coutinho:2013lta,
      author         = "Coutinho, Y. A. and Salustino Guimar\~aes, V. and
                        Nepomuceno, A. A.",
      title          = "{Bounds on Z' from 3-3-1 model at the LHC energies}",
      journal        = "Phys. Rev.",
      volume         = "D87",
      year           = "2013",
      number         = "11",
      pages          = "115014",
      doi            = "10.1103/PhysRevD.87.115014",
      eprint         = "1304.7907",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1304.7907;%%"
}

@article{Caetano:2013nya,
      author         = "Caetano, W. and de S. Pires, C. A. and Rodrigues da
                        Silva, P. S. and Cogollo, D. and Queiroz, Farinaldo S.",
      title          = "{Explaining ATLAS and CMS Results Within the Reduced
                        Minimal 3-3-1 model}",
      journal        = "Eur. Phys. J.",
      volume         = "C73",
      year           = "2013",
      number         = "10",
      pages          = "2607",
      doi            = "10.1140/epjc/s10052-013-2607-3",
      eprint         = "1305.7246",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1305.7246;%%"
}

@article{Hooper:2011aj,
      author         = "Hooper, Dan and Queiroz, Farinaldo S. and Gnedin,
                        Nickolay Y.",
      title          = "{Non-Thermal Dark Matter Mimicking An Additional Neutrino
                        Species In The Early Universe}",
      journal        = "Phys. Rev.",
      volume         = "D85",
      year           = "2012",
      pages          = "063513",
      doi            = "10.1103/PhysRevD.85.063513",
      eprint         = "1111.6599",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "FERMILAB-PUB-11-631-A",
      SLACcitation   = "%%CITATION = ARXIV:1111.6599;%%"
}

@article{Ferreira:2011hm,
      author         = "Ferreira, Jr, J. G. and Pinheiro, P. R. D. and Pires, C.
                        A. de S. and da Silva, P. S. Rodrigues",
      title          = "{The Minimal 3-3-1 model with only two Higgs triplets}",
      journal        = "Phys. Rev.",
      volume         = "D84",
      year           = "2011",
      pages          = "095019",
      doi            = "10.1103/PhysRevD.84.095019",
      eprint         = "1109.0031",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1109.0031;%%"
}

@article{Kelso:2013zfa,
      author         = "Kelso, Chris and Pinheiro, P. R. D. and Queiroz,
                        Farinaldo S. and Shepherd, William",
      title          = "{The Muon Anomalous Magnetic Moment in the Reduced
                        Minimal 3-3-1 Model}",
      journal        = "Eur. Phys. J.",
      volume         = "C74",
      year           = "2014",
      pages          = "2808",
      doi            = "10.1140/epjc/s10052-014-2808-4",
      eprint         = "1312.0051",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2013-023",
      SLACcitation   = "%%CITATION = ARXIV:1312.0051;%%"
}

@article{Alves:2011kc,
      author         = "Alves, A. and Ramirez Barreto, E. and Dias, A. G. and de
                        S. Pires, C. A. and Queiroz, F. S. and Rodrigues da Silva,
                        P. S.",
      title          = "{Probing 3-3-1 Models in Diphoton Higgs Boson Decay}",
      journal        = "Phys. Rev.",
      volume         = "D84",
      year           = "2011",
      pages          = "115004",
      doi            = "10.1103/PhysRevD.84.115004",
      eprint         = "1109.0238",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-11-893-A",
      SLACcitation   = "%%CITATION = ARXIV:1109.0238;%%"
}


@article{Queiroz:2010rj,
      author         = "Queiroz, F. and de S. Pires, C. A. and da Silva, P. S.
                        Rodrigues",
      title          = "{A minimal 3-3-1 model with naturally sub-eV neutrinos}",
      journal        = "Phys. Rev.",
      volume         = "D82",
      year           = "2010",
      pages          = "065018",
      doi            = "10.1103/PhysRevD.82.065018",
      eprint         = "1003.1270",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1003.1270;%%"
}

@article{Alves:2012yp,
      author         = "Alves, Alexandre and Ramirez Barreto, E. and Dias, A. G.
                        and de S. Pires, C. A. and Queiroz, Farinaldo S. and
                        Rodrigues da Silva, P. S.",
      title          = "{Explaining the Higgs Decays at the LHC with an Extended
                        Electroweak Model}",
      journal        = "Eur. Phys. J.",
      volume         = "C73",
      year           = "2013",
      number         = "2",
      pages          = "2288",
      doi            = "10.1140/epjc/s10052-013-2288-y",
      eprint         = "1207.3699",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-12-870-A",
      SLACcitation   = "%%CITATION = ARXIV:1207.3699;%%"
}

@article{Dias:2004dc,
      author         = "Dias, Alex G. and Martinez, R. and Pleitez, V.",
      title          = "{Concerning the Landau pole in 3-3-1 models}",
      journal        = "Eur. Phys. J.",
      volume         = "C39",
      year           = "2005",
      pages          = "101-107",
      doi            = "10.1140/epjc/s2004-02083-0",
      eprint         = "hep-ph/0407141",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0407141;%%"
}

@article{Sharma:1999ct,
      author         = "Sharma, S. Shelly and Pisano, F.",
      title          = "{Reply to ''comment on: Majoron emitting neutrinoless
                        double beta decay in the electroweak chiral gauge
                        extensions''}",
      journal        = "Phys. Rev.",
      volume         = "D60",
      year           = "1999",
      pages          = "098702",
      doi            = "10.1103/PhysRevD.60.098702",
      eprint         = "hep-ph/9904309",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/9904309;%%"
}

@article{Schechter:1980gr,
      author         = "Schechter, J. and Valle, J. W. F.",
      title          = "{Neutrino Masses in SU(2) x U(1) Theories}",
      journal        = "Phys. Rev.",
      volume         = "D22",
      year           = "1980",
      pages          = "2227",
      doi            = "10.1103/PhysRevD.22.2227",
      reportNumber   = "SU-4217-167, COO-3533-167",
      SLACcitation   = "%%CITATION = PHRVA,D22,2227;%%"
}

@article{Maltoni:2004ei,
      author         = "Maltoni, M. and Schwetz, T. and Tortola, M. A. and Valle,
                        J. W. F.",
      title          = "{Status of global fits to neutrino oscillations}",
      journal        = "New J. Phys.",
      volume         = "6",
      year           = "2004",
      pages          = "122",
      doi            = "10.1088/1367-2630/6/1/122",
      eprint         = "hep-ph/0405172",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-04-19, TUM-HEP-548-04, YITP-SB-04-29",
      SLACcitation   = "%%CITATION = HEP-PH/0405172;%%"
}
@article{Lindner:2016bgg,
      author         = "Lindner, Manfred and Platscher, Moritz and Queiroz,
                        Farinaldo S.",
      title          = "{A Call for New Physics : The Muon Anomalous Magnetic
                        Moment and Lepton Flavor Violation}",
      year           = "2016",
      eprint         = "1610.06587",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1610.06587;%%"
}

@article{Wei:2017ago,
      author         = "Wei, Ma and Chong-Xing, Yue",
      title          = "{Charged Higgs bosons from the 3-3-1 models and the
                        $\mathcal{R}(D^{(*)})$ anomalies}",
      journal        = "Phys. Rev.",
      volume         = "D95",
      year           = "2017",
      number         = "3",
      pages          = "035040",
      doi            = "10.1103/PhysRevD.95.035040",
      eprint         = "1702.01255",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1702.01255;%%"
}


@article{Rodriguez:2016cgr,
      author         = "Rodr\'iguez, Oscar and Benavides, Richard H. and Ponce,
                        William A. and Rojas, Eduardo",
      title          = "{Flipped versions of the universal 3-3-1 and the
                        left-right symmetric models in $[SU(3)]^3$: a
                        comprehensive approach}",
      journal        = "Phys. Rev.",
      volume         = "D95",
      year           = "2017",
      number         = "1",
      pages          = "014009",
      doi            = "10.1103/PhysRevD.95.014009",
      eprint         = "1605.00575",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1605.00575;%%"
}

@article{Borges:2016nne,
      author         = "Borges, J. Sá and Ramos, Rudnei O.",
      title          = "{Symmetry breaking patterns of the 3-3-1 model at finite
                        temperature}",
      journal        = "Eur. Phys. J.",
      volume         = "C76",
      year           = "2016",
      number         = "6",
      pages          = "344",
      doi            = "10.1140/epjc/s10052-016-4168-8",
      eprint         = "1602.08165",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1602.08165;%%"
}

@article{Pires:2016vek,
      author         = "de S. Pires, C. A. and Rodrigues da Silva, P. S. and
                        Santos, A. C. O. and Siqueira, Clarissa",
      title          = "{Higgs mass and right-handed sneutrino WIMP in a
                        supersymmetric 3-3-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "5",
      pages          = "055014",
      doi            = "10.1103/PhysRevD.94.055014",
      eprint         = "1606.01853",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1606.01853;%%"
}

@article{Ferreira:2017mvp,
      author         = "Ferreira, J. G. and de S. Pires, C. A. and Rodrigues da
                        Silva, P. S. and Siqueira, Clarissa",
      title          = "{On the Higgs-like boson in the Minimal Supersymmetric
                        3-3-1 Model}",
      year           = "2017",
      eprint         = "1706.04904",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1706.04904;%%"
}

@article{RamirezBarreto:2007cie,
      author         = "Ramirez Barreto, E. and do Amaral Coutinho, Yara and Sa
                        Borges, J.",
      title          = "{Extra neutral gauge boson from two versions of the 3-3-1
                        model in future linear colliders}",
      journal        = "Eur. Phys. J.",
      volume         = "C50",
      year           = "2007",
      pages          = "909-917",
      doi            = "10.1140/epjc/s10052-007-0254-2",
      eprint         = "hep-ph/0703099",
      archivePrefix  = "arXiv",
      primaryClass   = "HEP-PH",
      SLACcitation   = "%%CITATION = HEP-PH/0703099;%%"
}

@article{CiezaMontalvo:2008sa,
      author         = "Cieza Montalvo, J. E. and Cortez, Nelson V. and Tonasse,
                        M. D.",
      title          = "{Probing doubly charged Higgs in e+ e- Colliders in 3-3-1
                        Model}",
      journal        = "Phys. Rev.",
      volume         = "D78",
      year           = "2008",
      pages          = "116003",
      doi            = "10.1103/PhysRevD.78.116003",
      eprint         = "0804.0618",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0804.0618;%%"
}

@article{Cao:2016uur,
      author         = "Cao, Qing-Hong and Zhang, Dong-Ming",
      title          = "{Collider Phenomenology of the 3-3-1 Model}",
      year           = "2016",
      eprint         = "1611.09337",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1611.09337;%%"
}

@article{Hernandez:2013mcf,
      author         = "Carcamo Hernandez, A. E. and Martinez, R. and Ochoa, F.",
      title          = "{Radiative seesaw-type mechanism of quark masses in
                        $SU(3)_C \otimes SU(3)_L \otimes U(1)_X$}",
      journal        = "Phys. Rev.",
      volume         = "D87",
      year           = "2013",
      number         = "7",
      pages          = "075009",
      doi            = "10.1103/PhysRevD.87.075009",
      eprint         = "1302.1757",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1302.1757;%%"
}

@article{Ferreira:2016uao,
      author         = "Ferreira, J. G. and de S. Pires, C. A and Rodrigues, J.
                        G. and Rodrigues da Silva, P. S.",
      title          = "{Embedding cosmological inflation, axion dark matter and
                        seesaw mechanism in a 3-3-1 gauge model}",
      journal        = "Phys. Lett.",
      volume         = "B771",
      year           = "2017",
      pages          = "199-205",
      doi            = "10.1016/j.physletb.2017.05.034",
      eprint         = "1612.01463",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1612.01463;%%"
}

@article{Hernandez:2014lpa,
      author         = "Cárcamo Hernández, A. E. and Cataño Mur, E. and
                        Martinez, R.",
      title          = "{Lepton masses and mixing in $SU(3)_{C}\otimes
                        SU(3)_{L}\otimes U(1)_{X}$ models with a $S_3$ flavor
                        symmetry}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "7",
      pages          = "073001",
      doi            = "10.1103/PhysRevD.90.073001",
      eprint         = "1407.5217",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1407.5217;%%"
}

@article{Hernandez:2015tna,
      author         = "Cárcamo Hernández, A. E. and Martinez, Roberto",
      title          = "{A predictive 3-3-1 model with $A_4$ flavor symmetry}",
      journal        = "Nucl. Phys.",
      volume         = "B905",
      year           = "2016",
      pages          = "337-358",
      doi            = "10.1016/j.nuclphysb.2016.02.025",
      eprint         = "1501.05937",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1501.05937;%%"
}

@article{Hue:2015fbb,
      author         = "Hue, L. T. and Long, H. N. and Thuc, T. T. and Phong
                        Nguyen, T.",
      title          = "{Lepton flavor violating decays of Standard-Model-like
                        Higgs in 3-3-1 model with neutral lepton}",
      journal        = "Nucl. Phys.",
      volume         = "B907",
      year           = "2016",
      pages          = "37-76",
      doi            = "10.1016/j.nuclphysb.2016.03.034",
      eprint         = "1512.03266",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1512.03266;%%"
}

@article{Machado:2016jzb,
      author         = "Machado, A. C. B. and Montaño, J. and Pleitez, V.",
      title          = "{Lepton flavor violating processes in the minimal 3-3-1
                        model with singlet sterile neutrinos}",
      year           = "2016",
      eprint         = "1604.08539",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1604.08539;%%"
}

@article{DeConto:2016osh,
      author         = "De Conto, G. and Pleitez, V.",
      title          = "{Neutron electric dipole moment in the minimal 3-3-1
                        model}",
      year           = "2016",
      eprint         = "1606.01747",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1606.01747;%%"
}

@article{Cogollo:2013mga,
      author         = "Cogollo, D. and Queiroz, Farinaldo S. and Vasconcelos,
                        P.",
      title          = "{Flavor Changing Neutral Current Processes in a Reduced
                        Minimal Scalar Sector}",
      journal        = "Mod. Phys. Lett.",
      volume         = "A29",
      year           = "2014",
      number         = "32",
      pages          = "1450173",
      doi            = "10.1142/S0217732314501739",
      eprint         = "1312.0304",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1312.0304;%%"
}


@article{Ferreira:2013nla,
      author         = "Ferreira, J. G. and de S. Pires, C. A. and Rodrigues da
                        Silva, P. S. and Sampieri, A.",
      title          = "{Higgs sector of the supersymmetric reduced 331 model}",
      journal        = "Phys. Rev.",
      volume         = "D88",
      year           = "2013",
      number         = "10",
      pages          = "105013",
      doi            = "10.1103/PhysRevD.88.105013",
      eprint         = "1308.0575",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1308.0575;%%"
}

@article{Phong:2013cfa,
      author         = "Phong, Vo Quoc and Van, Vo Thanh and Long, Hoang Ngoc",
      title          = "{Electroweak phase transition in the reduced minimal
                        3-3-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D88",
      year           = "2013",
      pages          = "096009",
      doi            = "10.1103/PhysRevD.88.096009",
      eprint         = "1309.0355",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1309.0355;%%"
}

@article{Dong:2014bha,
      author         = "Dong, P. V. and Si, D. T.",
      title          = "{Discriminating the minimal 3-3-1 models}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "11",
      pages          = "117703",
      doi            = "10.1103/PhysRevD.90.117703",
      eprint         = "1411.4400",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1411.4400;%%"
}

@article{Kelso:2014qka,
      author         = "Kelso, Chris and Long, H. N. and Martinez, R. and
                        Queiroz, Farinaldo S.",
      title          = "{Connection of $g-2_{\mu}$, electroweak, dark matter, and
                        collider constraints on 331 models}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "11",
      pages          = "113011",
      doi            = "10.1103/PhysRevD.90.113011",
      eprint         = "1408.6203",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1408.6203;%%"
}

@article{deS.Pires:2010fu,
      author         = "de S. Pires, C. A. and Queiroz, F. S. and Rodrigues da
                        Silva, P. S.",
      title          = "{Singlet Majorana fermion dark matter, DAMA, CoGeNT, and
                        CDMS-II}",
      journal        = "Phys. Rev.",
      volume         = "D82",
      year           = "2010",
      pages          = "105014",
      doi            = "10.1103/PhysRevD.82.105014",
      eprint         = "1002.4601",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1002.4601;%%"
}

@article{Queiroz:2014pra,
      author         = "Queiroz, Farinaldo S. and Sinha, Kuver and Strumia,
                        Alessandro",
      title          = "{Leptoquarks, Dark Matter, and Anomalous LHC Events}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "3",
      pages          = "035006",
      doi            = "10.1103/PhysRevD.91.035006",
      eprint         = "1409.6301",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1409.6301;%%"
}

@article{Allanach:2015ria,
      author         = "Allanach, Ben and Alves, Alexandre and Queiroz, Farinaldo
                        S. and Sinha, Kuver and Strumia, Alessandro",
      title          = "{Interpreting the CMS $\ell^+\ell^- jj E\!\!\!\!/_{\rm
                        T}$ Excess with a Leptoquark Model}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "5",
      pages          = "055023",
      doi            = "10.1103/PhysRevD.92.055023",
      eprint         = "1501.03494",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1501.03494;%%"
}

@article{Tan:2016zwf,
      author         = "Tan, Andi and others",
      title          = "{Dark Matter Results from First 98.7 Days of Data from
                        the PandaX-II Experiment}",
      collaboration  = "PandaX-II",
      journal        = "Phys. Rev. Lett.",
      volume         = "117",
      year           = "2016",
      number         = "12",
      pages          = "121303",
      doi            = "10.1103/PhysRevLett.117.121303",
      eprint         = "1607.07400",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1607.07400;%%"
}

@article{Fu:2016ega,
      author         = "Fu, Changbo and others",
      title          = "{Spin-Dependent
                        Weakly-Interacting-Massive-Particle–Nucleon Cross
                        Section Limits from First Data of PandaX-II Experiment}",
      collaboration  = "PandaX-II",
      journal        = "Phys. Rev. Lett.",
      volume         = "118",
      year           = "2017",
      number         = "7",
      pages          = "071301",
      doi            = "10.1103/PhysRevLett.118.071301",
      eprint         = "1611.06553",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1611.06553;%%"
}

@article{Aprile:2016swn,
      author         = "Aprile, E. and others",
      title          = "{XENON100 Dark Matter Results from a Combination of 477
                        Live Days}",
      collaboration  = "XENON100",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "12",
      pages          = "122001",
      doi            = "10.1103/PhysRevD.94.122001",
      eprint         = "1609.06154",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1609.06154;%%"
}


@article{Akerib:2016lao,
      author         = "Akerib, D. S. and others",
      title          = "{Results on the Spin-Dependent Scattering of Weakly
                        Interacting Massive Particles on Nucleons from the Run 3
                        Data of the LUX Experiment}",
      collaboration  = "LUX",
      journal        = "Phys. Rev. Lett.",
      volume         = "116",
      year           = "2016",
      number         = "16",
      pages          = "161302",
      doi            = "10.1103/PhysRevLett.116.161302",
      eprint         = "1602.03489",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1602.03489;%%"
}

@article{Akerib:2017kat,
      author         = "Akerib, D. S. and others",
      title          = "{Limits on spin-dependent WIMP-nucleon cross section
                        obtained from the complete LUX exposure}",
      collaboration  = "LUX",
      year           = "2017",
      eprint         = "1705.03380",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1705.03380;%%"
}

@article{Aprile:2017iyp,
      author         = "Aprile, E. and others",
      title          = "{First Dark Matter Search Results from the XENON1T
                        Experiment}",
      collaboration  = "XENON",
      year           = "2017",
      eprint         = "1705.06655",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1705.06655;%%"
}


@article{Martinez:2014ova,
      author         = "Martínez, R. and Nisperuza, J. and Ochoa, F. and Rubio,
                        J. P.",
      title          = "{Scalar dark matter with CERN-LEP data and $Z′$ search
                        at the LHC in an $U(1)′$ model}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "9",
      pages          = "095004",
      doi            = "10.1103/PhysRevD.90.095004",
      eprint         = "1408.5153",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1408.5153;%%"
}

@article{Lindner:2016kqk,
      author         = "Lindner, Manfred and Platscher, Moritz and Yaguna, Carlos
                        E. and Merle, Alexander",
      title          = "{Fermionic WIMPs and vacuum stability in the scotogenic
                        model}",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "11",
      pages          = "115027",
      doi            = "10.1103/PhysRevD.94.115027",
      eprint         = "1608.00577",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MPP-2016-168",
      SLACcitation   = "%%CITATION = ARXIV:1608.00577;%%"
}

@article{Klasen:2016vgl,
      author         = "Klasen, Michael and Lamprea, David R. and Yaguna, Carlos
                        E.",
      title          = "{Lepton flavor violation and scalar dark matter in a
                        radiative model of neutrino masses}",
      year           = "2016",
      eprint         = "1602.05137",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1602.05137;%%"
}

@article{Campos:2017dgc,
      author         = "Campos, Miguel D. and Cogollo, D. and Lindner, Manfred
                        and Melo, T. and Queiroz, Farinaldo S. and Rodejohann,
                        Werner",
      title          = "{Neutrino Masses and Absence of Flavor Changing
                        Interactions in the 2HDM from Gauge Principles}",
      year           = "2017",
      eprint         = "1705.05388",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1705.05388;%%"
}

@article{Bonilla:2016diq,
      author         = "Bonilla, Cesar and Ma, Ernest and Peinado, Eduardo and
                        Valle, Jose W. F.",
      title          = "{Two-loop Dirac neutrino mass and WIMP dark matter}",
      journal        = "Phys. Lett.",
      volume         = "B762",
      year           = "2016",
      pages          = "214-218",
      doi            = "10.1016/j.physletb.2016.09.027",
      eprint         = "1607.03931",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-16-XX, IFIC-16-47",
      SLACcitation   = "%%CITATION = ARXIV:1607.03931;%%"
}

@article{Hoang:1996gi,
      author         = "Long, Hoang Ngoc",
      title          = "{SU(3)-L x U(1)-N model for right-handed neutrino neutral
                        currents}",
      journal        = "Phys. Rev.",
      volume         = "D54",
      year           = "1996",
      pages          = "4691-4693",
      doi            = "10.1103/PhysRevD.54.4691",
      eprint         = "hep-ph/9607439",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/9607439;%%"
}


@article{Foot:1994ym,
      author         = "Foot, Robert and Long, Hoang Ngoc and Tran, Tuan A.",
      title          = "{$SU(3)_L \otimes U(1)_N$ and $SU(4)_L \otimes U(1)_N$
                        gauge models with right-handed neutrinos}",
      journal        = "Phys. Rev.",
      volume         = "D50",
      year           = "1994",
      number         = "1",
      pages          = "R34-R38",
      doi            = "10.1103/PhysRevD.50.R34",
      eprint         = "hep-ph/9402243",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MCGILL-94-10",
      SLACcitation   = "%%CITATION = HEP-PH/9402243;%%"
}

@article{Montero:1992jk,
      author         = "Montero, J. C. and Pisano, F. and Pleitez, V.",
      title          = "{Neutral currents and GIM mechanism in SU(3)-L x U(1)-N
                        models for electroweak interactions}",
      journal        = "Phys. Rev.",
      volume         = "D47",
      year           = "1993",
      pages          = "2918-2929",
      doi            = "10.1103/PhysRevD.47.2918",
      eprint         = "hep-ph/9212271",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-039-92",
      SLACcitation   = "%%CITATION = HEP-PH/9212271;%%"
}

@article{Foot:1992rh,
      author         = "Foot, Robert and Hernandez, Oscar F. and Pisano, F. and
                        Pleitez, V.",
      title          = "{Lepton masses in an SU(3)-L x U(1)-N gauge model}",
      journal        = "Phys. Rev.",
      volume         = "D47",
      year           = "1993",
      pages          = "4158-4161",
      doi            = "10.1103/PhysRevD.47.4158",
      eprint         = "hep-ph/9207264",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MCGILL-92-31, IFT-P-025-92",
      SLACcitation   = "%%CITATION = HEP-PH/9207264;%%"
}

@article{Hoang:1995vq,
      author         = "Long, Hoang Ngoc",
      title          = "{The 331 model with right handed neutrinos}",
      journal        = "Phys. Rev.",
      volume         = "D53",
      year           = "1996",
      pages          = "437-445",
      doi            = "10.1103/PhysRevD.53.437",
      eprint         = "hep-ph/9504274",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ITP-95-10-HANOI, IC-95-118",
      SLACcitation   = "%%CITATION = HEP-PH/9504274;%%"
}

@article{Frampton:1992wt,
      author         = "Frampton, P. H.",
      title          = "{Chiral dilepton model and the flavor question}",
      journal        = "Phys. Rev. Lett.",
      volume         = "69",
      year           = "1992",
      pages          = "2889-2891",
      doi            = "10.1103/PhysRevLett.69.2889",
      reportNumber   = "IFP-427-UNC",
      SLACcitation   = "%%CITATION = PRLTA,69,2889;%%"
}


@article{Pisano:1991ee,
      author         = "Pisano, F. and Pleitez, V.",
      title          = "{An SU(3) x U(1) model for electroweak interactions}",
      journal        = "Phys. Rev.",
      volume         = "D46",
      year           = "1992",
      pages          = "410-417",
      doi            = "10.1103/PhysRevD.46.410",
      eprint         = "hep-ph/9206242",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-008-92",
      SLACcitation   = "%%CITATION = HEP-PH/9206242;%%"
}

@article{Ma:2017xxj,
      author         = "Ma, Ernest and Maniatis, Markos",
      title          = "{Pseudo-Majoron as Light Mediator of Singlet Scalar Dark
                        Matter}",
      year           = "2017",
      eprint         = "1704.06675",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T577",
      SLACcitation   = "%%CITATION = ARXIV:1704.06675;%%"
}

@article{Queiroz:2014yna,
      author         = "Queiroz, Farinaldo S. and Sinha, Kuver",
      title          = "{The Poker Face of the Majoron Dark Matter Model: LUX to
                        keV Line}",
      journal        = "Phys. Lett.",
      volume         = "B735",
      year           = "2014",
      pages          = "69-74",
      doi            = "10.1016/j.physletb.2014.06.016",
      eprint         = "1404.1400",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2013-025",
      SLACcitation   = "%%CITATION = ARXIV:1404.1400;%%"
}

@article{Gonzalez-Morales:2014eaa,
      author         = "Gonzalez-Morales, Alma X. and Profumo, Stefano and
                        Queiroz, Farinaldo S.",
      title          = "{Effect of Black Holes in Local Dwarf Spheroidal Galaxies
                        on Gamma-Ray Constraints on Dark Matter Annihilation}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "10",
      pages          = "103508",
      doi            = "10.1103/PhysRevD.90.103508",
      eprint         = "1406.2424",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1406.2424;%%"
}

@article{Cogollo:2014jia,
      author         = "Cogollo, D. and Gonzalez-Morales, Alma X. and Queiroz,
                        Farinaldo S. and Teles, Patricia R.",
      title          = "{Excluding the Light Dark Matter Window of a 331 Model
                        Using LHC and Direct Dark Matter Detection Data}",
      journal        = "JCAP",
      volume         = "1411",
      year           = "2014",
      number         = "11",
      pages          = "002",
      doi            = "10.1088/1475-7516/2014/11/002",
      eprint         = "1402.3271",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1402.3271;%%"
}

@article{Alves:2014yha,
      author         = "Alves, Alexandre and Profumo, Stefano and Queiroz,
                        Farinaldo S. and Shepherd, William",
      title          = "{Effective field theory approach to the Galactic Center
                        gamma-ray excess}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "11",
      pages          = "115003",
      doi            = "10.1103/PhysRevD.90.115003",
      eprint         = "1403.5027",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1403.5027;%%"
}

@article{Queiroz:2014zfa,
      author         = "Queiroz, Farinaldo S. and Shepherd, William",
      title          = "{New Physics Contributions to the Muon Anomalous Magnetic
                        Moment: A Numerical Code}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "9",
      pages          = "095024",
      doi            = "10.1103/PhysRevD.89.095024",
      eprint         = "1403.2309",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2013-024",
      SLACcitation   = "%%CITATION = ARXIV:1403.2309;%%"
}

@article{Arcadi:2017atc,
      author         = "Arcadi, Giorgio and Lindner, Manfred and Mambrini, Yann
                        and Pierre, Mathias and Queiroz, Farinaldo S.",
      title          = "{GUT Models at Current and Future Hadron Colliders and
                        Implications to Dark Matter Searches}",
      journal        = "Phys. Lett.",
      volume         = "B771",
      year           = "2017",
      pages          = "508-514",
      doi            = "10.1016/j.physletb.2017.05.023",
      eprint         = "1704.02328",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1704.02328;%%"
}

@article{Queiroz:2013lca,
      author         = "Queiroz, Farinaldo S.",
      title          = "{Non-thermal WIMPs as Dark Radiation}",
      booktitle      = "{Proceedings, Workshop on Dark Matter, Neutrino Physics
                        and Astrophysics CETUP* 2013: 7th International Conference
                        on Interconnection between Particle Physics and Cosmology
                        (PPC 2013): Lead/Deadwood, South Dakota, USA, July, 8-13,
                        2013}",
      journal        = "AIP Conf. Proc.",
      volume         = "1604",
      year           = "2014",
      pages          = "83-90",
      doi            = "10.1063/1.4883415",
      eprint         = "1310.3026",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1310.3026;%%"
}



@article{Queiroz:2014ara,
      author         = "Queiroz, Farinaldo S. and Sinha, Kuver and Wester,
                        William",
      title          = "{Rich tapestry: Supersymmetric axions, dark radiation,
                        and inflationary reheating}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "11",
      pages          = "115009",
      doi            = "10.1103/PhysRevD.90.115009",
      eprint         = "1407.4110",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2013-026, FERMILAB-PUB-14-233-A-PPD",
      SLACcitation   = "%%CITATION = ARXIV:1407.4110;%%"
}

@article{Allahverdi:2014bva,
      author         = "Allahverdi, Rouzbeh and Dutta, Bhaskar and Queiroz,
                        Farinaldo S. and Strigari, Louis E. and Wang, Mei-Yu",
      title          = "{Dark Matter from Late Invisible Decays to/of
                        Gravitinos}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "5",
      pages          = "055033",
      doi            = "10.1103/PhysRevD.91.055033",
      eprint         = "1412.4391",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1412.4391;%%"
}

@article{Arcadi:2017jqd,
      author         = "Arcadi, Giorgio and Ghosh, Pradipta and Mambrini, Yann
                        and Pierre, Mathias and Queiroz, Farinaldo S.",
      title          = "{$Z'$ portal to Chern-Simons Dark Matter}",
      year           = "2017",
      eprint         = "1706.04198",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1706.04198;%%"
}

@article{Aprile:2015uzo,
      author         = "Aprile, E. and others",
      title          = "{Physics reach of the XENON1T dark matter experiment}",
      collaboration  = "XENON",
      journal        = "JCAP",
      volume         = "1604",
      year           = "2016",
      number         = "04",
      pages          = "027",
      doi            = "10.1088/1475-7516/2016/04/027",
      eprint         = "1512.07501",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1512.07501;%%"
}

@article{Kelso:2013paa,
      author         = "Kelso, Chris and Profumo, Stefano and Queiroz, Farinaldo
                        S.",
      title          = "{Non-thermal WIMPs as "Dark Radiation" in Light of
                        ATACAMA, SPT, WMAP9 and Planck}",
      journal        = "Phys. Rev.",
      volume         = "D88",
      year           = "2013",
      number         = "2",
      pages          = "023511",
      doi            = "10.1103/PhysRevD.88.023511",
      eprint         = "1304.5243",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1304.5243;%%"
}

@article{Kelso:2013nwa,
      author         = "Kelso, Chris and de S. Pires, C. A. and Profumo, Stefano
                        and Queiroz, Farinaldo S. and Rodrigues da Silva, P. S.",
      title          = "{A 331 WIMPy Dark Radiation Model}",
      journal        = "Eur. Phys. J.",
      volume         = "C74",
      year           = "2014",
      number         = "3",
      pages          = "2797",
      doi            = "10.1140/epjc/s10052-014-2797-3",
      eprint         = "1308.6630",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2013-014",
      SLACcitation   = "%%CITATION = ARXIV:1308.6630;%%"
}
@article{Hooper:2012sr,
      author         = "Hooper, Dan and Kelso, Chris and Queiroz, Farinaldo S.",
      title          = "{Stringent and Robust Constraints on the Dark Matter
                        Annihilation Cross Section From the Region of the Galactic
                        Center}",
      journal        = "Astropart. Phys.",
      volume         = "46",
      year           = "2013",
      pages          = "55-70",
      doi            = "10.1016/j.astropartphys.2013.04.007",
      eprint         = "1209.3015",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "FERMILAB-PUB-12-505-A",
      SLACcitation   = "%%CITATION = ARXIV:1209.3015;%%"
}

@article{Barducci:2016fue,
      author         = "Barducci, Daniele and Bharucha, Aoife and Desai, Nishita
                        and Frigerio, Michele and Fuks, Benjamin and Goudelis,
                        Andreas and Kulkarni, Suchita and Polesello, Giacomo and
                        Sengupta, Dipan",
      title          = "{Monojet searches for momentum-dependent dark matter
                        interactions}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2017",
      pages          = "078",
      doi            = "10.1007/JHEP01(2017)078",
      eprint         = "1609.07490",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-041-16",
      SLACcitation   = "%%CITATION = ARXIV:1609.07490;%%"
}

@article{Kahlhoefer:2017dnp,
      author         = "Kahlhoefer, Felix",
      title          = "{Review of LHC Dark Matter Searches}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "A32",
      year           = "2017",
      number         = "13",
      pages          = "1730006",
      doi            = "10.1142/S0217751X1730006X",
      eprint         = "1702.02430",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-17-024",
      SLACcitation   = "%%CITATION = ARXIV:1702.02430;%%"
}

@article{Arcadi:2017kky,
      author         = "Arcadi, Giorgio and Dutra, Maíra and Ghosh, Pradipta and
                        Lindner, Manfred and Mambrini, Yann and Pierre, Mathias
                        and Profumo, Stefano and Queiroz, Farinaldo S.",
      title          = "{The Waning of the WIMP? A Review of Models, Searches,
                        and Constraints}",
      year           = "2017",
      eprint         = "1703.07364",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1703.07364;%%"
}


@article{Klasen:2016qux,
      author         = "Klasen, Michael and Lyonnet, Florian and Queiroz,
                        Farinaldo S.",
      title          = "{NLO+NLL collider bounds, Dirac fermion and scalar dark
                        matter in the B–L model}",
      journal        = "Eur. Phys. J.",
      volume         = "C77",
      year           = "2017",
      number         = "5",
      pages          = "348",
      doi            = "10.1140/epjc/s10052-017-4904-8",
      eprint         = "1607.06468",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MITP-16-065",
      SLACcitation   = "%%CITATION = ARXIV:1607.06468;%%"
}
@article{Alves:2016bib,
      author         = "Alves, Alexandre and Camargo, Daniel A. and Dias, Alex G.
                        and Longas, Robinson and Nishi, Celso C. and Queiroz,
                        Farinaldo S.",
      title          = "{Collider and Dark Matter Searches in the Inert Doublet
                        Model from Peccei-Quinn Symmetry}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2016",
      pages          = "015",
      doi            = "10.1007/JHEP10(2016)015",
      eprint         = "1606.07086",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MITP-16-060",
      SLACcitation   = "%%CITATION = ARXIV:1606.07086;%%"
}
@article{Dong:2013wca,
      author         = "Dong, P. V. and Hung, H. T. and Tham, T. D.",
      title          = "{3-3-1-1 model for dark matter}",
      journal        = "Phys. Rev.",
      volume         = "D87",
      year           = "2013",
      number         = "11",
      pages          = "115003",
      doi            = "10.1103/PhysRevD.87.115003",
      eprint         = "1305.0369",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1305.0369;%%"
}

@article{Dong:2014esa,
      author         = "Dong, P. V. and Ngan, N. T. K. and Soa, D. V.",
      title          = "{Simple 3-3-1 model and implication for dark matter}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "7",
      pages          = "075019",
      doi            = "10.1103/PhysRevD.90.075019",
      eprint         = "1407.3839",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1407.3839;%%"
}

@article{Dong:2015rka,
      author         = "Dong, P. V. and Kim, C. S. and Soa, D. V. and Thuy, N.
                        T.",
      title          = "{Investigation of Dark Matter in Minimal 3-3-1 Models}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "11",
      pages          = "115019",
      doi            = "10.1103/PhysRevD.91.115019",
      eprint         = "1501.04385",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1501.04385;%%"
}

@article{Huong:2016ybt,
      author         = "Huong, D. T. and Dong, P. V.",
      title          = "{Neutrino masses and superheavy dark matter in the
                        3-3-1-1 model}",
      journal        = "Eur. Phys. J.",
      volume         = "C77",
      year           = "2017",
      number         = "4",
      pages          = "204",
      doi            = "10.1140/epjc/s10052-017-4763-3",
      eprint         = "1605.01216",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1605.01216;%%"
}

@article{daSilva:2014qba,
      author         = "Rodrigues da Silva, P. S.",
      title          = "{A Brief Review on WIMPs in 331 Electroweak Gauge
                        Models}",
      year           = "2014",
      eprint         = "1412.8633",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1412.8633;%%"
}

@article{Allanach:2015gkd,
      author         = "Allanach, Ben and Queiroz, Farinaldo S. and Strumia,
                        Alessandro and Sun, Sichun",
      title          = "{$Z′$ models for the LHCb and $g-2$ muon anomalies}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "5",
      pages          = "055045",
      doi            = "10.1103/PhysRevD.93.055045",
      eprint         = "1511.07447",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2015-028",
      SLACcitation   = "%%CITATION = ARXIV:1511.07447;%%"
}

@article{Lindner:2016lpp,
      author         = "Lindner, Manfred and Queiroz, Farinaldo S. and
                        Rodejohann, Werner",
      title          = "{Dilepton bounds on left-right symmetry at the LHC run
                        II and neutrinoless double beta decay}",
      journal        = "Phys. Lett.",
      volume         = "B762",
      year           = "2016",
      pages          = "190-195",
      doi            = "10.1016/j.physletb.2016.08.068",
      eprint         = "1604.07419",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1604.07419;%%"
}
@article{Asakura:2014lma,
      author         = "Asakura, K. and others",
      title          = "{Results from KamLAND-Zen}",
      booktitle      = "{Proceedings, 26th International Conference on Neutrino
                        Physics and Astrophysics (Neutrino 2014): Boston,
                        Massachusetts, United States, June 2-7, 2014}",
      collaboration  = "KamLAND-Zen",
      journal        = "AIP Conf. Proc.",
      volume         = "1666",
      year           = "2015",
      pages          = "170003",
      doi            = "10.1063/1.4915593",
      eprint         = "1409.0077",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1409.0077;%%"
}

@article{Lindner:2016lxq,
      author         = "Lindner, Manfred and Queiroz, Farinaldo S. and
                        Rodejohann, Werner and Yaguna, Carlos E.",
      title          = "{Left-Right Symmetry and Lepton Number Violation at the
                        Large Hadron Electron Collider}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2016",
      pages          = "140",
      doi            = "10.1007/JHEP06(2016)140",
      eprint         = "1604.08596",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1604.08596;%%"
}

@article{Rodejohann:2011mu,
      author         = "Rodejohann, Werner",
      title          = "{Neutrino-less Double Beta Decay and Particle Physics}",
      journal        = "Int. J. Mod. Phys.",
      volume         = "E20",
      year           = "2011",
      pages          = "1833-1930",
      doi            = "10.1142/S0218301311020186",
      eprint         = "1106.1334",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1106.1334;%%"
}

@article{Olive:2016xmw,
      author         = "Patrignani, C. and others",
      title          = "{Review of Particle Physics}",
      collaboration  = "Particle Data Group",
      journal        = "Chin. Phys.",
      volume         = "C40",
      year           = "2016",
      number         = "10",
      pages          = "100001",
      doi            = "10.1088/1674-1137/40/10/100001",
      SLACcitation   = "%%CITATION = CHPHD,C40,100001;%%"
}

@article{Alves:2016cqf,
      author         = "Alves, Alexandre and Arcadi, Giorgio and Mambrini, Yann
                        and Profumo, Stefano and Queiroz, Farinaldo S.",
      title          = "{Augury of darkness: the low-mass dark Z$^{′}$ portal}",
      journal        = "JHEP",
      volume         = "04",
      year           = "2017",
      pages          = "164",
      doi            = "10.1007/JHEP04(2017)164",
      eprint         = "1612.07282",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1612.07282;%%"
}


@article{Queiroz:2016gif,
      author         = "Queiroz, Farinaldo S. and Siqueira, Clarissa and Valle,
                        José W. F.",
      title          = "{Constraining Flavor Changing Interactions from LHC Run-2
                        Dilepton Bounds with Vector Mediators}",
      journal        = "Phys. Lett.",
      volume         = "B763",
      year           = "2016",
      pages          = "269-274",
      doi            = "10.1016/j.physletb.2016.10.057",
      eprint         = "1608.07295",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1608.07295;%%"
}

@article{Altmannshofer:2016jzy,
      author         = "Altmannshofer, Wolfgang and Gori, Stefania and Profumo,
                        Stefano and Queiroz, Farinaldo S.",
      title          = "{Explaining dark matter and B decay anomalies with an
                        $L_\mu - L_\tau$ model}",
      journal        = "JHEP",
      volume         = "12",
      year           = "2016",
      pages          = "106",
      doi            = "10.1007/JHEP12(2016)106",
      eprint         = "1609.04026",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MITP-16-065",
      SLACcitation   = "%%CITATION = ARXIV:1609.04026;%%"
}

@article{Bauer:2017ota,
      author         = "Bauer, Martin and Haisch, Ulrich and Kahlhoefer, Felix",
      title          = "{Simplified dark matter models with two Higgs doublets:
                        I. Pseudoscalar mediators}",
      journal        = "JHEP",
      volume         = "05",
      year           = "2017",
      pages          = "138",
      doi            = "10.1007/JHEP05(2017)138",
      eprint         = "1701.07427",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-TH-2017-011, DESY-17-010",
      SLACcitation   = "%%CITATION = ARXIV:1701.07427;%%"
}

@article{Bell:2015rdw,
      author         = "Bell, Nicole F. and Cai, Yi and Leane, Rebecca K.",
      title          = "{Mono-W Dark Matter Signals at the LHC: Simplified Model
                        Analysis}",
      journal        = "JCAP",
      volume         = "1601",
      year           = "2016",
      number         = "01",
      pages          = "051",
      doi            = "10.1088/1475-7516/2016/01/051",
      eprint         = "1512.00476",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1512.00476;%%"
}


@article{Jacques:2015zha,
      author         = "Jacques, Thomas and Nordström, Karl",
      title          = "{Mapping monojet constraints onto Simplified Dark Matter
                        Models}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2015",
      pages          = "142",
      doi            = "10.1007/JHEP06(2015)142",
      eprint         = "1502.05721",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1502.05721;%%"
}

@article{DiFranzo:2013vra,
      author         = "DiFranzo, Anthony and Nagao, Keiko I. and Rajaraman,
                        Arvind and Tait, Tim M. P.",
      title          = "{Simplified Models for Dark Matter Interacting with
                        Quarks}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2013",
      pages          = "014",
      doi            = "10.1007/JHEP11(2013)014, 10.1007/JHEP01(2014)162",
      note           = "[Erratum: JHEP01,162(2014)]",
      eprint         = "1308.2679",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCI-HEP-TR-2013-17, KEK-TH-1659",
      SLACcitation   = "%%CITATION = ARXIV:1308.2679;%%"
}

@article{Buckley:2014fba,
      author         = "Buckley, Matthew R. and Feld, David and Goncalves,
                        Dorival",
      title          = "{Scalar Simplified Models for Dark Matter}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      pages          = "015017",
      doi            = "10.1103/PhysRevD.91.015017",
      eprint         = "1410.6497",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IPPP-14-92, DCPT-14-184",
      SLACcitation   = "%%CITATION = ARXIV:1410.6497;%%"
}



@article{Berlin:2014tja,
      author         = "Berlin, Asher and Hooper, Dan and McDermott, Samuel D.",
      title          = "{Simplified Dark Matter Models for the Galactic Center
                        Gamma-Ray Excess}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "11",
      pages          = "115022",
      doi            = "10.1103/PhysRevD.89.115022",
      eprint         = "1404.0022",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-14-060-A, MCTP-14-07",
      SLACcitation   = "%%CITATION = ARXIV:1404.0022;%%"
}



@article{Goodman:2010yf,
      author         = "Goodman, Jessica and Ibe, Masahiro and Rajaraman, Arvind
                        and Shepherd, William and Tait, Tim M. P. and Yu, Hai-Bo",
      title          = "{Constraints on Light Majorana dark Matter from
                        Colliders}",
      journal        = "Phys. Lett.",
      volume         = "B695",
      year           = "2011",
      pages          = "185-188",
      doi            = "10.1016/j.physletb.2010.11.009",
      eprint         = "1005.1286",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCI-HEP-TR-2010-09",
      SLACcitation   = "%%CITATION = ARXIV:1005.1286;%%"
}

@inproceedings{Queiroz:2016awc,
      author         = "Queiroz, Farinaldo S.",
      title          = "{Dark Matter Overview: Collider, Direct and Indirect
                        Detection Searches}",
      booktitle      = "{Proceedings, 51st Rencontres de Moriond on Electroweak
                        Interactions and Unified Theories: La Thuile, Italy, March
                        12-19, 2016}",
      organization   = "ARISF",
      publisher      = "ARISF",
      year           = "2016",
      url            = "http://inspirehep.net/record/1466249/files/arXiv:1605.08788.pdf",
      pages          = "427-436",
      eprint         = "1605.08788",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1605.08788;%%"
}


@inproceedings{Profumo:2013yn,
      author         = "Profumo, Stefano",
      title          = "{Astrophysical Probes of Dark Matter}",
      booktitle      = "{Proceedings, Theoretical Advanced Study Institute in
                        Elementary Particle Physics: Searching for New Physics at
                        Small and Large Scales (TASI 2012): Boulder, Colorado,
                        June 4-29, 2012}",
      year           = "2013",
      url            = "http://inspirehep.net/record/1209480/files/arXiv:1301.0952.pdf",
      pages          = "143-189",
      doi            = "10.1142/9789814525220_0004",
      eprint         = "1301.0952",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1301.0952;%%"
}

@phdthesis{Queiroz:2013zva,
      author         = "Queiroz, Farinaldo",
      title          = "{Direct and Indirect Dark Matter Detection in Gauge
                        Theories}",
      school         = "Paraiba U.",
      year           = "2013",
      url            = "http://lss.fnal.gov/archive/thesis/2000/fermilab-thesis-2013-38.shtml",
      reportNumber   = "FERMILAB-THESIS-2013-38",
      SLACcitation   = "%%CITATION = FERMILAB-THESIS-2013-38;%%"
}

@article{Dias:2004wk,
      author         = "Dias, Alex Gomes",
      title          = "{Evading the few TeV perturbative limit in 3-3-1 models}",
      journal        = "Phys. Rev.",
      volume         = "D71",
      year           = "2005",
      pages          = "015009",
      doi            = "10.1103/PhysRevD.71.015009",
      eprint         = "hep-ph/0412163",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0412163;%%"
}
@article{Batell:2010bp,
      author         = "Batell, Brian",
      title          = "{Dark Discrete Gauge Symmetries}",
      journal        = "Phys. Rev.",
      volume         = "D83",
      year           = "2011",
      pages          = "035006",
      doi            = "10.1103/PhysRevD.83.035006",
      eprint         = "1007.0045",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "PI-PARTPHYS-192",
      SLACcitation   = "%%CITATION = ARXIV:1007.0045;%%"
}

@article{Kumar:2015wya,
      author         = "Kumar, Jason and Marfatia, Danny and Yaylali, David",
      title          = "{Vector dark matter at the LHC}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "9",
      pages          = "095027",
      doi            = "10.1103/PhysRevD.92.095027",
      eprint         = "1508.04466",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1508.04466;%%"
}


@article{Sierra:2014kua,
      author         = "Aristizabal, Sierra D. and Dhen, Mikaël and Fong, Chee
                        Sheng and Vicente, Avelino",
      title          = "{Dynamical flavor origin of $\mathbb{Z}_N$ symmetries}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "9",
      pages          = "096004",
      doi            = "10.1103/PhysRevD.91.096004",
      eprint         = "1412.5600",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1412.5600;%%"
}

@article{Farzan:2012hh,
      author         = "Farzan, Yasaman and Akbarieh, Amin Rezaei",
      title          = "{VDM: A model for Vector Dark Matter}",
      journal        = "JCAP",
      volume         = "1210",
      year           = "2012",
      pages          = "026",
      doi            = "10.1088/1475-7516/2012/10/026",
      eprint         = "1207.4272",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1207.4272;%%"
}

@article{Alves:2015mua,
      author         = "Alves, Alexandre and Berlin, Asher and Profumo, Stefano
                        and Queiroz, Farinaldo S.",
      title          = "{Dirac-fermionic dark matter in U(1)$_{X}$ models}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2015",
      pages          = "076",
      doi            = "10.1007/JHEP10(2015)076",
      eprint         = "1506.06767",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2015-004",
      SLACcitation   = "%%CITATION = ARXIV:1506.06767;%%"
}

@article{Patra:2015bga,
      author         = "Patra, Sudhanwa and Queiroz, Farinaldo S. and Rodejohann,
                        Werner",
      title          = "{Stringent Dilepton Bounds on Left-Right Models using LHC
                        data}",
      journal        = "Phys. Lett.",
      volume         = "B752",
      year           = "2016",
      pages          = "186-190",
      doi            = "10.1016/j.physletb.2015.11.009",
      eprint         = "1506.03456",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2015-022",
      SLACcitation   = "%%CITATION = ARXIV:1506.03456;%%"
}

@article{Alves:2013tqa,
      author         = "Alves, Alexandre and Profumo, Stefano and Queiroz,
                        Farinaldo S.",
      title          = "{The dark $Z^{'}$ portal: direct, indirect and collider
                        searches}",
      journal        = "JHEP",
      volume         = "04",
      year           = "2014",
      pages          = "063",
      doi            = "10.1007/JHEP04(2014)063",
      eprint         = "1312.5281",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2013-022",
      SLACcitation   = "%%CITATION = ARXIV:1312.5281;%%"
}

@article{Dong:2014wsa,
      author         = "Dong, P. V. and Huong, D. T. and Queiroz, Farinaldo S.
                        and Thuy, N. T.",
      title          = "{Phenomenology of the 3-3-1-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "7",
      pages          = "075021",
      doi            = "10.1103/PhysRevD.90.075021",
      eprint         = "1405.2591",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1405.2591;%%"
}

@article{Alves:2015pea,
      author         = "Alves, Alexandre and Berlin, Asher and Profumo, Stefano
                        and Queiroz, Farinaldo S.",
      title          = "{Dark Matter Complementarity and the Z$^\prime$ Portal}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "8",
      pages          = "083004",
      doi            = "10.1103/PhysRevD.92.083004",
      eprint         = "1501.03490",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2015-023",
      SLACcitation   = "%%CITATION = ARXIV:1501.03490;%%"
}

@article{Rodejohann:2015lca,
      author         = "Rodejohann, Werner and Yaguna, Carlos E.",
      title          = "{Scalar dark matter in the B-L model}",
      journal        = "JCAP",
      volume         = "1512",
      year           = "2015",
      number         = "12",
      pages          = "032",
      doi            = "10.1088/1475-7516/2015/12/032",
      eprint         = "1509.04036",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1509.04036;%%"
}


@article{Patra:2016ofq,
      author         = "Patra, Sudhanwa and Rodejohann, Werner and Yaguna, Carlos
                        E.",
      title          = "{A new B-L model without right-handed neutrinos}",
      year           = "2016",
      eprint         = "1607.04029",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1607.04029;%%"
}


@article{Vicente:2014wga,
      author         = "Vicente, Avelino and Yaguna, Carlos E.",
      title          = "{Probing the scotogenic model with lepton flavor
                        violating processes}",
      journal        = "JHEP",
      volume         = "02",
      year           = "2015",
      pages          = "144",
      doi            = "10.1007/JHEP02(2015)144",
      eprint         = "1412.2545",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MS-TP-14-37",
      SLACcitation   = "%%CITATION = ARXIV:1412.2545;%%"
}


@article{Hambye:2008bq,
      author         = "Hambye, Thomas",
      title          = "{Hidden vector dark matter}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2009",
      pages          = "028",
      doi            = "10.1088/1126-6708/2009/01/028",
      eprint         = "0811.0172",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ULB-TH-08-35",
      SLACcitation   = "%%CITATION = ARXIV:0811.0172;%%"
}

@article{Frigerio:2009wf,
      author         = "Frigerio, Michele and Hambye, Thomas",
      title          = "{Dark matter stability and unification without
                        supersymmetry}",
      journal        = "Phys. Rev.",
      volume         = "D81",
      year           = "2010",
      pages          = "075002",
      doi            = "10.1103/PhysRevD.81.075002",
      eprint         = "0912.1545",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ULB-TH-09-42",
      SLACcitation   = "%%CITATION = ARXIV:0912.1545;%%"
}
@article{Duerr:2013lka,
      author         = "Duerr, Michael and Fileviez Perez, Pavel",
      title          = "{Baryonic Dark Matter}",
      journal        = "Phys. Lett.",
      volume         = "B732",
      year           = "2014",
      pages          = "101-104",
      doi            = "10.1016/j.physletb.2014.03.011",
      eprint         = "1309.3970",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1309.3970;%%"
}

@article{Lindner:2013awa,
      author         = "Lindner, Manfred and Schmidt, Daniel and Watanabe,
                        Atsushi",
      title          = "{Dark matter and 
                        symmetry for the right-handed neutrinos}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      number         = "1",
      pages          = "013007",
      doi            = "10.1103/PhysRevD.89.013007",
      eprint         = "1310.6582",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1310.6582;%%"
}

@article{Basso:2008iv,
      author         = "Basso, Lorenzo and Belyaev, Alexander and Moretti,
                        Stefano and Shepherd-Themistocleous, Claire H.",
      title          = "{Phenomenology of the minimal B-L extension of the
                        Standard model: Z' and neutrinos}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "055030",
      doi            = "10.1103/PhysRevD.80.055030",
      eprint         = "0812.4313",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SHEP-08-13",
      SLACcitation   = "%%CITATION = ARXIV:0812.4313;%%"
}

@article{Cacciapaglia:2006pk,
      author         = "Cacciapaglia, G. and Csaki, C. and Marandella, G. and
                        Strumia, A.",
      title          = "{The Minimal Set of Electroweak Precision Parameters}",
      journal        = "Phys. Rev.",
      volume         = "D74",
      year           = "2006",
      pages          = "033011",
      doi            = "10.1103/PhysRevD.74.033011",
      eprint         = "hep-ph/0604111",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0604111;%%"
}
@article{Okada:2010wd,
      author         = "Okada, Nobuchika and Seto, Osamu",
      title          = "{Higgs portal dark matter in the minimal gauged
                        $U(1)_{B-L}$ model}",
      journal        = "Phys. Rev.",
      volume         = "D82",
      year           = "2010",
      pages          = "023507",
      doi            = "10.1103/PhysRevD.82.023507",
      eprint         = "1002.2525",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "HGU-CAP-002",
      SLACcitation   = "%%CITATION = ARXIV:1002.2525;%%"
}

@article{Okada:2012sg,
      author         = "Okada, Nobuchika and Orikasa, Yuta",
      title          = "{Dark matter in the classically conformal B-L model}",
      journal        = "Phys. Rev.",
      volume         = "D85",
      year           = "2012",
      pages          = "115006",
      doi            = "10.1103/PhysRevD.85.115006",
      eprint         = "1202.1405",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KEK-TH-1518",
      SLACcitation   = "%%CITATION = ARXIV:1202.1405;%%"
}

@article{Basak:2013cga,
      author         = "Basak, Tanushree and Mondal, Tanmoy",
      title          = "{Constraining Minimal $U(1)_{B-L}$ model from Dark Matter
                        Observations}",
      journal        = "Phys. Rev.",
      volume         = "D89",
      year           = "2014",
      pages          = "063527",
      doi            = "10.1103/PhysRevD.89.063527",
      eprint         = "1308.0023",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1308.0023;%%"
}

@article{Sanchez-Vega:2014rka,
      author         = "Sánchez-Vega, B. L. and Montero, J. C. and Schmitz, E.
                        R.",
      title          = "{Complex Scalar DM in a B-L Model}",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "5",
      pages          = "055022",
      doi            = "10.1103/PhysRevD.90.055022",
      eprint         = "1404.5973",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1404.5973;%%"
}

@article{Duerr:2015wfa,
      author         = "Duerr, Michael and Fileviez Perez, Pavel and Smirnov,
                        Juri",
      title          = "{Simplified Dirac Dark Matter Models}",
      year           = "2015",
      eprint         = "1506.05107",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1506.05107;%%"
}

@article{Carena:2004xs,
      author         = "Carena, Marcela and Daleo, Alejandro and Dobrescu, Bogdan
                        A. and Tait, Timothy M. P.",
      title          = "{$Z^\prime$ gauge bosons at the Tevatron}",
      journal        = "Phys. Rev.",
      volume         = "D70",
      year           = "2004",
      pages          = "093009",
      doi            = "10.1103/PhysRevD.70.093009",
      eprint         = "hep-ph/0408098",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-04-129-T",
      SLACcitation   = "%%CITATION = HEP-PH/0408098;%%"
}

@article{Chatrchyan:2012oaa,
      author         = "Chatrchyan, Serguei and others",
      title          = "{Search for heavy narrow dilepton resonances in $pp$
                        collisions at $\sqrt{s}=7$ TeV and $\sqrt{s}=8$ TeV}",
      collaboration  = "CMS",
      journal        = "Phys. Lett.",
      volume         = "B720",
      year           = "2013",
      pages          = "63-82",
      doi            = "10.1016/j.physletb.2013.02.003",
      eprint         = "1212.6175",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-EXO-12-015, CERN-PH-EP-2012-364",
      SLACcitation   = "%%CITATION = ARXIV:1212.6175;%%"
}

@article{Guo:2015lxa,
      author         = "Guo, Jun and Kang, Zhaofeng and Ko, P. and Orikasa, Yuta",
      title          = "{Accidental dark matter: Case in the scale invariant
                        local B-L model}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "11",
      pages          = "115017",
      doi            = "10.1103/PhysRevD.91.115017",
      eprint         = "1502.00508",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1502.00508;%%"
}

@article{Aad:2014aba,
      author         = "Aad, Georges and others",
      title          = "{Measurement of the Higgs boson mass from the
                        $H\rightarrow \gamma\gamma$ and $H \rightarrow ZZ^{*}
                        \rightarrow 4\ell$ channels with the ATLAS detector using
                        25 fb$^{-1}$ of $pp$ collision data}",
      collaboration  = "ATLAS",
      journal        = "Phys. Rev.",
      volume         = "D90",
      year           = "2014",
      number         = "5",
      pages          = "052004",
      doi            = "10.1103/PhysRevD.90.052004",
      eprint         = "1406.3827",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-PH-EP-2014-122",
      SLACcitation   = "%%CITATION = ARXIV:1406.3827;%%"
}

@article{Aad:2015zhl,
      author         = "Aad, Georges and others",
      title          = "{Combined Measurement of the Higgs Boson Mass in $pp$
                        Collisions at $\sqrt{s}=7$ and 8 TeV with the ATLAS and
                        CMS Experiments}",
      collaboration  = "ATLAS, CMS",
      journal        = "Phys. Rev. Lett.",
      volume         = "114",
      year           = "2015",
      pages          = "191803",
      doi            = "10.1103/PhysRevLett.114.191803",
      eprint         = "1503.07589",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "ATLAS-HIGG-2014-14, CMS-HIG-14-042, CERN-PH-EP-2015-075",
      SLACcitation   = "%%CITATION = ARXIV:1503.07589;%%"
}

@article{Khachatryan:2014jba,
      author         = "Khachatryan, Vardan and others",
      title          = "{Precise determination of the mass of the Higgs boson and
                        tests of compatibility of its couplings with the standard
                        model predictions using proton collisions at 7 and 8
                        $\,\text {TeV}$}",
      collaboration  = "CMS",
      journal        = "Eur. Phys. J.",
      volume         = "C75",
      year           = "2015",
      number         = "5",
      pages          = "212",
      doi            = "10.1140/epjc/s10052-015-3351-7",
      eprint         = "1412.8662",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CMS-HIG-14-009, CERN-PH-EP-2014-288",
      SLACcitation   = "%%CITATION = ARXIV:1412.8662;%%"
}

@article{Silveira:1985rk,
      author         = "Silveira, Vanda and Zee, A.",
      title          = "{SCALAR PHANTOMS}",
      journal        = "Phys. Lett.",
      volume         = "B161",
      year           = "1985",
      pages          = "136",
      doi            = "10.1016/0370-2693(85)90624-0",
      reportNumber   = "DOE-ER-40048-13 P5",
      SLACcitation   = "%%CITATION = PHLTA,B161,136;%%"
}

@article{Guo:2010hq,
      author         = "Guo, Wan-Lei and Wu, Yue-Liang",
      title          = "{The Real singlet scalar dark matter model}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2010",
      pages          = "083",
      doi            = "10.1007/JHEP10(2010)083",
      eprint         = "1006.2518",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1006.2518;%%"
}

@article{Djouadi:2012zc,
      author         = "Djouadi, Abdelhak and Falkowski, Adam and Mambrini, Yann
                        and Quevillon, Jeremie",
      title          = "{Direct Detection of Higgs-Portal Dark Matter at the
                        LHC}",
      journal        = "Eur. Phys. J.",
      volume         = "C73",
      year           = "2013",
      number         = "6",
      pages          = "2455",
      doi            = "10.1140/epjc/s10052-013-2455-1",
      eprint         = "1205.3169",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LPT-ORSAY-12-42",
      SLACcitation   = "%%CITATION = ARXIV:1205.3169;%%"
}
@article{Cline:2013gha,
      author         = "Cline, James M. and Kainulainen, Kimmo and Scott, Pat and
                        Weniger, Christoph",
      title          = "{Update on scalar singlet dark matter}",
      journal        = "Phys. Rev.",
      volume         = "D88",
      year           = "2013",
      pages          = "055025",
      doi            = "10.1103/PhysRevD.88.055025",
      eprint         = "1306.4710",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1306.4710;%%"
}
@article{Feng:2014vea,
      author         = "Feng, Lei and Profumo, Stefano and Ubaldi, Lorenzo",
      title          = "{Closing in on singlet scalar dark matter: LUX, invisible
                        Higgs decays and gamma-ray lines}",
      journal        = "JHEP",
      volume         = "03",
      year           = "2015",
      pages          = "045",
      doi            = "10.1007/JHEP03(2015)045",
      eprint         = "1412.1105",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1412.1105;%%"
}

@article{Mambrini:2015sia,
      author         = "Mambrini, Yann and Profumo, Stefano and Queiroz,
                        Farinaldo S.",
      title          = "{Dark Matter and Global Symmetries}",
      journal        = "Phys. Lett.",
      volume         = "B760",
      year           = "2016",
      pages          = "807-815",
      doi            = "10.1016/j.physletb.2016.07.076",
      eprint         = "1508.06635",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2015-018",
      SLACcitation   = "%%CITATION = ARXIV:1508.06635;%%"
}

@article{Profumo:2016idl,
      author         = "Profumo, Stefano and Queiroz, Farinaldo S. and Yaguna,
                        Carlos E.",
      title          = "{Extending Fermi-LAT and H.E.S.S. Limits on Gamma-ray
                        Lines from Dark Matter Annihilation}",
      journal        = "Mon. Not. Roy. Astron. Soc.",
      volume         = "461",
      year           = "2016",
      number         = "4",
      pages          = "3976-3981",
      doi            = "10.1093/mnras/stw1600",
      eprint         = "1602.08501",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1602.08501;%%"
}

@article{Goodenough:2009gk,
      author         = "Goodenough, Lisa and Hooper, Dan",
      title          = "{Possible Evidence For Dark Matter Annihilation In The
                        Inner Milky Way From The Fermi Gamma Ray Space Telescope}",
      year           = "2009",
      eprint         = "0910.2998",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-09-494-A",
      SLACcitation   = "%%CITATION = ARXIV:0910.2998;%%"
}

@article{Bhattacharya:2013hva,
      author         = "Bhattacharya, Subhaditya and Drozd, Aleksandra and
                        Grzadkowski, Bohdan and Wudka, Jose",
      title          = "{Two-Component Dark Matter}",
      journal        = "JHEP",
      volume         = "10",
      year           = "2013",
      pages          = "158",
      doi            = "10.1007/JHEP10(2013)158",
      eprint         = "1309.2986",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCRHEP-T537",
      SLACcitation   = "%%CITATION = ARXIV:1309.2986;%%"
}

@article{Belanger:2007dx,
      author         = "Belanger, Genevieve and Pukhov, Alexander and Servant,
                        Geraldine",
      title          = "{Dirac Neutrino Dark Matter}",
      journal        = "JCAP",
      volume         = "0801",
      year           = "2008",
      pages          = "009",
      doi            = "10.1088/1475-7516/2008/01/009",
      eprint         = "0706.0526",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-1184-07, CERN-PH-TH-2007-083",
      SLACcitation   = "%%CITATION = ARXIV:0706.0526;%%"
}

@article{Arina:2007tm,
      author         = "Arina, Chiara and Fornengo, Nicolao",
      title          = "{Sneutrino cold dark matter, a new analysis: Relic
                        abundance and detection rates}",
      journal        = "JHEP",
      volume         = "11",
      year           = "2007",
      pages          = "029",
      doi            = "10.1088/1126-6708/2007/11/029",
      eprint         = "0709.4477",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DFTT-17-2007",
      SLACcitation   = "%%CITATION = ARXIV:0709.4477;%%"
}

@article{Dass:1984qc,
      author         = "Dass, G. V.",
      title          = "{DISTINGUISHING BETWEEN DIRAC AND MAJORANA NEUTRINOS IN
                        NEUTRINO - ELECTRON SCATTERING}",
      journal        = "Phys. Rev.",
      volume         = "D32",
      year           = "1985",
      pages          = "1239",
      doi            = "10.1103/PhysRevD.32.1239",
      reportNumber   = "Print-84-0962 (BOMBAY)",
      SLACcitation   = "%%CITATION = PHRVA,D32,1239;%%"
}


@article{Rosen:1982pj,
      author         = "Rosen, Simon Peter",
      title          = "{Analog of the Michel Parameter for Neutrino - Electron
                        Scattering: A Test for Majorana Neutrinos}",
      journal        = "Phys. Rev. Lett.",
      volume         = "48",
      year           = "1982",
      pages          = "842",
      doi            = "10.1103/PhysRevLett.48.842",
      reportNumber   = "PURD-TH-81-8",
      SLACcitation   = "%%CITATION = PRLTA,48,842;%%"
}

@article{Primack:1988zm,
      author         = "Primack, Joel R. and Seckel, David and Sadoulet, Bernard",
      title          = "{Detection of Cosmic Dark Matter}",
      journal        = "Ann. Rev. Nucl. Part. Sci.",
      volume         = "38",
      year           = "1988",
      pages          = "751-807",
      doi            = "10.1146/annurev.ns.38.120188.003535",
      reportNumber   = "SCIPP-88-14",
      SLACcitation   = "%%CITATION = ARNUA,38,751;%%"
}

@article{Esch:2014jpa,
      author         = "Esch, Sonja and Klasen, Michael and Yaguna, Carlos E.",
      title          = "{A minimal model for two-component dark matter}",
      journal        = "JHEP",
      volume         = "09",
      year           = "2014",
      pages          = "108",
      doi            = "10.1007/JHEP09(2014)108",
      eprint         = "1406.0617",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MS-TP-14-22",
      SLACcitation   = "%%CITATION = ARXIV:1406.0617;%%"
}

@article{Aoki:2012ub,
      author         = "Aoki, Mayumi and Duerr, Michael and Kubo, Jisuke and
                        Takano, Hiroshi",
      title          = "{Multi-Component Dark Matter Systems and Their
                        Observation Prospects}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "076015",
      doi            = "10.1103/PhysRevD.86.076015",
      eprint         = "1207.3318",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KANAZAWA-12-07",
      SLACcitation   = "%%CITATION = ARXIV:1207.3318;%%"
}

@article{Malling:2011va,
      author         = "Malling, D. C. and others",
      title          = "{After LUX: The LZ Program}",
      year           = "2011",
      eprint         = "1110.0103",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1110.0103;%%"
}

@article{D'Eramo:2010ep,
      author         = "D'Eramo, Francesco and Thaler, Jesse",
      title          = "{Semi-annihilation of Dark Matter}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2010",
      pages          = "109",
      doi            = "10.1007/JHEP06(2010)109",
      eprint         = "1003.5912",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MIT-CTP-4136",
      SLACcitation   = "%%CITATION = ARXIV:1003.5912;%%"
}

@article{Boucenna:2012rc,
      author         = "Boucenna, M. S. and Lineros, R. A. and Valle, J. W. F",
      title          = "{Planck-scale effects on WIMP dark matter}",
      journal        = "Front. Phys.",
      volume         = "1",
      year           = "2013",
      pages          = "34",
      doi            = "10.3389/fphy.2013.00034",
      eprint         = "1204.2576",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-12-16",
      SLACcitation   = "%%CITATION = ARXIV:1204.2576;%%"
}


@article{Doro:2012xx,
      author         = "Doro, M. and others",
      title          = "{Dark Matter and Fundamental Physics with the Cherenkov
                        Telescope Array}",
      collaboration  = "CTA Consortium",
      journal        = "Astropart. Phys.",
      volume         = "43",
      year           = "2013",
      pages          = "189-214",
      doi            = "10.1016/j.astropartphys.2012.08.002",
      eprint         = "1208.5356",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.IM",
      SLACcitation   = "%%CITATION = ARXIV:1208.5356;%%"
}

@inproceedings{Wood:2013taa,
      author         = "Wood, Matthew and Buckley, Jim and Digel, Seth and Funk,
                        Stefan and Nieto, Daniel and Sanchez-Conde, Miguel A.",
      title          = "{Prospects for Indirect Detection of Dark Matter with
                        CTA}",
      booktitle      = "{Community Summer Study 2013: Snowmass on the Mississippi
                        (CSS2013) Minneapolis, MN, USA, July 29-August 6, 2013}",
      url            = "http://www.slac.stanford.edu/econf/C1307292/docs/submittedArxivFiles/1305.0302.pdf",
      year           = "2013",
      eprint         = "1305.0302",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1305.0302;%%"
}

@article{Pierre:2014tra,
      author         = "Pierre, Mathias and Siegal-Gaskins, Jennifer M. and
                        Scott, Pat",
      title          = "{Sensitivity of CTA to dark matter signals from the
                        Galactic Center}",
      journal        = "JCAP",
      volume         = "1406",
      year           = "2014",
      pages          = "024",
      doi            = "10.1088/1475-7516/2014/10/E01,
                        10.1088/1475-7516/2014/06/024",
      note           = "[Erratum: JCAP1410,E01(2014)]",
      eprint         = "1401.7330",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1401.7330;%%"
}

@article{Lefranc:2015pza,
      author         = "Lefranc, Valentin and Moulin, Emmanuel and Panci, Paolo
                        and Silk, Joseph",
      title          = "{Prospects for Annihilating Dark Matter in the inner
                        Galactic halo by the Cherenkov Telescope Array}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "12",
      pages          = "122003",
      doi            = "10.1103/PhysRevD.91.122003",
      eprint         = "1502.05064",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1502.05064;%%"
}

@article{Abramowski:2011hc,
      author         = "Abramowski, A. and others",
      title          = "{Search for a Dark Matter annihilation signal from the
                        Galactic Center halo with H.E.S.S}",
      collaboration  = "HESS",
      journal        = "Phys. Rev. Lett.",
      volume         = "106",
      year           = "2011",
      pages          = "161301",
      doi            = "10.1103/PhysRevLett.106.161301",
      eprint         = "1103.3266",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1103.3266;%%"
}

@article{Ackermann:2015zua,
      author         = "Ackermann, M. and others",
      title          = "{Searching for Dark Matter Annihilation from Milky Way
                        Dwarf Spheroidal Galaxies with Six Years of Fermi Large
                        Area Telescope Data}",
      collaboration  = "Fermi-LAT",
      journal        = "Phys. Rev. Lett.",
      volume         = "115",
      year           = "2015",
      number         = "23",
      pages          = "231301",
      doi            = "10.1103/PhysRevLett.115.231301",
      eprint         = "1503.02641",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      reportNumber   = "FERMILAB-PUB-15-081-AE",
      SLACcitation   = "%%CITATION = ARXIV:1503.02641;%%"
}


@article{Acharya:2013sxa,
      author         = "Acharya, B. S. and others",
      title          = "{Introducing the CTA concept}",
      journal        = "Astropart. Phys.",
      volume         = "43",
      year           = "2013",
      pages          = "3-18",
      doi            = "10.1016/j.astropartphys.2013.01.007",
      SLACcitation   = "%%CITATION = APHYE,43,3;%%"
}
@article{Bergstrom:2010gh,
      author         = "Bergstrom, Lars and Bringmann, Torsten and Edsjo, Joakim",
      title          = "{Complementarity of direct dark matter detection and
                        indirect detection through gamma-rays}",
      journal        = "Phys. Rev.",
      volume         = "D83",
      year           = "2011",
      pages          = "045024",
      doi            = "10.1103/PhysRevD.83.045024",
      eprint         = "1011.4514",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1011.4514;%%"
}
@article{Bringmann:2007nk,
      author         = "Bringmann, Torsten and Bergstrom, Lars and Edsjo, Joakim",
      title          = "{New Gamma-Ray Contributions to Supersymmetric Dark
                        Matter Annihilation}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2008",
      pages          = "049",
      doi            = "10.1088/1126-6708/2008/01/049",
      eprint         = "0710.3169",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0710.3169;%%"
}

@article{Belanger:2015kga,
      author         = "Belanger, Genevieve and Dumont, Beranger and Goudelis,
                        Andreas and Herrmann, Bjorn and Kraml, Sabine and
                        Sengupta, Dipan",
      title          = "{Dilepton constraints in the Inert Doublet Model from Run
                        1 of the LHC}",
      journal        = "Phys. Rev.",
      volume         = "D91",
      year           = "2015",
      number         = "11",
      pages          = "115011",
      doi            = "10.1103/PhysRevD.91.115011",
      eprint         = "1503.07367",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LAPTH-015-15, CTPU-15-04, LPSC-15084",
      SLACcitation   = "%%CITATION = ARXIV:1503.07367;%%"
}

@article{Cirelli:2007xd,
      author         = "Cirelli, Marco and Strumia, Alessandro and Tamburini,
                        Matteo",
      title          = "{Cosmology and Astrophysics of Minimal Dark Matter}",
      journal        = "Nucl. Phys.",
      volume         = "B787",
      year           = "2007",
      pages          = "152-175",
      doi            = "10.1016/j.nuclphysb.2007.07.023",
      eprint         = "0706.4071",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFUP-TH-2007-12, SACLAY-T07-052",
      SLACcitation   = "%%CITATION = ARXIV:0706.4071;%%"
}

@article{Hisano:2006nn,
      author         = "Hisano, Junji and Matsumoto, Shigeki and Nagai, Minoru
                        and Saito, Osamu and Senami, Masato",
      title          = "{Non-perturbative effect on thermal relic abundance of
                        dark matter}",
      journal        = "Phys. Lett.",
      volume         = "B646",
      year           = "2007",
      pages          = "34-38",
      doi            = "10.1016/j.physletb.2007.01.012",
      eprint         = "hep-ph/0610249",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "KEK-TH-1111",
      SLACcitation   = "%%CITATION = HEP-PH/0610249;%%"
}

@misc{talkSEIDM,
  title = {{Sommerfeld Enhancement in the Inert Doublet Model}},
  howpublished = {Talk given at MIAPP in February 2015 by C. Garcia Cely.}
}

@article{Ripken:2012db,
      author         = "Ripken, Joachim and Cuoco, Alessandro and Zechlin,
                        Hannes-S. and Conrad, Jan and Horns, Dieter",
      title          = "{The sensitivity of Cherenkov telescopes to dark matter
                        and astrophysical anisotropies in the diffuse gamma-ray
                        background}",
      journal        = "JCAP",
      volume         = "1401",
      year           = "2014",
      number         = "01",
      pages          = "049",
      doi            = "10.1088/1475-7516/2014/01/049",
      eprint         = "1211.6922",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1211.6922;%%"
}

@inproceedings{Lefranc:2015vza,
      author         = "Lefranc, V. and Moulin, E.",
      title          = "{Dark matter search in the inner Galactic halo with
                        H.E.S.S. I and H.E.S.S. II}",
      booktitle      = "{Proceedings, 34th International Cosmic Ray Conference
                        (ICRC 2015)}",
      collaboration  = "HESS",
      url            = "http://inspirehep.net/record/1393231/files/arXiv:1509.04123.pdf",
      year           = "2015",
      eprint         = "1509.04123",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1509.04123;%%"
}
@phdthesis{GarciaCely:2014jha,
      author         = "Garcia Cely, Camilo A.",
      title          = "{Dark Matter Phenomenology in Scalar Extensions of the
                        Standard Model}",
      school         = "Munich, Tech. U.",
      year           = "2014-08-06",
      url            = "http://mediatum.ub.tum.de?id=1224968",
      SLACcitation   = "%%CITATION = INSPIRE-1329883;%%"
}

@article{Bringmann:2011ye,
      author         = "Bringmann, Torsten and Calore, Francesca and Vertongen,
                        Gilles and Weniger, Christoph",
      title          = "{On the Relevance of Sharp Gamma-Ray Features for
                        Indirect Dark Matter Searches}",
      journal        = "Phys. Rev.",
      volume         = "D84",
      year           = "2011",
      pages          = "103525",
      doi            = "10.1103/PhysRevD.84.103525",
      eprint         = "1106.1874",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-11-097, MPP-2011-60",
      SLACcitation   = "%%CITATION = ARXIV:1106.1874;%%"
}


@article{Cirelli:2012ut,
      author         = "Cirelli, Marco and Moulin, Emmanuel and Panci, Paolo and
                        Serpico, Pasquale D. and Viana, Aion",
      title          = "{Gamma ray constraints on Decaying Dark Matter}",
      journal        = "Phys. Rev.",
      volume         = "D86",
      year           = "2012",
      pages          = "083506",
      doi            = "10.1103/PhysRevD.86.083506, 10.1103/PhysRevD.86.109901",
      eprint         = "1205.5283",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "CERN-PH-TH-2012-110, SACLAY-T12-034, IRFU-12-34,
                        CP3-ORIGINS-2012-10, DIAS-2012-11, LAPTH-023-12,
                        SACLAY--T12-034, --CP3-ORIGINS-2012-10",
      SLACcitation   = "%%CITATION = ARXIV:1205.5283;%%"
}

@inproceedings{Carr:2015hta,
      author         = "Carr, J. and others",
      title          = "{Prospects for Indirect Dark Matter Searches with the
                        Cherenkov Telescope Array (CTA)}",
      booktitle      = "{Proceedings, 34th International Cosmic Ray Conference
                        (ICRC 2015)}",
      collaboration  = "CTA Consortium",
      url            = "http://inspirehep.net/record/1389681/files/arXiv:1508.06128.pdf",
      year           = "2015",
      eprint         = "1508.06128",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1508.06128;%%"
}

@article{Ibarra:2015tya,
      author         = "Ibarra, Alejandro and Lamperstorfer, Anna S. and
                        López-Gehler, Sergio and Pato, Miguel and Bertone,
                        Gianfranco",
      title          = "{On the sensitivity of CTA to gamma-ray boxes from
                        multi-TeV dark matter}",
      journal        = "JCAP",
      volume         = "1509",
      year           = "2015",
      number         = "09",
      pages          = "048",
      doi            = "10.1088/1475-7516/2015/09/048",
      eprint         = "1503.06797",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1503.06797;%%"
}

@article{Roszkowski:2014iqa,
      author         = "Roszkowski, Leszek and Sessolo, Enrico Maria and
                        Williams, Andrew J.",
      title          = "{Prospects for dark matter searches in the pMSSM}",
      journal        = "JHEP",
      volume         = "02",
      year           = "2015",
      pages          = "014",
      doi            = "10.1007/JHEP02(2015)014",
      eprint         = "1411.5214",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1411.5214;%%"
}

@article{Esmaili:2012us,
      author         = "Esmaili, Arman and Ibarra, Alejandro and Peres, Orlando
                        L. G.",
      title          = "{Probing the stability of superheavy dark matter
                        particles with high-energy neutrinos}",
      journal        = "JCAP",
      volume         = "1211",
      year           = "2012",
      pages          = "034",
      doi            = "10.1088/1475-7516/2012/11/034",
      eprint         = "1205.5281",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1205.5281;%%"
}
@article{Covi:2009xn,
      author         = "Covi, Laura and Grefe, Michael and Ibarra, Alejandro and
                        Tran, David",
      title          = "{Neutrino Signals from Dark Matter Decay}",
      journal        = "JCAP",
      volume         = "1004",
      year           = "2010",
      pages          = "017",
      doi            = "10.1088/1475-7516/2010/04/017",
      eprint         = "0912.3521",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-09-164, TUM-HEP-743-09",
      SLACcitation   = "%%CITATION = ARXIV:0912.3521;%%"
}
@article{Aisati:2015vma,
      author         = "El Aisati, Chaïmae and Gustafsson, Michael and Hambye,
                        Thomas",
      title          = "{New Search for Monochromatic Neutrinos from Dark Matter
                        Decay}",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "12",
      pages          = "123515",
      doi            = "10.1103/PhysRevD.92.123515",
      eprint         = "1506.02657",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ULB-TH-15-06",
      SLACcitation   = "%%CITATION = ARXIV:1506.02657;%%"
}

@article{Abbasi:2011eq,
      author         = "Abbasi, R. and others",
      title          = "{Search for Dark Matter from the Galactic Halo with the
                        IceCube Neutrino Observatory}",
      collaboration  = "IceCube",
      journal        = "Phys. Rev.",
      volume         = "D84",
      year           = "2011",
      pages          = "022004",
      doi            = "10.1103/PhysRevD.84.022004",
      eprint         = "1101.3349",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1101.3349;%%"
}

@article{Ando:2015qda,
      author         = "Ando, Shin'ichiro and Ishiwata, Koji",
      title          = "{Constraints on decaying dark matter from the
                        extragalactic gamma-ray background}",
      journal        = "JCAP",
      volume         = "1505",
      year           = "2015",
      number         = "05",
      pages          = "024",
      doi            = "10.1088/1475-7516/2015/05/024",
      eprint         = "1502.02007",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "DESY-15-020",
      SLACcitation   = "%%CITATION = ARXIV:1502.02007;%%"
}

@article{Cirelli:2010xx,
      author         = "Cirelli, Marco and Corcella, Gennaro and Hektor, Andi and
                        Hutsi, Gert and Kadastik, Mario and Panci, Paolo and
                        Raidal, Martti and Sala, Filippo and Strumia, Alessandro",
      title          = "{PPPC 4 DM ID: A Poor Particle Physicist Cookbook for
                        Dark Matter Indirect Detection}",
      journal        = "JCAP",
      volume         = "1103",
      year           = "2011",
      pages          = "051",
      doi            = "10.1088/1475-7516/2012/10/E01,
                        10.1088/1475-7516/2011/03/051",
      note           = "[Erratum: JCAP1210,E01(2012)]",
      eprint         = "1012.4515",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-PH-TH-2010-057, SACLAY-T10-025, IFUP-TH-2010-44",
      SLACcitation   = "%%CITATION = ARXIV:1012.4515;%%"
}
@article{Ciafaloni:2010ti,
      author         = "Ciafaloni, Paolo and Comelli, Denis and Riotto, Antonio
                        and Sala, Filippo and Strumia, Alessandro and Urbano,
                        Alfredo",
      title          = "{Weak Corrections are Relevant for Dark Matter Indirect
                        Detection}",
      journal        = "JCAP",
      volume         = "1103",
      year           = "2011",
      pages          = "019",
      doi            = "10.1088/1475-7516/2011/03/019",
      eprint         = "1009.0224",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFUP-TH-2010-24, CERN-PH-TH-2010-179",
      SLACcitation   = "%%CITATION = ARXIV:1009.0224;%%"
}

@article{Aartsen:2015bwa,
      author         = "Aartsen, M. G. and others",
      title          = "{The IceCube Neutrino Observatory - Contributions to ICRC
                        2015 Part IV: Searches for Dark Matter and Exotic
                        Particles}",
      collaboration  = "IceCube",
      year           = "2015",
      eprint         = "1510.05226",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1510.05226;%%"
}

@article{Aartsen:2015xej,
      author         = "Aartsen, M. G. and others",
      title          = "{Search for Dark Matter Annihilation in the Galactic
                        Center with IceCube-79}",
      collaboration  = "IceCube",
      journal        = "Eur. Phys. J.",
      volume         = "C75",
      year           = "2015",
      number         = "10",
      pages          = "492",
      doi            = "10.1140/epjc/s10052-015-3713-1",
      eprint         = "1505.07259",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1505.07259;%%"
}

@inproceedings{Frankiewicz:2015zma,
      author         = "Frankiewicz, Katarzyna",
      title          = "{Searching for Dark Matter Annihilation into Neutrinos
                        with Super-Kamiokande}",
      booktitle      = "{Meeting of the APS Division of Particles and Fields (DPF
                        2015) Ann Arbor, Michigan, USA, August 4-8, 2015}",
      collaboration  = "Super-Kamiokande",
      url            = "http://inspirehep.net/record/1401009/files/arXiv:1510.07999.pdf",
      year           = "2015",
      eprint         = "1510.07999",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1510.07999;%%"
}

@misc{Fermidata,
  title = {Figures and data files for a LAT paper},
  howpublished = {\url{http://www-glast.stanford.edu/pub_data/1048/}}
}

@article{Kavanagh:2017hcl,
      author         = "Kavanagh, Bradley J. and Queiroz, Farinaldo S. and
                        Rodejohann, Werner and Yaguna, Carlos E.",
      title          = "{Prospects for determining the particle/antiparticle
                        nature of WIMP dark matter with direct detection
                        experiments}",
      year           = "2017",
      eprint         = "1706.07819",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1706.07819;%%"
}

@article{Reig:2016ewy,
      author         = "Reig, Mario and Valle, Jose W. F. and Vaquera-Araujo, C.
                        A.",
      title          = "{Realistic $\mathrm{SU(3)_c \otimes SU(3)_L \otimes
                        U(1)_X}$ model with a type II Dirac neutrino seesaw
                        mechanism}",
      journal        = "Phys. Rev.",
      volume         = "D94",
      year           = "2016",
      number         = "3",
      pages          = "033012",
      doi            = "10.1103/PhysRevD.94.033012",
      eprint         = "1606.08499",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFIC-16-44",
      SLACcitation   = "%%CITATION = ARXIV:1606.08499;%%"
}

@article{Akhmedov:2006de,
      author         = "Akhmedov, Evgeny K. and Frigerio, M.",
      title          = "{Interplay of type I and type II seesaw contributions to
                        neutrino mass}",
      journal        = "JHEP",
      volume         = "01",
      year           = "2007",
      pages          = "043",
      doi            = "10.1088/1126-6708/2007/01/043",
      eprint         = "hep-ph/0609046",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "SACLAY-T06-105",
      SLACcitation   = "%%CITATION = HEP-PH/0609046;%%"
}

@article{Gu:2006wj,
      author         = "Gu, Pei-Hong and Zhang, He and Zhou, Shun",
      title          = "{A Minimal Type II Seesaw Model}",
      journal        = "Phys. Rev.",
      volume         = "D74",
      year           = "2006",
      pages          = "076002",
      doi            = "10.1103/PhysRevD.74.076002",
      eprint         = "hep-ph/0606302",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0606302;%%"
}

@article{Mohapatra:1999zr,
      author         = "Mohapatra, R. N. and Perez-Lorenzana, Abdel and de Sousa
                        Pires, Carlos Antonio",
      title          = "{Type II seesaw and a gauge model for the bimaximal
                        mixing explanation of neutrino puzzles}",
      journal        = "Phys. Lett.",
      volume         = "B474",
      year           = "2000",
      pages          = "355-360",
      doi            = "10.1016/S0370-2693(00)00026-5",
      eprint         = "hep-ph/9911395",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UMD-PP-00-043",
      SLACcitation   = "%%CITATION = HEP-PH/9911395;%%"
}
@article{Montero:2001ts,
      author         = "Montero, J. C. and De S. Pires, C. A. and Pleitez, V.",
      title          = "{Neutrino masses through the seesaw mechanism in 3-3-1
                        models}",
      journal        = "Phys. Rev.",
      volume         = "D65",
      year           = "2002",
      pages          = "095001",
      doi            = "10.1103/PhysRevD.65.095001",
      eprint         = "hep-ph/0112246",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-074-2001",
      SLACcitation   = "%%CITATION = HEP-PH/0112246;%%"
}

@article{Montero:2001ji,
      author         = "Montero, J. C. and de S. Pires, C. A. and Pleitez, V.",
      title          = "{Seesaw tau lepton mass and calculable neutrino masses in
                        a 3-3-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D65",
      year           = "2002",
      pages          = "093017",
      doi            = "10.1103/PhysRevD.65.093017",
      eprint         = "hep-ph/0103096",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-098-2000",
      SLACcitation   = "%%CITATION = HEP-PH/0103096;%%"
}

@article{Montero:1999su,
      author         = "Montero, J. C. and de Sousa Pires, Carlos Antonio and
                        Pleitez, V.",
      title          = "{Comment on ''Majoron emitting neutrinoless double beta
                        decay in the electroweak chiral gauge extensions''}",
      journal        = "Phys. Rev.",
      volume         = "D60",
      year           = "1999",
      pages          = "098701",
      doi            = "10.1103/PhysRevD.60.098701",
      eprint         = "hep-ph/9902448",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-020-99",
      SLACcitation   = "%%CITATION = HEP-PH/9902448;%%"
}

@article{Cabarcas:2009vb,
      author         = "Cabarcas, J. M. and Gomez Dumm, D. and Martinez, R.",
      title          = "{Flavor changing neutral currents in 331 models}",
      journal        = "J. Phys.",
      volume         = "G37",
      year           = "2010",
      pages          = "045001",
      doi            = "10.1088/0954-3899/37/4/045001",
      eprint         = "0910.5700",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0910.5700;%%"
}

@Article{Martínez2007,
author="Martinez, R.
and Ochoa, F.",
title="{The Landau pole and Z' decays in the 331 dilepton model}",
journal="The European Physical Journal C",
year="2007",
month="Aug",
day="01",
volume="51",
number="3",
pages="701--711",
abstract="We calculate the decay widths and branching ratios of the extra neutral boson Z' predicted by the 331 dilepton model in the framework of two different particle contents. These calculations are performed taking into account oblique radiative corrections and flavor changing neutral currents (FCNC) under the ansatz of Matsuda as a texture for the quark mass matrices. Contributions of the order of 10-1--10-2 are obtained in the branching ratios, and the partial widths about one order of magnitude bigger in relation with other 331 models are also obtained. A Landau-like pole arises at 3.5 TeV considering the full particle content of the minimal dilepton model (MDM), where the exotic sector is considered as a degenerate spectrum at the 3 TeV scale. The Landau pole problem can be avoided at the TeV scales if a new leptonic content running below the threshold at 3 TeV is implemented as suggested by other authors. ",
issn="1434-6052",
doi="10.1140/epjc/s10052-007-0307-6",
url="https://doi.org/10.1140/epjc/s10052-007-0307-6"
}


@article{Martinez:2009ik,
      author         = "Martinez, R. and Ochoa, F.",
      title          = "{Heavy quark signals from radiative corrections to the
                        Z-prime boson decay in 3-3-1 models}",
      journal        = "Phys. Rev.",
      volume         = "D80",
      year           = "2009",
      pages          = "075020",
      doi            = "10.1103/PhysRevD.80.075020",
      eprint         = "0909.1121",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0909.1121;%%"
}

@article{Cabarcas:2008ys,
      author         = "Cabarcas, J. M. and Gomez Dumm, D. and Martinez, R.",
      title          = "{Phenomenological aspects of the exotic $T$ quark in 331
                        models}",
      journal        = "Eur. Phys. J.",
      volume         = "C58",
      year           = "2008",
      pages          = "569-578",
      doi            = "10.1140/epjc/s10052-008-0803-3",
      eprint         = "0809.0821",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:0809.0821;%%"
}
@article{CarcamoHernandez:2005ka,
      author         = "Carcamo Hernandez, A. E. and Martinez, R. and Ochoa, F.",
      title          = "{Z and Z' decays with and without FCNC in 331 models}",
      journal        = "Phys. Rev.",
      volume         = "D73",
      year           = "2006",
      pages          = "035007",
      doi            = "10.1103/PhysRevD.73.035007",
      eprint         = "hep-ph/0510421",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0510421;%%"
}

@article{Ochoa:2005ch,
      author         = "Ochoa, Fredy and Martinez, R.",
      title          = "{Family dependence in $\mathrm{SU(3)_c \otimes SU(3)_L \otimes
                        U(1)_X}$ models}",
      journal        = "Phys. Rev.",
      volume         = "D72",
      year           = "2005",
      pages          = "035010",
      doi            = "10.1103/PhysRevD.72.035010",
      eprint         = "hep-ph/0505027",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0505027;%%"
}

@article{GonzalezSprinberg:2005zd,
      author         = "Gonzalez-Sprinberg, G. A. and Martinez, R. and Sampayo,
                        O.",
      title          = "{Bilepton and exotic quark mass limits in 331 models from
                        Z ---> b anti-b decay}",
      journal        = "Phys. Rev.",
      volume         = "D71",
      year           = "2005",
      pages          = "115003",
      doi            = "10.1103/PhysRevD.71.115003",
      eprint         = "hep-ph/0504078",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0504078;%%"
}
@article{Diaz:2004fs,
      author         = "Diaz, Rodolfo A. and Martinez, R. and Ochoa, F.",
      title          = "{$\mathrm{SU(3)_c \otimes SU(3)_L \otimes
                        U(1)_X}$ models for beta arbitrary
                        and families with mirror fermions}",
      journal        = "Phys. Rev.",
      volume         = "D72",
      year           = "2005",
      pages          = "035018",
      doi            = "10.1103/PhysRevD.72.035018",
      eprint         = "hep-ph/0411263",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0411263;%%"
}

@article{Diaz:2003dk,
      author         = "Diaz, Rodolfo A. and Martinez, R. and Ochoa, F.",
      title          = "{The Scalar sector of the $\mathrm{SU(3)_c \otimes SU(3)_L \otimes
                        U(1)_X}$
                        model}",
      journal        = "Phys. Rev.",
      volume         = "D69",
      year           = "2004",
      pages          = "095009",
      doi            = "10.1103/PhysRevD.69.095009",
      eprint         = "hep-ph/0309280",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0309280;%%"
}

@article{Dias:2005jm,
      author         = "Dias, Alex G. and Doff, A. and de S. Pires, C. A. and
                        Rodrigues da Silva, P. S.",
      title          = "{Neutrino decay and neutrinoless double beta decay in a
                        3-3-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D72",
      year           = "2005",
      pages          = "035006",
      doi            = "10.1103/PhysRevD.72.035006",
      eprint         = "hep-ph/0503014",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0503014;%%"
}

@article{Montero:2000ar,
      author         = "Montero, J. C. and de Sousa Pires, Carlos Antonio and
                        Pleitez, V.",
      title          = "{Neutrinoless double beta decay with and without Majoron
                        - like boson emission in a 3-3-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D64",
      year           = "2001",
      pages          = "096001",
      doi            = "10.1103/PhysRevD.64.096001",
      eprint         = "hep-ph/0003284",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-033-2000",
      SLACcitation   = "%%CITATION = HEP-PH/0003284;%%"
}

@article{Montero:2001tq,
      author         = "Montero, J. C. and de S. Pires, C. A. and Pleitez, V.",
      title          = "{Lepton masses from a TeV scale in a 3-3-1 model}",
      journal        = "Phys. Rev.",
      volume         = "D66",
      year           = "2002",
      pages          = "113003",
      doi            = "10.1103/PhysRevD.66.113003",
      eprint         = "hep-ph/0112203",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-073-2001",
      SLACcitation   = "%%CITATION = HEP-PH/0112203;%%"
}

@article{Montero:1999mc,
      author         = "Montero, J. C. and de Sousa Pires, Carlos Antonio and
                        Pleitez, V.",
      title          = "{Spontaneous breaking of a global symmetry in a 331
                        model}",
      journal        = "Phys. Rev.",
      volume         = "D60",
      year           = "1999",
      pages          = "115003",
      doi            = "10.1103/PhysRevD.60.115003",
      eprint         = "hep-ph/9903251",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFT-P-022-99",
      SLACcitation   = "%%CITATION = HEP-PH/9903251;%%"
}

@inproceedings{Abchiche:2016ywf,
      author         = "Abchiche, A. and others",
      title          = "{Contributions of the Cherenkov Telescope Array (CTA) to
                        the 6th International Symposium on High-Energy Gamma-Ray
                        Astronomy (Gamma 2016)}",
      booktitle      = "{Proceedings, 6th International Symposium on High-Energy
                        Gamma-Ray Astronomy (Gamma 2016): Heidelberg, Germany,
                        July 11-15, 2016}",
      year           = "2016",
      eprint         = "1610.05151",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1610.05151;%%"
}

@proceedings{Proceedings:2016rni,
      editor         = "Szczerbinska, Barbara and Allahverdi, Rouzbeh and Babu,
                        Kaladi and Balantekin, Baha and Dutta, Bhaskar and Kamon,
                        Teruki and Kumar, Jason and Queiroz, Farinaldo and
                        Strigari, Louis and Surman, Rebecca",
      title          = "{Proceedings, Workshop on Neutrino Physics : Session of
                        CETUP* 2015 and  9th International Conference on
                        Interconnections between Particle Physics and Cosmology
                        (PPC2015)}",
      year           = "2016",
      url            = "http://aip.scitation.org/toc/apc/1743/1",
      journal        = "AIP Conf. Proc.",
      volume         = "1743",
      ISBN           = "9780735414006",
      SLACcitation   = "%%CITATION = APCPC,1743,;%%"
}

@article{Baring:2015sza,
      author         = "Baring, Matthew G. and Ghosh, Tathagata and Queiroz,
                        Farinaldo S. and Sinha, Kuver",
      title          = "{New Limits on the Dark Matter Lifetime from Dwarf
                        Spheroidal Galaxies using Fermi-LAT}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "10",
      pages          = "103009",
      doi            = "10.1103/PhysRevD.93.103009",
      eprint         = "1510.00389",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CETUP2015-025",
      SLACcitation   = "%%CITATION = ARXIV:1510.00389;%%"
}



@article{Liu:1993fwa,
      author         = "Liu, James T. and Ng, Daniel",
      title          = "{Z - Z-prime mixing and oblique corrections in an SU(3) x
                        U(1) model}",
      journal        = "Z. Phys.",
      volume         = "C62",
      year           = "1994",
      pages          = "693-700",
      doi            = "10.1007/BF01574173",
      eprint         = "hep-ph/9302271",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "IFP-460-UNC, TRI-PP-93-11",
      SLACcitation   = "%%CITATION = HEP-PH/9302271;%%"
}






